Quantum Extremal Islands Made Easy, Part I: Entanglement on the Brane

Recent progress in our understanding of the black hole information paradox has lead to a new prescription for calculating entanglement entropies, which involves special subsystems in regions where gravity is dynamical, called \textit{quantum extremal islands}. We present a simple holographic framework where the emergence of quantum extremal islands can be understood in terms of the standard Ryu-Takayanagi prescription, used for calculating entanglement entropies in the boundary theory. Our setup describes a $d$-dimensional boundary CFT coupled to a ($d$-1)-dimensional defect, which are dual to global AdS${}_{d+1}$ containing a codimension-one brane. Through the Randall-Sundrum mechanism, graviton modes become localized at the brane, and in a certain parameter regime, an effective description of the brane is given by Einstein gravity on an AdS${}_d$ background coupled to two copies of the boundary CFT. Within this effective description, the standard RT formula implies the existence of quantum extremal islands in the gravitating region, whenever the RT surface crosses the brane. This indicates that islands are a universal feature of effective theories of gravity and need not be tied to the presence of black holes.

==> sections/HEE.tex <==
% !TEX root = ../lifeonbrane3.tex
In this section we relate the brane setup to the calculation of entanglement entropies for regions on the boundary CFT whose RT surface falls deep into the bulk and connects to the brane.

In AdS/CFT, branes such as the ones describes above play an essential role in the description of Boundary CFT (BCFT). If the CFT itself is living on a manifold with a boundary, the holographic prescription states that the dual geometry consists also of a manifold with a boundary - an AdS-like spacetime that ends on a brane, which is itself anchored at the boundary of the CFT (an `end-of-the-world brane') \cite{ads/bcft}.

In general, the holographic recipe shows that the entanglement entropy of a subregion $A$ of the field theory is given by an extremal surface $\sigma$ that is anchored at the asymptotic boundary at $A$, that extends into the bulk and remains homologous to $A$. In the case of a BCFT, the new ingredient is that the R-T surface $\sigma$ is also allowed to end up at the brane. This introduces a new set of interesting `candidate' surfaces that compete in the minimization process.

Recently, a new formula for the computation of holographic entanglement entropy was proposed, relevant for situations when the quantum system of interest is in contact with another system that contains gravity as a dynamical field. We will investigate this formula using the same bulk setup as described in previous sections. \iar{explain some more}

\subsection{Bulk RT to Brane Wald}\label{sec:genera}

In this subsection we study the leading order contributions to holography entanglement entropies for our brane setup in arbitrary dimension. We find that the Wald-Dong entropies associated to the induced $d$-dimensional gravity action match the leading order contributions from the RT surface in the $(d+1)$-dimensional bulk.


\subsubsection{Bulk RT surface contributions \label{bulkrt}}

As before, the bulk consists of two copies of a patch of global AdS$_{d+1}$, glued together along that surface, which creates a spacetime with a tensionfull brane located at that surface. The asymptotic boundary now consists of two copies of a hemisphere cross time, $S^{d-1}\times \mathbb R_t$, glued along a defect. As our entangling region, we choose two identical discs, centered at the pole of each hemisphere, see figure \ref{fig:rtsurface}, which depicts half of the geometry. In this setting, the R-T surface $\sigma$ has two different `phases'. The disconnected or `trivial' phase (phase "I") consists of two independent surfaces with the topology of a disc. On the other hand, in phase II the R-T surface ends on the brane at some codimension-$3$ surface $\del \sigma_B$, which due to symmetry will correspond to a higher dimensional sphere. \iar{add figure of phase I and II}.

%\begin{figure}[h]
%	\centering
%	\includegraphics[width=0.5\linewidth]{images/rtSurface}
%	\caption{Sketch of RT surface for AdS$_4$. Sorry but I messed up the labellings... $\sigma_A$ is should be on the top and $\sigma_B$ is on the bottom. \iar{Can we actually stick to the labelling as in the figure? looks much more natural} }
%	\label{fig:rtsurface}
%\end{figure}


\begin{figure}[h]
	\def\svgwidth{0.6\linewidth}
	\centering{
		\input{3dBrane.pdf_tex}
		\caption{A timeslice of AdS$_{d+1}$ space. Constant $\rho$ hyperbolic foliations are drawn and a brane lives on an AdS$_d$ slice at large $\rho$. On the other boundary of the bulk spacetime lies a $d$-dimensional CFT.
		}
		\label{fig:cutoffs}
	}
\end{figure}



\josh{the area labelling notation should be cleaned up.}

Following Faulkner et al. \cite{Faulkner:2013ana}, we expect \iar{But we are going to prove this later?}
\beq\label{gen}
S_{EE} = \text{ext}\Big(2\frac{A(\sigma)}{4 \Gbk}+ \frac{A(\partial\sigma_\mt{brane})}{4 \Gbr}\Big)\,,
\eeq where $\partial \sigma_\mt{brane}$ is the area of the intersection of the surface $\sigma$ and the brane. The factor of two in the bulk area term accounts for our two bulks that are glued together along the brane.


Before solving for the area of the surface between a disk on the lower AdS boundary and the brane we will first understand the dominant behaviour at very large tension and small $\delta_\mt{CFT}$ cutoff, which is a UV cutoff around the CFT boundary. Since we are considering the leading order behaviour, we simply apply the Fefferman-Graham coordinates for some asymptotic metric and set the cutoff in the radial $z$ coordinate. Since the geometry in question is time-independent, we perform all calculations on a fixed timeslice.

Recall that to compute an extremal areas we parametrize the surface by parameters $\xi^i$ and set up an variational problem in terms of an action for the surface area. For instance, in the Fefferman-Graham coordinates for AdS$_{d+1}$, we have
\beq
I_\mt{extremal}=\int d^{d-1}\xi \frac{L^{d-1}}{z^{d-1}}\sqrt{\det\Big(\frac{\partial z}{\partial \xi^i} \frac{\partial z}{\partial \xi^j} + g_{k l} (x,z)\frac{\partial x^{k}}{\partial \xi^i} \frac{\partial x^{l}}{\partial \xi^i} \Big)}\,.
\eeq

Following Rangamani and Takayanagi's book \cite{Rangamani_2017}, we find that around small $z$ in Fefferman-Graham coordinates the metric on the extremal surface $\sigma$ is decomposed as
\beq
ds^2_{\sigma}=\frac{L^2}{z^2}(dz^2 + \tilde{\gamma}_{a b}d\alpha^a d\alpha^b)\,,
\eeq where $\alpha_i$ are coordinates on the entangling surface. Assuming that the minimal surface falls straight into the bulk from the CFT boundary, we fix $\xi^1$ to be $z$ and find that the leading contribution to the area at this boundary is
\beq\label{area}
A(\sigma)_{\delta_B} = \int_{\delta_B}^{z_{IR}}\frac{L^{d-1}dz}{z^{d-1}}\int d\xi^{d-2}\sqrt{\tilde{\gamma}}+\dots=\frac{ L^{d-1}A(\partial \sigma_\mt{CFT})}{(d-2)\delta_B^{d-2}}+\dots\,,
\eeq where $\partial \sigma_\mt{CFT}$ is the area of the entangling surface on CFT boundary.\iar{clarify here} We can play the same game at the $\rho=\rho_*$ end of the surface, although in this calculation we ``rebundle" the divergent quantity into the induced metric on the brane, as in (\ref{bundle}).

Explicitly, the calculation goes as follows:
\beq\label{branearea}
A(\sigma)_{brane} = \int_s^{z_{IR}} dz \Big[\frac{L^{d-1}}{z^{d-1}}\Big(1+\frac{1}{2}\frac{z^2}{L^2}+\frac{1}{16}\frac{z^4}{L^4}\Big)^{\frac{d-2}{2}}\Big]\int d^{d-2}x \sqrt{-\bar{g}_{AdS_d}}\,,
\eeq where here $\bar{g}_{AdS_d}$ related to the induced metric on the intersection of the brane and the RT surface (denoted $\bar{g}_{ij}$) by
\beq
\bar{g}_{ij} = \frac{L^2}{s^2}\Big(1+\frac{1}{2}\frac{s^2}{L^2}+\frac{1}{16}\frac{s^4}{L^4}\Big) \bar{g}_{ij}^{AdS_d}\,.
\eeq We now simply integrate over the $z$ direction and find, after expanding at small $s$,
\beq\label{brane area}
A(\sigma)_{brane} = \frac{L}{d-2}A(\partial \sigma_\mt{brane}) + \frac{1}{2(d-4)}\frac{s^2}{L}A(\partial \sigma_\mt{brane}) + \mathcal{O}(s^4/L^4)\,.
\eeq
From the calculations above we expect that to leading order
\beq\label{bulk area}
\frac{A(\sigma)}{4 \Gbk}=\frac{L^{d-1}A(\partial \sigma_\mt{CFT})}{4 (d-2)\Gbk \delta_B^{d-2}} + \frac{L A(\partial \sigma_\mt{brane})}{4(d-2) \Gbk}\,.
\eeq Therefore we find
\beq
S_{EE} = \frac{2 L^{d-1}A(\partial \sigma_\mt{CFT})}{4 (d-2)\Gbk \delta_B^{d-2}} + \frac{A(\partial \sigma_\mt{brane})}{4 \Geff}\,,
\eeq where
\beq
\frac{1}{\Geff} = \frac{2 L}{(d-2) }\frac{1}{\Gbk} + \frac{1}{\Gbr}\,,
\eeq which matches (\ref{Geff}) as was desired. Note that we included two contributions of the bulk area (\ref{bulk area}) to account for both sides of the AdS space. Hence we see that the Wald entropy associated to the induced action term is really contained in the bulk RT surface and not a genuine generalized correction to the entanglement entropy. \iar{Good, but need to clarify}. In section \ref{Wald}, we compare the second order term of equation (\ref{brane area}) to the Wald entropy for the curvature-squared terms of the induced action.


\subsubsection{Wald entropies \label{Wald}}

In the generalized entanglement entropy there are contributions from the brane action which take the form of the Wald entropy, as justified in section \ref{waldjustification}.

We start by computing the Wald entropy for the standard Einstein-Hilbert action because of its relevance to both the induced brane action and physical brane action. The Wald entropy formula is \cite{Myers:2010tj}
\beq
S = -2\pi \int_{\Sigma}d^{d-2}x\sqrt{-h}\frac{\partial\mathcal{L}}{\partial R^{ab}_{\,\,\,\,\,cd}}\hat{\epsilon}^{ab}\hat{\epsilon}_{cd}\,,
\eeq where $\mathcal{L}$ is the Lagrangian density and $\hat{\epsilon}_{ab}$ is the binormal to the region $\Sigma$, and $h_{ij}=\tilde{g}_{ij}$ is the induced metric along that region. In our setup, $\Sigma\equiv \partial\sigma_\mt{brane}$ is the ($d-2$)-dimensional intersection surface between the brane and the bulk Ryu-Takayanagi (RT) surface. As in section \ref{bulkrt}, we refer to the induced metric along this surface by $\bar{g}_{ij}$, which is simply the restriction of $\tilde{g}$ to the surface $\partial\sigma_\mt{brane}$.

Note that the integrand is constant along the brane in our geometry so the equation reduces to
\beq
S = -2\pi \frac{\partial\mathcal{L}}{\partial R^{ab}_{\,\,\,\,\,cd}}\hat{\epsilon}^{ab}\hat{\epsilon}_{cd}\int_{\partial\sigma_\mt{brane}}d^{d-2}x\sqrt{-\bar{g}} = -2\pi \frac{\partial\mathcal{L}}{\partial R^{ab}_{\,\,\,\,\,cd}}\hat{\epsilon}^{ab}\hat{\epsilon}_{cd} A(\partial\sigma_\mt{brane}) \,.
\eeq
The Einstein-Hilbert Lagrangian density takes the form
\beq
\mathcal{L} = \alpha \tilde{R} = \alpha \tilde{R}^{ab}_{\,\,\,\,\,cd} \tilde{g}^{ic}\tilde{g}^{jd}\tilde{g}_{ai}\tilde{g}_{bj}\,
\eeq from which we compute
\beq
\hat{\epsilon}^{ab}\hat{\epsilon}_{cd}\frac{\partial\mathcal{L}}{\partial \tilde{R}^{ab}_{\,\,\,\,\,cd}} =\alpha \hat{\epsilon}^{ab}\hat{\epsilon}_{cd} \tilde{g}^{ic}\tilde{g}^{jd}\tilde{g}_{ai}\tilde{g}_{bj} = -2 \alpha\,,
\eeq where we used $\hat{\epsilon}^{ij}\hat{\epsilon}_{ij} = -2$ from \cite{Myers:2010tj}. For the actions on the brane, this gives the standard result
\beq
S_{brane} = \frac{A(\partial\sigma_\mt{brane})}{4 \Gbr}\,\,\,\,\,\text{and}\,\,\,\,\, S_{induced}^{(1)} = \frac{L A(\partial\sigma_\mt{brane})}{4(d-2)\Gbk}\,.
\eeq These standard results were already used at the end of section \ref{bulkrt}. As promised, we can use this formalism to study the higher curvature terms in the induced brane action to ensure that they provide the same information as the area of the bulk RT surface.

We first consider the two curvature-squared terms independently, which will be combined by linearity. Consider the Lagrangian density
\beq
\mathcal{L} = \kappa R^2\implies \hat{\epsilon}^{ab}\hat{\epsilon}_{cd}\frac{\partial\mathcal{L}}{\partial R^{ab}_{\,\,\,\,\,cd}} = - 4 \kappa R\,.
\eeq Also, we need to consider
\beq\label{RicciTensorTerm}
\mathcal{L} = \gamma R^{de}R_{de} =\gamma R^{ab}_{\,\,\,\,\,cd}R^{\,\,\,\,\,ld}_{jk}g_{ai}g_{be}g^{ic}g_{jm}g_{ml}g^{ke}\implies \hat{\epsilon}^{ab}\hat{\epsilon}_{cd}\frac{\partial\mathcal{L}}{\partial R^{ab}_{\,\,\,\,\,cd}} =-4\gamma\hat{R}\,,
\eeq
whenever $R_{ij} = \hat{R}g_{ij}$.
Now we turn to the curvature-squared terms of the induced bulk action (\ref{bulkaction}). Applying the variations above, we find
\beq
S_{induced}^{(2)} = \frac{8 L^3 s^2}{(d-4)(4L^2+s^2)^2}\frac{A(\partial\sigma_\mt{brane})}{4 \Gbk}\,.
\eeq Now expanding this to leading order in $s$, we find
\beq
S_{induced}^{(2)} = \frac{ s^2}{2(d-4)L}\frac{A(\partial\sigma_\mt{brane})}{4 \Gbk}\,,
\eeq which matches the analogous term from \ref{brane area}.

\subsubsection{Dong entropies and extrinsic curvature corrections}

So far we ignored the extrinsic curvatures of the entangling surface on the brane. Following \cite{Bhattacharyya_2014_2, Dong_2014}, we consider a second derivative theory of gravity ($\mathcal{L}^{(2)} = \lambda_1 \tilde{R}^2 + \lambda_2 \tilde{R}_{\mu\nu}\tilde{R}^{\mu\nu}$) with entropy
\beq\label{dong}
S = -4\pi \int d^{d-2}x \sqrt{-\bar{g}}\Big[2 \lambda_1 \tilde{R} +\lambda_2 \Big(\tilde{R}_{\mu\nu}n_i^{\mu}n_i^{\nu}-\frac{1}{2}\tilde{\mathcal{K}}_i\tilde{\mathcal{K}}^i\Big)\Big]\,,
\eeq where $n_i$'s are the two normals to the entangling surface. Note that in our setup,
\beq
\tilde{R}_{\mu\nu}n_i^{\mu}n_i^{\nu} = \hat{R}\tilde{g}_{\mu\nu}n_i^{\mu}n_i^{\nu} = \hat{R}\sum_{i=1}^2 n_i^{\mu}n_{i \mu} = 2\hat{R}\,,
\eeq where we used the normalization of the normal vector. This contribution to the entropy agrees with equation (\ref{RicciTensorTerm}). In our calculations below we consider only the one-sided bulk. Including both contributions simply requires a factor of two multiplying the Dong entropy.

We now present an argument to show that the minimal surface calculation also includes the extrinsic term of equation (\ref{dong}). The argument follows \cite{Hung_2011}.

First we describe the embedding of the RT surface by the bulk coordinates $X^{\mu} = {x^i,z}$, which can be expanded near the brane surface as
\beq
X^i(y^a, z) = X^{(0)i}(y^a) + \frac{z^2}{L^2}X^{(1)i}(y^a)+\dots\,,
\eeq where $y^a$ are the coordinates along the bulk surface. The induced metric along the surface is given by
\beq
h_{\alpha\beta} = \partial_{\alpha}X^{\mu}\partial_{\beta}X^{\nu}G_{\mu\nu}[X]\,,
\eeq which can be expanded around the brane as
\beq
h_{zz} = \frac{L^2}{z^2}\Big(1+\frac{z^2}{L^2}h_{zz}^{(1)}+\dots\Big),\,\,\,\,\, h_{ab}=\frac{L^2}{z^2}\Big(h^{(0)}_{ab}+\frac{z^2}{L^2}h^{(1)}_{ab}+\dots\Big)\,.
\eeq
Note that $h_{ab}=\tilde{g}_{ab}|_{\sigma_b}$ is the induced metric at the intersection of the RT surface and the brane. Now when we studied the behaviour of the RT surface in equation (\ref{branearea}), we assumed that the brane fell straight into the bulk, which is why the extrinsic curvature contributions did not appear. The correct expansion around the brane is \cite{Hung_2011}
\begin{multline}\label{correctedarea}
A(\sigma)_{brane} = \int_s^{z_{IR}}dz \Big[\frac{L^{d-1}}{z^{d-1}}\Big(1+\frac{1}{2}\frac{z^2}{L^2}+\frac{1}{16}\frac{z^4}{L^4}\Big)^{\frac{d-2}{2}}\Big]\int d^{d-2}x \sqrt{-\bar{g}_{AdS_d}}\\\times\Big[1+\Big(h^{(1)}_{zz}+h^{(0)ab}h^{(1)}_{ab}\Big)\frac{z^2}{2L^2}+\dots \Big]\,,
\end{multline} where we notice that the first-order term was the contribution evaluated already. We now focus on the second order term. To raise the indices in the $h^{(0)ab}$, we used the metric $h^{ab}$, which is order $z^2/L^2$. Hence we see that at second order we only need to focus on the $h^{(1)}_{zz}$ term. \josh{Check this is correct, i.e. this second term is indeed subdominant. ALSO, double-check that $\tilde{\mathcal{K}}_i$ is the same as the $K_i$ in Dong.}

It was shown in \cite{Hung_2011} that the second-order contribution to the RT surface embedding coordinates can be written in terms of the extrinsic curvature,
\beq
X^{(1)i} = \frac{L^2 \tilde{\mathcal{K}}^i}{2(d-2)}\,,
\eeq and the induced metric can be expanded via
\beq
h_{zz} = \frac{L^2}{z^2}\Big(1+\frac{4z^2}{L^4}(X^{(1)i})^2+\dots\Big)\implies h^{(1)}_{zz} = \frac{L^2 (\tilde{\mathcal{K}}^i)^2}{(d-2)^2}\,.
\eeq
We now substitute this expression into equation (\ref{correctedarea}) and integrate out the $z$ direction. Upon expanding at small $s$, we obtain
\beq
A(\sigma)^{(1)}_{brane} = \frac{L s^2}{2 (d-4)(d-2)^2}(\tilde{\mathcal{K}}^i)^2 \int d^{d-2}x \sqrt{-\tilde{g}}\,,
\eeq and hence the second order contribution to the entanglement entropy is
\beq
S^{(1)} = \frac{1}{4 \Gbk} \frac{L s^2}{2 (d-4)(d-2)^2}(\tilde{\mathcal{K}}^i)^2 A(\partial\sigma_\mt{brane})\,,
\eeq which precisely matches equation (\ref{dong}) after computing $\lambda_2$ from the induced brane action (\ref{bulkaction}),
\beq
\lambda_2= \frac{L^3}{16 \pi(d-4)(d-2)^2 \Gbk}\,.
\eeq
\josh{I need to be a bit more careful... the left over $s^2/L^2$ comes from the raising and lowering of the $i$ indices compared to Dong's formula or from the metric in Dong's formula?.}
From these calculations we conclude that the entropies associated to the induced action on the brane in the Randall-Sundrum picture give exactly the leading contributions to the RT surface area in the $(d+1)$-dimensional bulk!







\subsubsection{A comment on $d=2$ case}

We see that the equations are slightly different in $d=2$ since the calculation in (\ref{area}) will introduce a log rather than a powerlaw behaviour. This will again match the RS-picture side.

The leading order behaviour of the bulk RT surface is just a single integral,
\beq
S = \frac{1}{4 G_3}\int_{s}^{\lambda} \frac{L}{z}dz = -\frac{L}{4G_3} \log\Big(\frac{s}{L}\Big)\,,
\eeq where we have ignored the infrared contribution. We also take the variation of the $d=2$ induced action to compute its Wald entropy \cite{Dong_2014}. We find
\begin{multline}
S = \frac{1}{4 G_{3}}\frac{\partial \mathcal{L}}{\partial \tilde{R}} = \frac{1}{4 G_{3}}\frac{\partial }{\partial \tilde{R}}\Big(\frac{2}{L} -\frac{1}{2}L \tilde{R} \log\Big(-\frac{L^2}{ 2} \tilde{R}\Big) + \frac{L}{2}\tilde{R}+\frac{L^3}{16}\tilde{R}^2\Big)\\=-\frac{L}{4G_3} \log\Big(\frac{s}{L}\Big)\,,
\end{multline} which matches the RT surface calculation (after expanding to leading order in $s$)!



\subsection{Examples}\label{sec:examples}

\rcm{Let's stream line this, \ie minimize the number of coordinate systems/transformations. Don't need embedding space or Poincare coordinates, etcetera:}

Recall that eq.~\reef{metric} described the AdS$_{d+1}$ geometry foliated by AdS$_d$ slices with
\beq\label{metric1a}
ds^2 %= g_{ab}\,dx^{a}dx^{b}
= d\rho^2 + \cosh^2\left({\rho}/{L}\right)\, g_{ij}^{\mt{AdS}_d}\,dx^{i}dx^{j}\,.
\eeq
but we really discussed the brane geometry and the background solution in terms of eq.~\reef{metric3}
\beq\label{metric3a}
ds^2=\frac{L^2}{z^2}\left[dz^2 +  \left(1 + \frac{z^2}{4\,L^2}\right)^2 g_{ij}^{\mt{AdS}_d}\,dx^{i}dx^{j} \right]\,.
\eeq 
So I would really prefer to start with these coordinates! While these coordinates are ideally suited to discuss the brane geometry and the back-reacted background, we would also like to consider `global' coordinates for the AdS$_{d+1}$ geometry
\beq\label{metric2s}
ds^2=L^2\left[-\cosh^2\!r\,dt^2+dr^2+\sinh^2\!r\,d\Omega_{d-1}^2 \right]\,.
\eeq 
These coordinates are better adapted to discuss the boundary theory, which we consider to be on an $R\times S^{d-1}$ background. While we refered to these as `global' coordinates, they do not cover the entire back-reacted bulk solution depicted in figure \ref{fig:brane2}. Rather we could use the coordinates in eq.~\reef{metric2s} to cover two patches on either side of the brane and near the asymptotic AdS$_{d+1}$ boundary.

\rcm{So what is the coordinate transformation between eqs.~\reef{metric3a} and \reef{metric2s}?? need to pick some `nice' coordinates for $g_{ij}^{\mt{AdS}_d}\,dx^{i}dx^{j}$ in eq.~\reef{metric3a}. It would be convenient if we can use the same time $t$ in both metrics. Is this transformation needed? Yes because we will need to describe the brane location $z=z_\mt{B}$ in the following.} 

Now following \cite{Krtous:2014pva}, we introduce cylindrical coordinates
\beq\label{cylindd}
ds^2=L^2\[ -\rcm{???}dt^2+\frac{dP^2}{1+P^2}+\left( 1+P^2 \right)d\zeta^2+P^2\,d\Omega_{d-2}^2\]
\eeq
\rcm{Note that I want to show the full spacetime metric and I want to show a metric for AdS$_{d+1}$. Where is the $r$ cutoff in global/spherical coordinates? Shouldn't matter in comparing areas but be careful.}

\rcm{Now what is the coordinate transformation between eq.~\reef{metric2s} and \reef{cylindd}?? What is the position of the brane in the cylindrical coordinates?}

\rcm{Now should be able to start, \eg set up eqs.~\reef{area} and \reef{zetap}, in general dimensions. Only then proceed to $d=3$ and proceed with explicit calculations for the example. Somewhere in there (\ie $d=3$) we have to talk about adding Gauss-Bonnet term to bulk gravity and adding Euler character to RT formula!
 (Working first part with general $d$ allows us to do bubbles in general dimensions in next section.)}


\rcm{*****************************}

In this section, we consider concrete examples of the construction outlined in the previous sections. We work out explicitly the cases of bulk AdS$_{d+1}$ spacetimes with $d=2,3,4$. As before, we begin by examining $d>2$ first, since it is simpler in that the analysis can be done purely in terms of Einstein (or higher derivative) gravity. We then turn to $d=2$, which involves the addition of a Jackiw-Teitelboim term for the dilaton.

In particular, we are interested in exploring the physics of quantum systems that are entangled with degrees of freedom in a theory with gravity. According to a recent proposal, the formula for the generalised entanglement entropy must include an extra term, that of eq. \eqref{gen} \cite{Almheiri:2019hni}. Our setup is one of the simplest scenarios where to test this proposal explicitly.

As usual, the areas of surfaces in both the connected and disconnected phases are UV divergent. Since we will be mainly interested in the connected solution (phase II), we will always work with the renormalised area obtained by subtracting the contribution of phase I, rendering a finite result. In this way, one can safely take the UV cutoff to infinity from the beginning of the calculations.

We begin with a general analysis for an AdS$_d$ brane embedded in AdS$_{d+1}$. We then consider the particular case of $d=3$, where most computations can be done analytically. In order to introduce the coordinate system, we begin with the basics. As usual, AdS$_{d+1}$ is defined by
\begin{align}\label{adsdef}
-U^2-V^2+\sum_{i=1}^{d} X_i^2=-L^2
\end{align}
embedded into $\mathbb R^{2,d}$. As is well known, the following change of coordinates
\begin{align}\label{}
U&=\frac{z}{2}\left( 1+\frac{L^2-t^2+\vec{x}^2}{z^2} \right) \\
X_{d}&= \frac{z}{2} \left( 1-\frac{L^2+t^2-\vec{x}^2}{z^2} \right) \\
V&=\frac{Lt}{z}\\
X_j&=\frac{Lx_j}{z}\ \ ,\ \ j=1,\hdots,d-1
\end{align}
with $\vec{x}=(x_1,\hdots,x_{d-1})$ leads to the Poincare half space metric,
\begin{align}\label{Poincare}
ds^2=L^2 \frac{dz^2-dt^2+ d\vec{x}^2}{z^2}
\end{align}

Another representation that will be useful for us is achieved by performing a further change of variables in the $(z,x_j)$ for a given $j$. Without loss of generality, let us simply choose $j=1$, and transform according to
\begin{align}\label{zx1}
z=\frac{y}{\cosh \left( \rho/L \right)}\ \ ,\ \ x_1=y\tanh\left( \rho/L \right)
\end{align}
while leaving all other coordinates unchanged. This leads to the metric already given in \eqref{metric},
\begin{align}\label{hyper}
ds^2=d\rho^2+\cosh^2\left( \rho/L \right) ds^2_{\text{AdS}_{d}}
\end{align}
where the AdS$_d$ metric take the Poincare form
\begin{align}\label{}
ds^2_{\text{AdS}_{d}}&=L^2 \frac{dy^2-dt^2+dx_2^2+\hdots dx_{d-1}^2}{y^2}
\end{align}

The metric \eqref{hyper} represents a \textit{hyperbolic} foliation of AdS space: surfaces of constant $\rho$ correspond also to AdS$_{d}$, embedded in the global AdS$_{d+1}$. Moreover, these surfaces possess a constant value of the extrinsic curvature scalar $\mathcal{K}$. In terms of the Poincare coordinates \eqref{Poincare}, these are defined by planes of a given slope in the $(x_1,z)$ directions which can be parametrized by their respective value for $\rho$:
\begin{align}\label{}
\frac{x_1}{z}=\frac{X_1}{L}=\sinh \left( \rho/L \right)
\end{align}

Of course, as mentioned above, due to symmetry the same would apply to any other $x_{j}$ (or $X_j$) for $j=1,\hdots,d-1$, had we chosen it instead of $x_1$ ($X_1$) in \eqref{zx1}. This simply reflects the $SO(d-1)$ rotational symmetry of \eqref{adsdef}.

Finally, another representation of AdS$_{d+1}$ is the well known global chart in spherical coordinates:
\begin{align}\label{}
U&=L\cosh r \cos \tau\\
V&=L\cosh r \sin \tau\\
X_i&=L\sinh r\ \hat{x}_i\ \ \ ,\ \ i=1,\hdots,d
\end{align}
with $\sum_{i=1}^{d}\hat{x}_i^2=1$ so the $\hat{x}_i$ parametrize the unit sphere $S^{d-1}$, and the metric reads
\begin{align}\label{globalads}
ds^2=L^2\left( -\cosh^2r\, d\tau^2+dr^2+\sinh^2 r\, d\Omega_{d-1}^2 \right)
\end{align}

In these coordinates, a hypersurface of constant $X_j$ - equivalent to a fixed $\rho$ as discussed above - corresponds to
\begin{align}\label{brane}
\frac{X_i}{L}=\sinh r\, \hat{x}_i=\sinh \left(  \rho/L \right)
\end{align}
For simplicity, we will use the freedom to choose the orientation of the spacial spherical axes such that both the entangling surface and the brane have azimuthal symmetry.

\subsubsection{Explicit results in AdS$_{4}$}

In this section we will particularize the discussion to $d=3$, that is our bulk spacetime will be AdS$_4$ and we will consider branes with an induced AdS$_3$ geometry. For this case, some analytic expressions can be obtained. We start by reviewing the problem of finding minimal surfaces in empty global AdS$_4$ first with no brane inserted, as explored in \cite{Krtous:2014pva}. In section \ref{AdS/BCFT} we will use the standard AdS/BCFT tools \cite{Takayanagi:2011zk} to deal with a CFT with a boundary, which requires the introduction of the brane.

Our starting point is the AdS$_4$ metric in global coordinates \eqref{globalads},
\begin{align}\label{}
\frac{ds^2}{L^2}=-\cosh^2 r d\tau^2+dr^2+\sinh^2r \left( d\theta^2+\sin^2\theta d\varphi^2 \right)
\end{align}

Since we will focus on entanglement entropies, we shall fix $\tau=0$ and work with three-dimensional hyperbolic space $\mathbb H^3$
\begin{align}\label{H3}
\frac{ds^2}{L^2}=dr^2+\sinh^2r \left( d\theta^2+\sin^2\theta d\varphi^2 \right)
\end{align}
The main strategy of \cite{Krtous:2014pva} was to move from the spherical coordinates $r,\theta$ to cylindrical coordinates $P,\zeta$ where $\zeta$ specifies the position along the axis of the cylinder while $P$ measure the distance from that axis. The azimuthal angle $\varphi$ is left unchanged.



The transformation is given by
\begin{align}\label{}
\sinh r&=\sqrt{\frac{P^2+\tanh^2\zeta}{1-\tanh^2\zeta}}\\
\tan\theta&=\frac{P}{\sqrt{1+P^2}}\frac{\sqrt{1-\tanh^2\zeta}}{\tanh\zeta}
\end{align}
with $P\in (0,\infty),\zeta\in(-\infty,\infty)$. The equator of the sphere $\theta=\pi/2$ is mapped to the `equator' of the cylinder $\zeta=0$, while the upper (lower) hemisphere is mapped to the upper (lower) half space in the cylindrical system. The conformal boundary at infinity corresponds to $P\to \infty$.

In this coordinates, the spatial section \eqref{H3} takes the particularly simple form
\begin{align}\label{H3cyl}
\frac{ds^2}{L^2}=\frac{dP^2}{1+P^2}+\left( 1+P^2 \right)d\zeta^2+P^2d\varphi^2
\end{align}
The convenience of these coordinates is now evident: the metric \eqref{H3cyl} has now \textit{two} manifest Killing vectors, as it doesn't depend explicitly on either $\varphi$ nor $\zeta$.

In order to make use of this symmetry, we will restrict to settings that possess cylindrical symmetry around $P=0$. We will consider entangling surfaces (circles for $d=3$) that are centred around this axis, and similarly for the brane in section \ref{AdS/BCFT}. Therefore, and without further loss of generality, we choose the axis $\hat{x}_1$ of the brane as the $\theta=0$ line in spherical coordinates, such that both the brane and the entangling surface will be symmetric around $\varphi$.



\paragraph{Minimal surfaces in global AdS$_4$}

As we restrict to settings with cylindrical symmetry, it is convenient to parametrize a surface by $\zeta=\zeta(P)$. The associated area functional is
\begin{align}\label{area}
\frac{A}{L^2}=\int dP P \sqrt{\frac{1}{1+P^2}+(1+P^2)\zeta'^2}
\end{align}
\vc{missing factor of $2\pi$ on RHS from $\varphi$ integral?}The Euler-Lagrange equation associated to \eqref{area} becomes particularly simple since the metric in cylindrical coordinates is independent of $\zeta$. The solution for the derivative is given by
\begin{align}\label{zetap}
\zeta'(P)=\pm \frac{1}{1+P^2}\sqrt{\frac{P_0^4+P_0^2}{P^4+P^2-P_0^4-P_0^2}}
\end{align}
where the two branches correspond to two identical surfaces related by a reflection with respect to $\zeta=0$. As is well known in the holographic context, the minimal surface anchored to a fixed entangling region at conformal infinity needs not be unique. For a given setting there may be multiple local minima of the area functional, and one is instructed to pick the global minima amongst them. This leads to possible `phase transitions' in the RT surface as we now discuss.

The disconnected `trivial' solution corresponds uniquely to $P_0=0$. This implies $\zeta(P)=\zeta_0$ which in cylindrical coordinates looks simply as a disk anchored at the boundary region. The entanglement wedge corresponds to two identical disconnected pieces.

On the other hand, for $P_0>0$ the surface is very nontrivial, and the two branches of \eqref{zetap} meet at the locus $\zeta=\zeta_0,P=P_0$ which is where the minimal surface reaches its maximal depth into the bulk. Integrating the explicit form of the curve \eqref{zetap}, one finds
\begin{align}\label{zetasol}
\zeta(P;P_0,\zeta_0)&=\zeta_0\pm \frac{P_0}{\sqrt{(1+P_0^2)(1+2P_0^2)}} \nonumber \\
&\left[ (1+P_0^2) F\left( \mbox{Arcos} \frac{P_0}{P},\sqrt{\frac{1+P_0^2}{1+2P_0^2}} \right)-P_0^2 \Pi\left( \mbox{Arccos}\frac{P}{P_0},\frac{1}{1+P_0^2},\sqrt{\frac{1+P_0^2}{1+2P_0^2}} \right) \right]
\end{align}

The integration constant $\zeta_0$ corresponds to the value of $\zeta$ when the surfaces reaches the deepest into the bulk, while $F$ and $P$ correspond to the elliptic integrals.


Notice that we are characterising the minimal surfaces \eqref{zetasol} in terms of $\zeta_0$ and $P_0$, which does not directly provide the location at which the surface is anchored at the boundary.  To find this location - the entangling region corresponding to a given $\zeta_0,P_0$ - we can consider the inverse function, $\zeta_\infty(P_0)$, defined via $\zeta(P\to \infty)=\zeta_0\pm \zeta_\infty$, and given by
\begin{align}\label{}
\zeta_{\infty}(P_0)=\frac{P_0\left( (1+P_0^2)K\left( \frac{1+P_0^2}{1+2P_0^2} \right) - P_0^2 \Pi \left( \frac{1}{1+P_0^2},\frac{1+P_0^2}{1+2P_0^2} \right) \right)}{\sqrt{(1+P_0^2)(1+2P_0^2)}}
\end{align}

In figure \ref{figzetainfty} we plot the asymptotic value $\zeta_\infty$ as a function of $P_0$. One of the interesting observations of \cite{Krtous:2014pva} was that, for a given $\zeta_\infty<\zeta_\infty^{\text{max}}\approx 0.5$, there exist \textit{two} values of $P_0$ with the same $\zeta_\infty$. This implies that, for two discs that are sufficiently `close' on the sphere, there actually exist \textit{two} minimal surfaces that connect them. However, one of them (the branch which has smaller value of $P_0$ is always subdominant, and therefore will be of little interest in our analysis). On the other hand, if the `height' of the RT surface (in cylindrical coordinates) is larger than a critical value, there exist no connected minimal surface that joins them.

\begin{figure}[h]
\begin{center}
\includegraphics[scale=0.4]{images/zetainfty}
\caption{Plot of the `height' of the RT surface in cylindrical coordinates, as a function of the parameter $P_0$ characterising the surface. For $2\zeta_\infty\leq 2\zeta_\infty^{\text{max}}\approx 1$, there are two minimal surfaces anchored at the same regions; for $2\zeta_\infty> 2\zeta_\infty^{\text{max}}$ there exists no connected minimal surface joining them. }
\label{figzetainfty}
\end{center}
\end{figure}

Next we consider the areas. Although the area of the surfaces is divergent, one can compute the integral of the area element from $P_0$ to some $P>P_0$ along the surface\cite{Krtous:2014pva}. For the disconnected solution (phase I), the area of the pair of disks of radius $P$ is
\begin{align}\label{zetainfty}
\frac{1}{L^2}A_{\text {I}}(P)=2\times2\pi\left( \sqrt{1+P^2}-1 \right)
\end{align}

On the other hand, for the connected surfaces one can compute the area from $P_0$ to some $P>P_0$, yielding
\begin{align}\label{}
\frac{1}{L^2}A_{\text {II}}(P,P_0)&= 2\times\frac{2P_0^2}{\sqrt{1+2P_0^2}} \Pi\left( \mbox{Arccos}\frac{P_0}{P},1,\sqrt{\frac{1+P_0^2}{1+2P_0^2}} \right)
\end{align}
The factor of two is due to the fact that, in both the disconnected and connected cases, the surface is identical on both sides of the brane.

Of course, as usual in AdS/CFT, these areas possess a divergent contribution for large radius $P$. We define the renormalised area $\Delta A$ by subtracting the area of the disconnected solution:
\begin{align}\label{dAP01}
\Delta A(P_0)&=\lim_{P\to \infty}\left( A_{\text {II}}(P,P_0)-A_{\text {I}} (P)\right)
\end{align}
where we can safely take the limit, since the divergences match. The plot of $\Delta A$ is shown in figure \ref{figdeltaA}. Of course, the renormalised area is closely related to the mutual information. Mutual information between two subsystems $A$ and $B$ is defined via $I=S_{A\cup B}-S_A-S_B$. Notice that whenever $\Delta A>0$, phase $I$ dominates and therefore the mutual information vanishes, since $S_{A\cup B}=S_A+S_B$.

\begin{figure}[h]
\begin{center}
\includegraphics[scale=0.3]{images/dAP0}
\caption{Renormalised area from eq. \eqref{dAP01}. For $\Delta A>0$, the disconnected surface I has less area and dominates, while for $\Delta A<0$ the connected solution II is the global minimum.}
\label{figdeltaA}
\end{center}
\end{figure}


\subsubsection{Introducing a brane: R-T surfaces in AdS/BCFT}\label{AdS/BCFT}

With this choice, the equation for the brane \eqref{brane} becomes
\begin{align}\label{}
\sinh r\, \cos\theta=\left( 1+P^2 \right)\sinh^2\zeta=\sinh\left( \rho/L \right):=u^2=\cot\theta_\brane
\label{eq:foobar}
\end{align}
\vc{second expression (and probably third expression also) should be squarerooted.}
From here we see that the brane intersects the conformal boundary at the equator $\theta\to\pi/2,r\to\infty$ or equivalently $\zeta\to 0,P\to \infty$ in the cylindrical coordinates.

In the small $\Gbk$ expansion, the standard R-T formula states that the entanglement entropy of a subregion $\Sigma$ in the CFT is given by the area of a classical minimal surface that can probe the bulk but is anchored at $\partial \Sigma$ and remains homologous to $\Sigma$. The extension of this recipe to the case of boundary CFTs (BCFT) is a natural extrapolation of the dictionary\,\cite{Takayanagi:2011zk}: the bulk spacetime is instructed to `end' at a brane that lives in the bulk and asymptotes to the boundary of the CFT. This introduces a new physical effect in the system: the R-T surfaces are now allowed to end at the brane and thus a new set of `competing' surfaces enter the minimisation problem, which must also be taken into account. In cases where there are multiple local extrema, the EE is then given by the area of the global minimum.

As the first step towards understanding the physics of the formula \eqref{Sgenint}, in this subsection we consider the problem of the BCFT at the leading order in $1/\Gbk$. That is, we solve the problem of finding the R-T surfaces anchored at the CFT subregion that end on the brane, see figure \ref{figsetup}.
\begin{figure}[h]
\begin{center}
\includegraphics[scale=0.3]{images/setup}
\caption{A half of the geometric setup in cylindrical coordinates, with the radial direction compactified to a finite coordinate value. The `tube' (orange) represents the RT surface $\sigma$ in phase II, anchored at conformal infinity and intersecting the brane (green) at the codim-$3$ surface $\del\sigma_{brane}$ (red). The disk (blue) corresponds to the trivial phase I. We subtract their areas to obtain a finite result. }
\label{figsetup}
\end{center}
\end{figure}

The total renormalised area of phase II has now two contributions\footnote{Since we will focus on the regime of branes of large tensions, the second term term in eq. \eqref{A2tobrane} indeed comes with a positive sign. For small tensions, some minimal surfaces would intersect the brane before reaching the point where $P=P_0$, and therefore the second term would appear with a negative sign in front. }
\begin{align}\label{A2tobrane}
\Delta \tilde A(u,\zeta_{cft},P_0)=\Delta A[P_0]+A[P_b,P_0]\ \ ,\ \ P_b=P_b(u,\zeta_{cft},P_0)
\end{align}
The first term is simply the renormalised area term introduced in \eqref{dAP01}, which involves an integral from $P_0$ to $\infty$ in the lower half of the surface of figure \ref{figsetup}. In the second, we integrate from $P_0$ to $P_b$, defined as the intersection of the surface with the brane. We have emphasised that the radius of intersection $P_b$ depends on the location of the brane via $u$, together with the anchoring hight $\zeta_{cft}$ and the parameter $P_0$ of the given curve. To find the entanglement entropy of the disk in the BCFT, one must take the area \eqref{A2tobrane} and vary $P_0$ in order to find the minimum, for fixed $u$ and $\zeta_{cft}$.

We perform this computation numerically, since the special functions involved in the calculation are difficult to invert. Some sample curves are displayed in figure \ref{}, where we plot the area of the R-T surface for fixed anchoring point $\zeta_{cft}$ as we vary $P_0$, for different values of $u$, the parameter controlling the tension of the brane. In particular, we notice that the renormalised area is always positive for sufficiently large $u$. Therefore we find that, although a local minimum exists, the renormalised area up to the brane is always larger than that of the disk -  that is, the disconnected R-T solution always dominates. Thus, in the regime of large $u$, the disconnected phase always dominates. By itself, this phase would not be too interesting, since the presence of the brane would not play a significant role, and the mutual information between the two discs would simply vanish.
\begin{figure}[h]
\begin{center}
\includegraphics[scale=0.3]{images/ClassAreas}
\caption{ Renormalised area $\Delta\tilde A$ of connected R-T surfaces as a function of $P_0$, from the anchoring point on the CFT up to the intersection with the brane, for different values of $u$. }
\label{figClassAreas}
\end{center}
\end{figure}

However, the story has a twist: as discussed recently in the context of black hole evaporation models and also discussed above, the RT formula to compute entanglement entropies must be corrected if the quantum system of interest is entangled with another system where gravity is dynamical. This is precisely the case at hand, since the CFT is entangled with degrees of freedom on the RS brane, where we have an Einstein-Hilbert gravity action.


\subsubsection{The generalised entropy on the brane}\label{sec:generalised}

Let us define the dimensionless `generalised area' functional as
\begin{align}\label{Agen}
\mathcal{A}_{gen}(\sigma)=\frac{A(\sigma)}{4\Gbk}+\frac{A(\partial\sigma_{brane})}{4\Gbr}
\end{align}
Then, the generalised entropy is defined as the minimum (or extremum for the covariant case) of the generalised area under variations of the surface $\sigma$:
\begin{align}\label{}
S_{gen}=\min_{\sigma} \mathcal{A}_{gen}(\sigma)
\end{align}
Notice that each $\sigma$ determines its own $\partial\sigma_{brane}$, which is not an independent variable.

As before, we are interested in the renormalised area of the connected surface, where we subtract the disconnected contribution. Notice that this affects only the bulk area term, and not the second term of \eqref{Agen}. Now let us specify to the concrete case of our geometric setup. We must consider
\begin{align}\label{dAgen}
\Delta \mathcal{A}_{gen}&=\frac{\Delta \tilde A(\sigma)}{4\Gbk}+\frac{A_{\text{II}}(\partial\sigma_{brane})}{4\Gbr}
\end{align}

The first term, $\Delta \tilde A=A_{\text{II}}(\sigma)-A_{\text{I}}(\sigma)$, is simply the renormalised area up to the brane, already considered in section \ref{AdS/BCFT}. The new term, $A_{\text{I}}(\partial\sigma_{brane})$, the area of the intersection between $\sigma$ and the brane. In this case, due to the axial symmetry around $P=0$, this consists of a circle of radius $P_b$, which according to the metric \eqref{H3cyl} has an area (perimeter) of
\begin{align}\label{ring}
A_{\text{II}}(\partial\sigma_{brane})=2\pi L P_b
\end{align}

It will prove convenient to work with the dimensionless ratio
\begin{align}\label{lambdaratio}
\lambda:=\frac{\Gbk}{2L\Gbr}
\end{align}
which controls the relative strength between the bulk and brane Newton constants, and therefore the effect of the extra term in the generalised entropy.

We explore the generalised area and their associated entropies numerically. In figure \ref{figA_gen} we plot the renormalised generalised area of eq. \eqref{dAgen} as function of $P_0$, for different values of the anchoring point $\zeta_{cft}$, brane tension $u$ and the ratio $\lambda$.  Finally, the renormalised generalised entropy is the minimum over all allowed $P_0$:
\begin{align}\label{}
\Delta S_{gen}=\min_{P_0} \Delta \mathcal{A}_{gen}
\end{align}

Let us recall what parameters are in play. The tension of the brane is controlled by $u$, which we keep large but finite. The dimensionless ratio between the bulk and brane gravitational constants is controlled by $\lambda$. In this regime, the interesting physics arises when $\lambda<0$, which in this context is obtained by allowing $\Gbr<0$ while $\Gbk>0$.  As discussed above, a negative gravitational constant on the brane can be naturally obtained via quantum corrections. Moreover, the parameter $P_0$ is not free, but must be varied in order to find the minimum of the total area functional. For a given $\zeta_{cft}$, only those R-T surfaces with $P_0$ such that they actually intersect the brane are allowed to `compete' in the minimisation problem.
\begin{figure}[h]
\begin{center}
\includegraphics[scale=0.3]{images/A_gen}
\caption{Generalised area for different values of $-1<\lambda<0$, as function of $P_0$. For each curve, the generalised entropy is given by the global minimum. The critical value for which the minimum lies below the axis signals the transition when phase II dominates.}
\label{figA_gen}
\end{center}
\end{figure}

Figure \ref{figA_gen} contains information about the phase diagram of our system. First, we see the existence of a first order phase transition between two different R-T surfaces that end on the brane. Notice that this non-trivial structure is induced by the second term in the generalised entropy. Indeed, when $\lambda=0$, one obtains the results of figure \ref{figClassAreas}, where there is a single global and local minimum, for each value of the brane tension.

\iar{Figure: plot $\lambda_c$ vs $u$}



%\newpage

%\subsubsection{Higher dimensions}

%\paragraph{Mutual information of two discs}

\paragraph{Entanglement Wedge cross sections}

$P_0$ is defined as the point where $\zeta'$ diverges, we need some characterisation in terms of CFT data, the same for mutual info


==> sections/HEE1__Joshua_Sandor_s_conflicted_copy_2020-03-12_.tex <==
% !TEX root = ../lifeonbrane3.tex

In this section, we shall look for `quantum extremal islands' using the holographic setup described in the previous sections. Of course, quantum extremal islands have recently proven especially enlightening in the context of the black hole information paradox in two-dimensional JT gravity, where the emergence of these islands has signalled a transition to a phase where entropy of the Hawking radiation decreases over time, \eg \cite{Almheiri:2019psf, Almheiri:2019hni, Almheiri:2019yqk, Chen:2019uhq, Penington:2019kki, Almheiri:2019qdq, Chen:2019iro}. Some preliminary investigations of quantum extremal islands in higher dimensions also appear in \cite{Penington:2019npb,Almheiri:2019psy}. In a companion paper \cite{QEI}, we will use the holographic model developed here to further extend these discussions to consider the black holes in arbitrary dimensions. However, our present discussion departs somewhat from this line of investigation because black holes are not involved. Rather, we are simply considering the holographic entanglement entropies for certain regions in the vacuum of the boundary CFT coupled to the conformal defect. In certain situations, we find that the corresponding RT surfaces cross the brane in the bulk and this can be interpreted in terms of the appearance of a quantum extremal island in the effective theory of gravity on the brane.

To expand on this last comment, let us consider a specific calculation of the entanglement entropy (EE): We consider the vacuum state of our boundary CFT on $\Rbb(\text{time})\times S^{d-1}(\text{space})$ with a conformal defect running along the equator of the $S^{d-1}$. As described in section \ref{sec:branegravity}, the bulk spacetime has locally an AdS$_{d+1}$ geometry and is bisected by a brane extending out to the defect position on the asymptotic boundary. Now we wish to evaluate the EE in the boundary CFT for a region $\xR$ comprised of the union of two polar spherical caps on the $S^{d-1}$ -- see figure \ref{EEprob}.
%
%\begin{figure}[h]
% \def\svgwidth{0.6\linewidth}
% \centering{
% % \input{xyz.pdf}
%  \caption{\rcm{New figure illustrating EE problem in the boundary CFT.}}
% \label{EEprob}}
%\end{figure}
\begin{figure}
	\def\svgwidth{0.8\linewidth}
	\centering{
		\input{sec4.pdf_tex}
		\caption{Caption... } \label{fig:sec4}
	}
\end{figure}
We follow the usual holographic prescription to compute the EE. That is, we examine the bulk surfaces $\xV$ which are homologous to  $\xR$ and extremize the generalized entropy functional
\beq
 S_\EE(\xR) = {\rm min}\left\{\extr\,
 S_\gen(\xV)\right\}={\rm min}\left\{\extr
  \(
  \frac{A(\xV)}{4 G_\bulk} + \frac{A(\xV \cap {\rm brane})}{4 G_\brane}\)\right\}\,.
 \label{eq:sad}
\eeq
Of course, the first term above corresponds to the usual Ryu-Takayanagi (RT)  term \cite{Ryu:2006bv,Ryu:2006ef} while  we argue in Appendix \ref{generalE}, that the second term will arise whenever the bulk surface crosses a DGP brane.\footnote{Implicitly, eq.~\eqref{eq:sad} assumes that the bulk and brane gravitational actions both correspond to the Einstein-Hilbert action (with a cosmological constant term), as in eqs.~\reef{act2} and \reef{newbran}.} Let us denote the extremal bulk surface as $\Sigma_\xR$, and the intersection with the brane $\sigma_\xR=\Sigma_\xR \cap {\rm brane}$. Importantly, if there are multiple extrema, the EE is given by chosing the extremal surface yielding the smallest value for $S_\gen(\Sigma_\xR)$, as indicated above.

For the calculation described above, the candidate RT surfaces are anchored at the AdS boundary to the entangling surface $\SCFT=\partial \xR = \partial \RTsurf$, \ie the boundaries of these surfaces are comprised of two $(d-2)$-spheres, which are the boundaries of the two polar caps. We will find that there are two topologically distinct candidates for $\RTsurf$ which extremize the generalized entropy in eq.~\reef{eq:sad}. The first consists of two disconnected disks on either side of the brane (in which case $\sigma_\xR=\{\varnothing\}$). The second candidate has a cylindrical geometry which pierces the brane. Hence it is only in this latter case that the second term contributes in eq.~\reef{eq:sad}. As noted above, the correct RT surface is chosen from these two candidates as the one which yields a smaller generalized entropy. Generally, we shall find that when the two polar caps are small, the disconnected discs are favoured, while the cylindrical surface can be the leading saddle for large polar caps are large. We will denote the first situation as the `disconnected' phase and the latter as the `connected' phase. As we will describe in section \ref{sec:examples}, the details of the transition between these two phases also depends on other parameters in the holographic model, \eg the tension and gravitational coupling of the brane.

To understand the interpretation of these results in terms of quantum extremal islands, we turn to the `brane perspective' described in the previous section. In this effective description, the entanglement entropy is given the `island rule' proposed in \cite{Almheiri:2019hni},
\beqa
 S_\EE(\xR) &=& {\rm min}\left\{\extr\,
 S_\gen(R\cup \text{islands} )\right\} \labell{rule1}\\
&=&{\rm min}\left\{\extr
  \(  S_\EE(\braneR \cup \text{islands}) + \frac{A\(\partial(\islands)\)}{4 G_\brane}\)\right\}\,.
 \nonumber
\eeqa
As geometries $\CFTR=\braneR$, but we have used a different font on the right-hand side to emphasize the fact that from the effective `boundary perspective' does not give the same detailed description of the CFT state on $\CFTR$, as the boundary or bulk perspectives.

Now it is straightforward to interprete the previous holographic discussion in terms of eq.~\reef{rule1}. In particular, in the disconnected phase, the EE only involves the modes enclosed within the two polar caps and there is no contribution from the CFT in the gravitational region, \ie on the AdS$_d$ brane. In passing, let us recall that the short wavelength modes in the vicinity of the entangling surface $\SCFT$ produce various UV divergent boundary contributions, such as the celebrated area law term \cite{Sorkin_1983,Bombelli:1986rw,Srednicki:1993im}. Of course, these contributions are regulated in the holographic calculation by introducing a cutoff surface near the asymptotic AdS boundary \cite{Rangamani:2016dms}.

However, in the connected phase, the holographic RT surface crosses the brane and we see an explicit brane contribution in eq.~\reef{eq:sad} (evaluated on $\sigma_\xR$). From the brane perspective, a quantum extremal island has formed in the gravitational region (\ie the region on the brane enclosed by $\sigma_\xR$)\footnote{Let us add that from the bulk perspective, entanglement wedge reconstruction \cite{EW1,EW2,EW3,Jafferis:2015del,Dong:2016eik,Faulkner:2017vdd,Cotler:2017erl} ensures that operators within this island can be reconstructed from boundary CFT data in $\xR$.} and the analogous gravitational term appears in the island rule \reef{rule1}. The bulk RT contribution in eq.~\reef{eq:sad} then corresponds to $S_\EE(\braneR \cup \text{islands})$ in eq.~\reef{rule1} -- just as it did in the disconnected phase. Comparing to the gravitational action \reef{act3} on the brane, one might expect that the gravitational term in eq.~\reef{rule1} would involve $1/G_\eff$ rather than $1/G_\brane$. However, from eq.~\reef{Newton33}, \rcm{and explained in previous section??} we can see that $1/G_\eff$ is comprised of two components: the bare contribution $1/G_\brane$, and the bulk contribution proportional to $L/G_\bulk$. From the brane perspective, we can regard the latter as being induced by integrating out the CFT degrees of freedom on the brane. We might further split the CFT entropy into UV-finite and UV-`divergent' contributions, where the latter are contributions proportional to inverse powers of $\s$. These are the analog of the UV divergent boundary contributions discussed above for the boundary CFT in the regions without gravity. As discussed in section \ref{face}, the brane position imposes  a UV cutoff for the CFT on the brane, and hence the corresponding `divergent' contributions to the EE are in fact finite and instead yield contributions which match those expected for the gravitational entropy from the induced contributions to eq.~\reef{act3}. This makes contact with the usual notion of generalized entropy as the sum of the geometric gravitational entropy and the entropy of the quantum fields \cite{Faulkner:2013ana,Engelhardt:2014gca}. We elaborate on this perspective in more detail in section \ref{sec:genera}. In section \ref{sec:enzyme}, we also discuss how varying the position of the $\sigma_\xR$ can be interpreted as finding the quantum extremal surface from the brane perspective.



%\rcm{****} The remainder of this section is organized as follows: In section \ref{sec:enzyme}, we introduce the bulk metrics and other technical details required for the holographic calculation of entanglement entropy. In section \ref{sec:genera}, we interpret the HRT calculation of entanglement entropy from the brane perspective. Finally, in section \ref{sec:examples}, we explicitly carry out the extremization of generalized entropy and evaluating the generalized entropy in the disconnected no-island and connected island phases. $d=3$

% \vc{OLD STUF BELOW --- OLD STUFF BELOW --- OLD STUFF BELOW}
% In this section we relate the brane setup to the calculation of entanglement entropies for regions on the boundary CFT whose RT surface falls deep into the bulk and connects to the brane.
%
% \rcm{words:} Following Faulkner et al. \cite{Faulkner:2013ana}, we expect \iar{But we are going to prove this later?} \rcm{Refer to appendix \ref{generalE} as supporting evidence for the brane term. Use appendix notation for surface names; drop the factor of 2 below.}
% \beq\label{gen}
% \sgen = \text{ext}\Big(\frac{A(\Sigma_\mt{b})}{4 \Gbk}+ \frac{A(\sigma_\mt{b})}{4 \Gbr}\Big)\,,
% \eeq
% where $\sigma_b$ is the area of the intersection of the surface $\Sigma_b$ and the brane. The factor of two in the bulk area term accounts for our two bulks that are glued together along the brane.
%
%
% In AdS/CFT, branes such as the ones describes above play an essential role in the description of Boundary CFT (BCFT). If the CFT itself is living on a manifold with a boundary, the holographic prescription states that the dual geometry consists also of a manifold with a boundary - an AdS-like spacetime that ends on a brane, which is itself anchored at the boundary of the CFT (an `end-of-the-world brane') \cite{ads/bcft}.
%
% In general, the holographic recipe shows that the entanglement entropy of a subregion $A$ of the field theory is given by an extremal surface $\sigma$ that is anchored at the asymptotic boundary at $A$, that extends into the bulk and remains homologous to $A$. In the case of a BCFT, the new ingredient is that the R-T surface $\sigma$ is also allowed to end up at the brane. This introduces a new set of interesting `candidate' surfaces that compete in the minimization process.
%
% Recently, a new formula for the computation of holographic entanglement entropy was proposed, relevant for situations when the quantum system of interest is in contact with another system that contains gravity as a dynamical field. We will investigate this formula using the same bulk setup as described in previous sections. \iar{explain some more}
%
% \vc{OLD STUF ABOVE --- OLD STUFF ABOVE --- OLD STUFF ABOVE}

\subsection{RT meets the Brane}
\label{sec:enzyme}
%
In this section, we shall introduce some technical details, which are useful to calculate the EE associated with the two polar caps in the boundary CFT. In particular, we examine the behaviour of the bulk RT surface $\Sigma_\xR$ as it crosses the brane, \ie how the intersection surface $\sigma_\xR$ is determined.
However, we begin by specifying our EE calculation more precisely and reviewing the metrics describing the bulk spacetime.

Let us describe the $\Rbb\times S^{d-1}$ geometry on which the boundary CFT lives with,
\beq\label{metricCFT}
ds^2=R^2\left[-dt^2+
d\theta^2+\sin^2\!\theta\,d\Omega_{d-2}^2 \right]\,,
\eeq
where $R$ is the radius of curvature of the $(d-1)$-sphere. The polar angle $\theta$ runs over $0\le\theta\le\pi$, and the conformal defect sits at the equator $\theta=\pi/2$. As illustrated in figure \ref{EEprob}, we wish to evaluate the EE in the boundary CFT for a region $\xR$ comprised of two polar caps on the $S^{d-1}$. More specifically, we choose the entangling surface $\SCFT$ to be two circles placed  symmetrically on either side of the defect at $\theta=\pi/2\pm\thb$. Hence we are evaluating the EE between these two balls and the complementary region, which corresponds to a `belt' of width $2\thb$ centered on the conformal defect.

Turning now to the bulk geometry, recall that in section \ref{BranGeo}, we discussed the background solution in terms a metric where the AdS$_{d+1}$ geometry was foliated by AdS$_d$ slices. Eq.~\reef{metric3} describes the local geometry on either side of the brane
located at $z=\s$ with
\beq\label{metric3a}
ds^2=\frac{L^2}{z^2}\left[dz^2 +  L^2\left(1 + \frac{z^2}{4\,L^2}\right)^2 \left(-\cosh^2\!\tdr\,dt^2+d\tdr^2+\sinh^2\!\tdr\,d\Omega_{d-2}^2 \right)\right]\,.
\eeq
While these coordinates are well suited to discuss the brane geometry, we also consider `global' coordinates for the AdS$_{d+1}$ geometry
\beq\label{metric2s}
ds^2=L^2\left[-\cosh^2\!r\,dt^2+dr^2+\sinh^2\!r\,\left(
d\theta^2+\sin^2\!\theta\,d\Omega_{d-2}^2\right) \right]\,,
\eeq
which are better adapted to discuss the boundary theory. That is, up to a Weyl rescaling, the geometry on fixed $r$ surfaces matches eq.~\reef{metricCFT}  in the asymptotic region, and the UV regulator surface needed to properly define the holographic EE can be simply chosen as some slice $r=r_\mt{UV}\gg L$.

However, while we refer to eq.~\reef{metric2s} as `global' coordinates, they do not cover the entire back-reacted bulk solution depicted in figure \ref{fig:brane2}. Rather we use the coordinates in eq.~\reef{metric2s} to cover two patches on either side of the brane and near the asymptotic AdS$_{d+1}$ boundary.\footnote{Of course, the same applies for the previous coordinates in eq.~\reef{metric3a}.} Comparing eqs.~\reef{metric3a} and \reef{metric2s}, it is straightforward to identify the transformation between the two coordinate systems as
\beq\label{transfor1}
\tanh\tdr=\tanh r\sin\theta\,,\quad \frac{z}L=-2\sinh r\,\cos\theta\pm2\sqrt{\sinh^2\! r\,\cos^2\!\theta+1}\,.
\eeq
With the + (--) sign, the brane at $z=z_\mt{B}\ll L$ resides near the boundary hemisphere with $0\le\theta\le\pi/2$ ($\pi/2\le\theta\le\pi$) and $r\to\infty$. Therefore letting $\theta$ run from 0 to $\pi$ on the boundary with the defect at $\theta=\pi/2$, we choose the -- (+) sign to cover the patch covering the asymptotic boundary hemisphere $0\le\theta\le\pi/2$ ($\pi/2\le\theta\le\pi$).

Recall that using the AdS foliation \reef{metric3a}, the position of the brane was specified by $z=\s$. In terms of the global coordinates \reef{metric2s} , the brane position can be specified with
\beq\label{eq:foobar}
\sinh^2\! r\, \cos^2\!\theta= \frac{L^2}{\s^2}\(1-\frac{\s^2}{4L^2}\)^2\,.
\eeq
Note that the specific sign of $\cos\theta$ depends on whether one considers the coordinate patch above or below the brane -- see comments below eq.~\reef{transfor1}. Further, we reach the asymptotic boundary on the brane by taking $\tdr\to\infty$, which in the global coordinates then corresponds to $r\to\infty$ and $\theta\to\pi/2$. Hence, we see that the brane intersects the asymptotic boundary at the position of the conformal defect, as expected.

To examine the behaviour of the bulk RT surface $\Sigma_\xR$ where it crosses the brane, it is useful  to consider the problem of extremal surfaces using eq.~\reef{metric3a}. Of course, because the bulk geometry is static, the RT surfaces will be confined to a constant time slice in the bulk. Further, the entangling surfaces in the boundary are spherically symmetric and so we only need to consider bulk surfaces with the same rotational symmetry on the $S^{d-2}$. That is, we parametrize the surfaces as $\tdr=\tdr(z)$ and the bulk contribution to the holographic EE is then given by
\beq\label{area0}
S_\mt{bulk}= 2\,\frac{L^{d-1}\, \Omega_{d-2}}{4\,\Gbk} \int \frac{dz}z \,\[\frac{L}{z}\left(1 + \frac{z^2}{4\,L^2}\right)\sinh\tdr\]^{d-2} \sqrt{1+L^2\left(1 + \frac{z^2}{4\,L^2}\right)^2\(\frac{d\tdr}{dz}\)^2}
\eeq
where $\Omega_{d-2}$ is the area of a unit $(d-2)$-sphere.\footnote{Recall that the area of a unit $n$-sphere is given by $\Omega_{n} = 2\pi^{\frac{n+1}2}/\Gamma\(\frac{n+1}2\)$. \label{footsphere}} An overall factor of 2 is included here because we assume that the profile $\tdr(z)$ will be reflection symmetric about the brane, and hence $S_\mt{RT}$ recieves the same contribution from both sides.

Now treating eq.~\reef{area0} as an action, we would derive an `Euler-Lagrange' equation for the profile whose solution corresponds to an extremal surface in the bulk, \ie away from the brane.\footnote{This equation is rather involved and the details are not important here.} However, this equation is second order and so the solutions are parameterized by two integration constants. One of these constants is fixed by the angle $\theta_\mt{CFT}$ on the asymptotic boundary (\ie the position of the entangling surface $\SCFT$ in the boundary theory), and the other, by the radius $\tdr_\mt{B}$ at which the RT surface intersects the brane, \ie $\tdr(z=\s)=\tdr_\mt{B}$. Hence we are left with the question of fixing the boundary condition at the brane.

In fact, there are two contributions that come into play at the brane. The first is the DGP contribution in eq.~\reef{eq:sad},
\beq\label{area1}
S_\mt{brane}= \frac{L^{d-2}\, \Omega_{d-2}}{4\,\Gbr} \,\[\frac{L}{\s}\left(1 + \frac{\s^2}{4\,L^2}\right)\sinh\tdr_\mt{B}\]^{d-2} \,.
\eeq
The second is a boundary term that comes from integrating by parts in the variation of the RT functional \reef{area0}. Combining these, one arrives at the following expression\footnote{Implicitly, we assume that we care considering the RT surfaces with a cylindrical topology, \ie in the connected phase. Examining these boundary terms carefully, one also finds that they are eliminated with $\tdr_\mt{B}=0$. This solution points towards the existence of the second phase of disconnected surfaces, which do not intersect the brane.}
\beq\label{ortho1}
L\,\frac{d\tdr}{dz}\bigg|_{z=\s}=\frac1{\Gbr}\,
\frac{\s/L}{1 + \frac{\s^2}{4\,L^2}}\[
\left(1 + \frac{\s^2}{4\,L^2}\right)^2\(\frac{2L}{\Gbk}\,\tanh\tdr_\mt{B}\)^2-\(\frac{\s/L}{\Gbr} \)^2\]^{-\frac12}\,.
\eeq
Hence scanning through the family of RT surfaces parametrized by $\tdr_\mt{B}$, the solution which satisfies the above boundary condition is the one that properly extremizes the full entropy functional in eq.~\reef{eq:sad}. \rcm{Add a picture to illustrate this discussion?? Could this be combined with a picture for the geometric discussion below??} One observation is that without the DGP term, \ie $1/\Gbr=0$, the boundary condition simplifies to $L\,{d\tdr}/{dz}|_{z=\s}=0$. That is, the RT surface intersects the brane at a right angle. Turning on the gravitational action on the brane (with a positive coupling) produces $L\,{d\tdr}/{dz}|_{z=\s}>0$, which arises from pushing $\tdr_\mt{B}$ to a smaller value. The decrease in $\tdr_\mt{B}$ is natural here because the DGP contribution in eq.~\reef{area1} adds an additional penalty for large areas on the brane and hence the effect is to shrink the area of $\sigma_\xR$.\footnote{Of course, if $1/\Gbr<0$ as we consider in section \ref{sec:examples}, then the DGP entropy \reef{area1} facilitates a larger area for $\sigma_\xR$ and so we find that $\tdr_\mt{B}$ increases.}

We observe that the above analysis has a simple interpretation in terms of the island rule \reef{rule1}. Recall that extremizing the RT functional \reef{area0} leads to a family of bulk solutions that are parametrized by $\tdr_\mt{B}$, their radius on the brane. Evaluating $S_\mt{bulk}+S_\mt{brane}$ for these different solutions is equivalent to evaluating the $S_\gen$ in eq.~\reef{rule1} with different candidates for the island geometry. The final step of extremizing with respect variations of $\tdr_\mt{B}$ then matches the extremization in the island rule and identifies the quantum extremal surface $\sigma_\xR$ on the brane.



To close the discussion here, we provide a more general geometric discussion of the boundary conditions.
The orthogonality between the RT suface and the RS brane is a special feature of the reflection symmetry of our setup. For a better geometric understanding of the boundary conditions, let us examine eq.~\reef{eq:sad} in more detail. Consider a $(d-1)$-dimensional surface $\xV$ parametrized by intrinsic coordinates $\xi^\alpha$, embedded in the $(d+1)$-dimensional bulk spacetime with coordinates $X^\mu$ and metric $g_{\mu\nu}$. Hence we describe the embedding of this surface in the bulk spacetime as $X^\mu = X^\mu(\xi^\alpha)$, and the induced metric then becomes
\beq
h_{\alpha\beta}= g_{\mu\nu}\,
  \frac{\partial X^\mu}{\partial \xi^\alpha}\,
  \frac{\partial X^\nu}{\partial \xi^\beta}\,.
\label{badnote}
\eeq
Hence the bulk contribution in eq.~\reef{eq:sad} becomes
\beq
  S_\mt{bulk}=\frac{A(\xV)}{4 G_\bulk}
  = \frac{1}{4G_\bulk}\int_\xV d^{d-1}\xi\; \sqrt{h}\,.
\label{eq:badNotation}
\eeq
Next to evaluate the brane contribution in eq.~\reef{eq:sad}, we introduce $(d-2)$ coordinates $y^a$ to parameterize the intersection of $\xV$ and the brane. The induced metric on this intersection surface then becomes
\beq\label{badnote2}
  \tilh_{ab}
  = h_{\alpha\beta}
  \frac{\partial \xi^\alpha}{\partial y^a}
  \frac{\partial \xi^\beta}{\partial y^b}\,,
\eeq
and the corresponding contribution to the generalized entropy is
\begin{align}
  S_\brane
  =& \frac{1}{4\Gbr}\int d^{d-2}y\; \sqrt{\tilh}\,.
  \label{eq:facundo}
\end{align}

Now following the prescription in eq.~\reef{eq:sad}, we wish to  extremize the sum of the two quantities above. So we begin with the variation of $S_\mt{bulk}$, which yields
\beq
\begin{split}
  \delta S_\mt{bulk}
  =& \frac{1}{4G_\bulk}\Bigg[ \int_{\xV\cap{\rm brane}}\!\!\!\!\!\!\!\! d^{d-2} y\,
  \sqrt{\tilh}\, g_{\mu\nu}\, (\partial_{n_\mt{R}} X^\mu+\partial_{n_\mt{L}}X^\mu) \,\delta X^\nu
  \\
  &+\int_\xV d^{d-1}\xi \sqrt{h}(\text{e.o.m.})_\nu \delta X^\nu
  \Bigg]\,.
\end{split}
  \label{eq:recipe}
\eeq
Here we assume that the equations of motion along the bulk of $\xV$ can be satisfied and so the second term above vanishes. However, one must integrate by parts to arrive at these equations and so we are left with a boundary term where $\xV$ crosses the brane.\footnote{Dirichlet boundary conditions remove the analogous boundary contributions at the asymptotic AdS boundary.} Here we are assuming that the extremal surface is not necessarily smooth at the brane and so $n_\mt{R}^\alpha$ and $n_\mt{L}^\alpha$ are unit normals to the intersection surface directed along the extremal surface approaching the brane from either side -- see figure \rcm{new fig}.

In fact, in the absence of the DGP term \reef{newbran}, there is no brane contribution \reef{eq:facundo} and then the vanishing of the boundary term in eq.~\reef{eq:recipe} dictates $n_\mt{R}^\alpha+n_\mt{L}^\alpha=0$. That is, with $1/\Gbr=0$, the boundary condition is that the RT surface should pass smoothly through the brane. In the reflection symmetric setup considered above, this can only be accomplished if the RT surface is orthogonal to the brane, \ie both $n_\mt{R}^\alpha$ and $n_\mt{L}^\alpha$ are orthogonal to the brane.

Of course, with a DGP brane, we must also consider the variation of $S_\brane$ in eq.~\reef{eq:facundo}, which yields
\begin{align}
  \delta S_\brane
  =& \frac{1}{4\Gbr}
  \int d^{d-2}y\; \sqrt{\tilh}\,
  \inducedK_i \,\frac{\partial x^i}{\partial X^\nu}\, \delta X^\nu,
  \label{eq:puerto}
\end{align}
where $\inducedK_i$ denotes the trace of the extrinsic curvatures of the intersection surface and the brane, as viewed from the brane geometry with $(d-1)$ coordinates $x^i$. (In deriving \eqref{eq:puerto}, we have interpretted $\inducedK_i$ as the expansion\footnote{Note that $\inducedK_i$ gives the expansion of the area element under the map produced by geodesics shot out normal to $\RT\cap\brane$. However, the images of $\RT\cap\brane$ under $\delta X^\nu$ and under the map obtained by projecting $\delta X^\nu$ perpendicular to $\RT\cap\brane$ differs only at second order in $\delta X^\nu$ (assuming $\delta X^\nu$ is smooth). \vc{I drew a picture to convince myself... does this seem right? (Even if it's not right, I think it suffices to restrict $\delta X^\nu|_{\RT\cap\brane}$ to be orthogonal to the intersection.)}} of the area element $\sqrt{\tilh}$.)
Requiring the sum of eqs.~\eqref{eq:recipe} and \eqref{eq:puerto} to vanish then yields the boundary condition
\beq\label{ortho7}
 0  =  g_{\mu\nu} (\partial_{n_\mt{R}} X^\mu+\partial_{n_\mt{L}}X^\mu)
  + \frac{G_\bulk}{G_\brane}\,\inducedK_i \,\partial_\nu x^i\,.
\eeq
\rcm{Am I missing a projection onto the brane or something here?}\vc{Yes, it's the components (index $\nu$) of \eqref{ortho7} along the brane that need to vanish. This is because there is a a contraction with $\delta X^\nu$ in \eqref{eq:recipe} and \eqref{eq:puerto}. Note that $\delta X^\nu$ cannot be chosen arbitrarily. Rather, $\delta X^\nu$ is restricted to be parallel to the brane. (In writing \eqref{eq:recipe}, we have assumed that the same domain of the parametrization coordinates $\xi^a$ maps to the portion of the RT surface on a given side of the brane under both $X^\mu(y^a)$ and $X^\mu(y^a)+\delta X^\mu(y^a)$. Said another way, $S_\bulk$ has the same integration limits in $y^a$ both before and after the variation.) Note that, in the special case $1/G_\brane=0$, the fact the components of $n_\mt{R},-n_\mt{L}$ along the brane are the same implies that $n_\mt{R}=-n_\mt{L}$, since normalization determines the components of $n_\mt{R},n_\mt{L}$ along the only other possible direction they can point. Similarly, when $1/G_\brane\ne 0$, given $n_\mt{R}$, \eqref{ortho7} (projected along the brane directions) contains enough information, together with normalization, to determine $n_\mt{L}$ --- take the components of $n_\mt{R}$ along the brane, add $(G_\bulk/G_\brane)\curvK$ to them, and that gives the components of $-n_\mt{L}$ along the brane; again the remaining degree of freedom in $-n_\mt{L}$ is determined by normalization.}
Hence the brane contribution \reef{eq:facundo} leads to a discontinuity in the first derivative of the RT surface at the brane, as was implicitly found in eq.~\reef{ortho1} above.

\rcm{****} We note that, in the absence of DGP gravity $1/G_\brane=0$, we obtain the orthogonality condition: the tangent $\partial_n X^\mu$ of the RT surface orthogonal to its intersection of the brane, must be orthogonal to the brane. When the brane bisects rather than end the bulk spacetime (\eg for a brane emanating from a defect separating two parts of a CFT), the RT surface approaches the brane from both sides, giving two terms from the boundary contribution in \eqref{eq:maestro}:
\begin{align}
  0
  =& \left.
  \left[
  \frac{g_{\mu\nu} (\partial_n + \partial_{n'})X^\mu}{4 G_\bulk}
  + \frac{\inducedK_i \partial_\nu x^i}{4G_\brane}
  \right] \delta X^\nu
  \right|_{\RT\cap\brane}
  & &(\text{defect brane})
  \\
  =& \left.
  \left[
  \frac{g_{\mu\nu} \partial_n X^\mu}{2 G_\bulk}
  + \frac{\inducedK_i \partial_\nu x^i}{4G_\brane}
  \right] \delta X^\nu
  \right|_{\RT\cap\brane}.
  & &(\text{$\Zbb_2$-symmetry})
  \label{eq:caprice}
\end{align}
Here, $n^\alpha$ and $(n')^\alpha$ are unit normals to the intersection of the RT surface with the brane, as the RT surface approaches the brane from either side. In general, $\partial_n X^\mu|_{\RT\cap\brane}$ and $\partial_{n'}X^\mu|_{\RT\cap\brane}$ need not be individually orthogonal to the brane, even in the absence of DGP gravity. However, in the presence of $\Zbb_2$ symmetry, the extremization problem can be treated as two copies of a corresponding end of the world brane problem (with half the ratio between DGP and bulk gravity). In particular, $g_{\mu\nu}(\partial_n+\partial_{n'})X^\mu \delta X^\nu|_{\RT\cap\brane}=2 g_{\mu\nu} \partial_n X^\mu \delta X^\nu|_{\RT\cap\brane}$, and we obtain \eqref{eq:caprice}. Again, the orthogonality condition is recovered when $1/G_\brane=0$.


\subsection{RT on the Brane}\label{sec:genera}

As alluded to above, one of striking features of EE for subregions in quantum field theory is that the result is dominated by short wavelength modes in the vicinity of the entangling surface and the EE is UV divergent. Of course, the leading contribution is the famous area law term \cite{Sorkin_1983,Bombelli:1986rw,Srednicki:1993im} and in higher dimensions, there are subleading UV divergences which also determined by the geometry of the entangling surface (as well as the dimensionful couplings of the underlying theory). In the holographic context, these divergences arise because the RT surface in the bulk extends out to the asymptotic boundary and hence the unregulated area is infinite \cite{Ryu:2006bv,Ryu:2006ef,Rangamani:2016dms}. In the context of braneworld gravity, like the construction in the previous section with $\s\ll L$, one expects large UV contributions when the RT surface crosses the brane. However, in this instance, the corresponding UV cutoff remains finite and set by the position of the brane, as discussed at the end of section \ref{indyaction}. We show below that the corresponding UV contributions to the holographic EE can be interpreted as the Wald-Dong entropy \cite{Wald:1993nt,Iyer:1994ys,Jacobson:1993vj,Dong:2013qoa}\footnote{Our calculations will include the subleading contributions arising from the curvature-squared terms in eq.~\reef{act3}. Because the corresponding quantum extremal surfaces have nonvanishing extrinsic curvature, we will need the full expression for the gravitational entropy derived by Dong \cite{Dong:2013qoa}.} of the induced gravity on the brane \cite{Emparan:2006ni,Myers:2013lva}. Of course, the leading UV contributions studied here do not probe the full bulk profile of the RT surface, and we leave the full calculation of holographic EE to Section \ref{sec:examples}.

\rcm{*******}

% In this subsection, we wish to study the leading order contributions to holography entanglement entropies for our brane setup in arbitrary dimension. We begin by identifying such contributions coming from the bulk area of the RT surface. Then, we shall show that these contributions match the Wald-Dong entropy of the induced $d$-dimensional gravity action of the brane.


% \subsubsection{Leading bulk RT surface contributions \label{bulkrt}}
\rcm{CAREFUL: is this calculation affected if we have a DGP term and RT surface is not orthogonal to brane??} \vc{I think it's fine now.}
%
\vc{write out Dong-Wald entropy for action \reef{act3} (no derivation!; just refer to refs); show the two contributions found above match this result}


% As before, the bulk consists of two copies of a patch of global AdS$_{d+1}$, glued together along that surface, which creates a spacetime with a tensionfull brane located at that surface. The asymptotic boundary now consists of two copies of a hemisphere cross time, $S^{d-1}\times \mathbb R_t$, glued along a defect. As our entangling region, we choose two identical discs, centered at the pole of each hemisphere, see figure \ref{fig:rtsurface}, which depicts half of the geometry. In this setting, the R-T surface $\RTsurf$ has two different `phases'. The disconnected or `trivial' phase consists of two independent surfaces with the topology of a disc. On the other hand, in the connected phase the R-T surface ends on the brane at some codimension-$3$ surface $ \RTsurf\cap\brane$, which due to symmetry will correspond to a higher dimensional sphere.

%\begin{figure}[h]
%	\centering
%	\includegraphics[width=0.5\linewidth]{images/rtSurface}
%	\caption{Sketch of RT surface for AdS$_4$. Sorry but I messed up the labellings... $\sigma_A$ is should be on the top and $\sigma_B$ is on the bottom. \iar{Can we actually stick to the labelling as in the figure? looks much more natural} }
%	\label{fig:rtsurface}
%\end{figure}


\begin{figure}[h]
 \def\svgwidth{0.6\linewidth}
 \centering{
  \input{3dBrane.pdf_tex}
  \caption{A timeslice of AdS$_{d+1}$ space. Constant $\rho$ hyperbolic foliations are drawn and a brane lives on an AdS$_d$ slice at large $\rho$. On the other boundary of the bulk spacetime lies a $d$-dimensional CFT. \josh{I have to update the figure with correct labellings.}
  }
  \label{fig:cutoffs}
 }
\end{figure}


% Before solving for the area of the surface between a disk on the lower AdS boundary and the brane we will first understand the dominant behaviour at very large tension and small $\delta_\mt{CFT}$ cutoff, which is a UV cutoff around the CFT boundary. Since we are considering the leading order behaviour, we simply apply the Fefferman-Graham coordinates for some asymptotic metric and set the cutoff in the radial $z$ coordinate. Since the geometry in question is time-independent, we perform all calculations on a fixed timeslice.

% Following Rangamani and Takayanagi's book \cite{Rangamani_2017}, we find that around small $z$ in Fefferman-Graham coordinates the metric on the extremal surface $\RTsurf$ is decomposed as
% \beq
% ds^2_{\RTsurf}=\frac{L^2}{z^2}(dz^2 + \tilde{\gamma}_{a b}d\alpha^a d\alpha^b)\,,
% \eeq where $\alpha_i$ are coordinates on the entangling surface. Assuming that the minimal surface falls straight into the bulk from the CFT boundary, we fix $\xi^1$ to be $z$ and find that the leading contribution to the area at this boundary is
% \beq\label{area}
% A(\RTsurf)_{\delta_B} = \int_{\delta_B}^{z_{IR}}\frac{L^{d-1}dz}{z^{d-1}}\int d\xi^{d-2}\sqrt{\tilde{\gamma}}+\dots=\frac{ L^{d-1}A( \sigma_\mt{CFT})}{(d-2)\delta_B^{d-2}}+\dots\,,
% \eeq where $ \sigma_\mt{CFT}$ is the area of the entangling surface on CFT boundary. We can play the same game at the $\rho=\rho_*$ end of the surface, although in this calculation we ``rebundle" the divergent quantity into the induced metric on the brane, as in (\ref{bundle}).



% \beq\label{branearea}
% A(\RTsurf)_{brane} = \int_{\s}^{z_{IR}} dz \Big[\frac{L^{d-1}}{z^{d-1}}\Big(1+\frac{z^2}{4L^2}\Big)^{d-2}\Big]\int d^{d-2}y \sqrt{\AdSdmetric}\,.
% \eeq
% \josh{The $\tg$ determinant has been decomposed into the $z$-dependent part and the $AdS_d$ bare part. The $z$ part can then just be integrated as in chapter 2.}
% where here $\bar{g}_{AdS_d}$ related to the induced metric on the intersection of the brane and the RT surface (denoted $\bar{g}_{ij}$) by
% \beq
% \bar{g}_{ij} = \frac{L^2}{\s^2}\Big(1+\frac{\s^2}{4L^2}\Big)^2 \bar{g}_{ij}^{AdS_d}\,.
% \eeq
% We now simply integrate over the $z$ direction and find, after expanding at small $s$,
% \beq\label{brane area}
% A(\RTsurf)_{brane} = \frac{L}{d-2}A( \RTsurf\cap\brane) + \frac{1}{2(d-4)}\frac{\s^2}{L}A( \RTsurf\cap\brane) + \mathcal{O}(\s^4/L^4)\,.
% \eeq
% From the calculations above we expect that to leading order
% \beq\label{bulk area}
% \frac{A(\RTsurf)}{4 \Gbk}=\frac{L^{d-1}A( \sigma_\mt{CFT})}{4 (d-2)\Gbk \delta_B^{d-2}} + \frac{L A( \RTsurf\cap\brane)}{4(d-2) \Gbk}\,.
% \eeq Therefore we find
% \beq
% S_{EE} = \frac{2 L^{d-1}A( \sigma_\mt{CFT})}{4 (d-2)\Gbk \delta_B^{d-2}} + \frac{A( \RTsurf\cap\brane)}{4 \Geff}\,,
% \eeq where
% \beq
% \frac{1}{\Geff} = \frac{2 L}{(d-2) }\frac{1}{\Gbk} + \frac{1}{\Gbr}\,,
% \eeq which matches (\ref{Geff}) as was desired. Note that we included two contributions of the bulk area (\ref{bulk area}) to account for both sides of the AdS space. Hence we see that the Wald entropy associated to the induced action term is really contained in the bulk RT surface and not a genuine generalized correction to the entanglement entropy. In section \ref{Wald}, we compare the second order term of equation (\ref{brane area}) to the Wald entropy for the curvature-squared terms of the induced action.


We consider the area functional \eqref{eq:badNotation}, with $X^\mu=(z,x^i)$, as in slicing coordinates \eqref{metric3a}, and $\xi^\alpha=(z,y^a)$ for some arbitrary $(d-2)$-many coordinates $y^a$ of the brane. We can expand the transversal profile $X^i=x^i(\xi)$ of the brane in $z$, giving
\beq\label{run11}
x^i(z,y^a) = x^{(0)i}(y^a) + \frac{z^2}{L^2}x^{(1)i}(y^a) + O\left(\frac{z^4}{L^4}\right)
\eeq
The, functions $x^{(n)i}(y^a)$ can in principle be found recursively through extremization of the area of the RT surface; however, we will simply quote the result \cite{Hung_2011}:
\beq
x^{(1)i} = -\frac{L^4 \inducedK^i}{2(d-2) \s^2}\,,
\eeq
with $\inducedK^i$ the extrinsic curvature of the intersection between the brane and the RT surface $\RTsurf$, with respect to the brane. Here, $\inducedK_{iab} = \partial_i h_{ab}$ with $h_{ab}$ being the induced metric on the intersection of the RT surface and the brane, and the index $i$ projected normal to this intersection. Traces and raising and lowering of indices shall be performed with induced metrics; \eg $\inducedK^i \sim O(\inducedK_i \s^2/L^2)$. \vc{I'm trying to choose the normalization of $\inducedK$ to match with \cite{Dong:2013qoa}. I believe our $\inducedK^i$ is $-\s^2/L^2$ times the one in \cite{Hung_2011} (which I think has its index raised using the boundary CFT metric)--- is this correct?} With this, the non-vanishing components of the induced metric $h_{\alpha\beta}$, defined in \eqref{eq:badNotation}, read
\begin{align}
% h_{zz} =& \frac{L^2}{z^2}\Big(1+\frac{z^2}{L^2}h_{zz}^{(1)}+\dots\Big),
\RTmetric_{zz}
=& \frac{L^2}{z^2}\left[
1 + \frac{z^2}{L^2} h_{zz}^{(1)} + O\left(\frac{z^4}{L^4}\right)
\right],
\label{eq:bacardi}\\
% h_{ab}=&\frac{L^2}{z^2}\Big(h^{(0)}_{ab}+\frac{z^2}{L^2}h^{(1)}_{ab}+\dots\Big)\,.
\RTmetric_{ab}
=& \frac{L^2}{z^2}\left(1+\frac{z^2}{4L^2}\right)^2 \QESmetricNoz_{ab},
&
\QESmetricNoz_{ab}
\equiv& \AdSdmetric_{ij}
\frac{\partial x^i}{\partial y^a}
\frac{\partial x^j}{\partial y^b}
= \QESmetricNoz_{ab}^{(0)}
+ \frac{z^2}{L^2} \QESmetricNoz_{ab}^{(1)}
+ O\left(\frac{z^4}{L^4}\right)
\label{eq:jackDaniels}
\end{align}
where
\begin{align}
  \RTmetric_{zz}^{(1)}=& \frac{4}{L^2} \AdSdmetric_{ij} x^{(1)i} x^{(1)j}
  = \frac{L^6}{(d-2)^2 \s^4} \AdSdmetric_{ij} \inducedK^i \inducedK^j
  \sim \frac{L^4}{(d-2)^2 \s^2} \inducedK_i \inducedK^i
  \label{eq:zirkova}
  \\
  \QESmetricNoz_{ab}^{(0)}
  =& \AdSdmetric_{ij}
  \frac{\partial x^{(0)i}}{\partial y^a}
  \frac{\partial x^{(0)j}}{\partial y^b}
\end{align}
\rcm{Comment: I am not a fan of all this funky notation.}
While we will not need an expression for the individual components of $\QESmetricNoz^{(1)}_{ab}$, we will instead use
\begin{align}
  \sqrt{\QESmetricNoz}
  =& \sqrt{\QESmetricNoz^{(0)}}\left[
  1 + \frac{z^2}{L^2} \inducedK_i x^{(1)j}
  + O\left(\frac{z^4}{L^4}\right)
  \right]
  \\
  =& \sqrt{\QESmetricNoz^{(0)}}\left[
  1 - \frac{L^2 z^2}{2(d-2)\s^2} \inducedK_i \inducedK^i
  + O\left(\frac{z^4}{L^4}\right)
  \right]
  \label{eq:absolut}
\end{align}
which comes from using the expansion $\inducedK_i$ to obtain the area element $\sqrt{\QESmetricNoz}$ at $x^i(z,y^a)$ as a perturbation from $\sqrt{\QESmetricNoz^{(0)}}$ at $x^{(0)i}(y^a)$ due to a shift by $z^2 x^{(1)j}/L^2$. With \eqref{eq:bacardi} and \eqref{eq:jackDaniels}, the area functional \eqref{eq:badNotation} now reads
\begin{align}
  \begin{split}
  \frac{\area(\bulkbndry)}{4 G_\bulk}
  =& \frac{1}{4 G_\bulk} \int dz\;\Bigg\{
  \left(\frac{L}{z}\right)^{d-1}
  \left(1+\frac{z^2}{4L^2}\right)^{d-2}
  \\
  &\times \int d^{d-2}y\; \sqrt{
  \QESmetricNoz
  }
  \left[
  1 + \frac{z^2}{2L^2} \RTmetric^{(1)}_{zz}
  + O\left(\frac{z^4}{L^4}\right)
  \right]
  \Bigg\}
\end{split}
\end{align}
Further plugging in \eqref{eq:zirkova} and \eqref{eq:absolut}, we may integrate in $z$ to obtain the leading UV contributions near the brane:
\begin{align}
  \frac{\area(\bulkbndry)}{4 G_\bulk}
  \sim&
  \frac{1}{4 G_\bulk}
  \left(
  \frac{2L}{d-2}
  + \frac{\s^2}{(d-4)L}
  \right)\area(\bulkbndry\cap\brane)
  \\
  &- \frac{L^3}{4(d-2)^2 (d-4) G_\bulk}
  \int d^{d-2}y\; \sqrt{\det(\RTmetric_{ab})} \inducedK_i \inducedK^i
  + O\left(\frac{\s^4}{L^4}\right),
  \label{eq:bazinga}
  \end{align}
  where
  \begin{align}
  A(\sigma\cap\brane)
  =& \int d^{d-2}y\; \sqrt{\det(h_{ab})}
  \\
  \begin{split}
  =& \int dz\;\Bigg\{
  \left(\frac{L}{z}\right)^{d-2}
  \left(1+\frac{z^2}{4L^2}\right)^{d-2}
  \\
  &\times \int d^{d-2}y\;
  \sqrt{\QESmetricNoz^{(0)}}\left[
  1 - \frac{L^2 z^2}{2(d-2)\s^2} \inducedK_i \inducedK^i
  + O\left(\frac{z^4}{L^4}\right)
  \right]
  \Bigg\}.
\end{split}
\end{align}
In \eqref{eq:bazinga}, we have included a factor of $2$ to account for the pieces of the RT surface on the two sides of the brane.
% Alternatively, written in terms of $G_\eff$,
% \begin{align}
%   \begin{split}
%   \frac{\area(\bulkbndry)}{4 G_\bulk}
%   + \frac{\area(\partial(\islands))}{4 G_\brane}
%   =& \frac{1}{4G_\eff}\left[
%   1 + \frac{(d-2)\s^2}{2(d-4)L^2}
%   \right] \area(\bulkbndry \cap\brane)
%   \\
%   &+ \frac{L^2}{8(d-2)(d-4)G_\eff}
%   \int d^{d-2}y\; \sqrt{\det(\RTmetric_{ab})} \inducedK_i \inducedK^i
%   + O\left(\frac{\s^4}{L^4}\right)
% \end{split}
% \end{align}
% where we have assumed the lack of DGP gravity.

We now show that \eqref{eq:bazinga} matches the Wald-Dong entropy formula \cite{Dong:2013qoa}
\beq\label{dong}
S = 4\pi \int d^{d-2}y \sqrt{\det(h_{ab})}
\left[
\lambda_0
+2 \lambda_1 \tilde{R}
+\lambda_2 \left(
\inducedR_{ij} n^{im} \tensor{n}{^j_m}
-\frac{1}{2}
\inducedK_i
\inducedK^i
\right)
\right]\,,
\eeq
for the gravity action
\begin{align}
  \int d^d x\; \sqrt{\inducedg} \left(
  \lambda_{-1} + \lambda_0 \inducedR + \lambda_1 \inducedR^2
  +\lambda_2 \inducedR^{ij} \inducedR_{ij}
  \right).
  \label{eq:woopie}
\end{align}
Here, $h_{ab}$ and $n^i_m$ are the induced metric and unit normals of the entangling surface embedded in the $d$-dimensional spacetime with metric $\inducedg_{ij}$. The tildes denote geometric quantities evaluated using $\inducedg_{ij}$. The coefficients $\lambda_{-1},\ldots,\lambda_2$ are constants, which for us, are chosen so that \eqref{eq:woopie} matches the induced brane gravity action \eqref{totaction}. In particular,
\begin{align}
  \lambda_0
  =& \frac{L}{8\pi (d-2) G_\bulk}
  \\
  \lambda_1
  =& -\frac{d L^3}{32 \pi (d-1)(d-2)^2(d-4) G_\bulk}
  \\
  \lambda_2
  =& \frac{L^3}{8\pi (d-2)^2 (d-4) G_\bulk}.
\end{align}
Immediately, we see that the $O(\s^0/L^0)$ area term and extrinsic curvature term of \eqref{eq:bazinga} match the first and last terms of \eqref{dong}. Using \eqref{curve1} and \eqref{Ricky2}, we find that the remaining two terms in \eqref{dong},
\begin{align}
  \MoveEqLeft[3]4\pi \int d^{d-2}y \sqrt{\det(h_{ab})}
  \left[
  2 \lambda_1 \tilde{R}
  +\lambda_2
  \inducedR_{ij} n^{im} \tensor{n}{^j_m}
  \right]
  \\
  =& 4\pi \int d^{d-2}y \sqrt{\det(h_{ab})}
  \left[
  -\frac{2d(d-1)\s^2}{L^4} \lambda_1
  -\frac{2(d-1)\s^2}{L^4} \lambda_2
  \right]
\end{align}
sum to the $O(\s^2/L^2)$ area term of \eqref{eq:bazinga}. Hence, we see that bulk RT formula produces leading UV contributions near the brane which correspond to the Wald-Dong entropy of the induced gravity on the brane.

% \vc{
% \begin{align}
% h_{zz} =& \frac{L^2}{z^2}\Big(1+\frac{z^2}{L^2}h_{zz}^{(1)}+\dots\Big),
% % h_{zz}
% % =& \frac{L^2}{z^2}\left[
% % 1 + \frac{z^2}{L^2} h_{zz}^{(1)} + O\left(\frac{z^4}{L^4}\right)
% % \right]
% % h_{zz}^{(1)}=& \frac{4z^2}{L^2} \AdSdmetric_{ij} x^{(1)i} x^{(1)j}
% % = \left(\frac{zL}{d-2}\right)^2 \AdSdmetric_{ij} \inducedK^i \inducedK^j
% \\
% h_{ab}=&\frac{L^2}{z^2}\Big(h^{(0)}_{ab}+\frac{z^2}{L^2}h^{(1)}_{ab}+\dots\Big)\,.
% \end{align}
% Note that $h_{ab}=\tilde{g}_{ab}|_{\RTsurf\cap\brane}$ is the induced metric at the intersection of the RT surface and the brane. Now when we studied the behaviour of the RT surface in equation (\ref{branearea}), we assumed that the brane fell straight into the bulk, which is why the extrinsic curvature contributions did not appear. The correct expansion around the brane is \cite{Hung_2011}
% \begin{multline}\label{correctedarea}
%  A(\RTsurf)_{brane} = \int_{\s}^{z_{IR}}dz \Big[\frac{L^{d-1}}{z^{d-1}}\Big(1+\frac{z^2}{4L^2}\Big)^{d-2}\Big]\int d^{d-2}x \sqrt{-\AdSdmetric} \\\times\Big[1+\Big(h^{(1)}_{zz}+h^{(0)ab}h^{(1)}_{ab}\Big)\frac{z^2}{2L^2}+\dots \Big]\,,
% \end{multline} where we notice that the first-order term was the contribution evaluated already. We now focus on the second order term. To raise the indices in the $h^{(0)ab}$, we used the metric $h^{ab}$, which is order $z^2/L^2$. Hence we see that at second order we only need to focus on the $h^{(1)}_{zz}$ term. \josh{Check this is correct, i.e. this second term is indeed subdominant. ALSO, double-check that $\tilde{\mathcal{K}}_i$ is the same as the $K_i$ in Dong.} \vc{$h^{(0)ab}$ is just the inverse of $h^{(0)}_{ab}$ and isn't suppressed.}
% }


% \subsubsection{Wald entropies \label{Wald}}
%
% In the generalized entanglement entropy there are contributions from the brane action which take the form of the Wald entropy, as justified in section \ref{waldjustification}.
%
% We start by computing the Wald entropy for the standard Einstein-Hilbert action because of its relevance to both the induced brane action and physical brane action. The Wald entropy formula is \cite{Myers:2010tj}
% \beq
% S = -2\pi \int_{\mathcal{R}}d^{d-2}x\sqrt{-h}\frac{\partial\mathcal{L}}{\partial R^{ab}_{\,\,\,\,\,cd}}\hat{\epsilon}^{ab}\hat{\epsilon}_{cd}\,,
% \eeq where $\mathcal{L}$ is the Lagrangian density and $\hat{\epsilon}_{ab}$ is the binormal to some region $\mathcal{R}$, and $h_{ij}=\tilde{g}_{ij}$ is the induced metric along that region. In our setup, $\mathcal{R}\equiv \RTsurf\cap\brane$ is the ($d-2$)-dimensional intersection surface between the brane and the bulk Ryu-Takayanagi (RT) surface. As in section \ref{bulkrt}, we refer to the induced metric along this surface by $\bar{g}_{ij}$, which is simply the restriction of $\tilde{g}$ to the surface $\RTsurf\cap\brane$.
%
% Note that the integrand is constant along the brane in our geometry so the equation reduces to
% \beq
% S = -2\pi \frac{\partial\mathcal{L}}{\partial R^{ab}_{\,\,\,\,\,cd}}\hat{\epsilon}^{ab}\hat{\epsilon}_{cd}\int_{\RTsurf\cap\brane}d^{d-2}x\sqrt{-\bar{g}} = -2\pi \frac{\partial\mathcal{L}}{\partial R^{ab}_{\,\,\,\,\,cd}}\hat{\epsilon}^{ab}\hat{\epsilon}_{cd} A(\RTsurf\cap\brane) \,.
% \eeq
% The Einstein-Hilbert Lagrangian density takes the form
% \beq
% \mathcal{L} = \alpha \tilde{R} = \alpha \tilde{R}^{ab}_{\,\,\,\,\,cd} \tilde{g}^{ic}\tilde{g}^{jd}\tilde{g}_{ai}\tilde{g}_{bj}\,
% \eeq from which we compute
% \beq
% \hat{\epsilon}^{ab}\hat{\epsilon}_{cd}\frac{\partial\mathcal{L}}{\partial \tilde{R}^{ab}_{\,\,\,\,\,cd}} =\alpha \hat{\epsilon}^{ab}\hat{\epsilon}_{cd} \tilde{g}^{ic}\tilde{g}^{jd}\tilde{g}_{ai}\tilde{g}_{bj} = -2 \alpha\,,
% \eeq where we used $\hat{\epsilon}^{ij}\hat{\epsilon}_{ij} = -2$ from \cite{Myers:2010tj}. For the actions on the brane, this gives the standard result
% \beq
% S_{brane} = \frac{A(\RTsurf\cap\brane)}{4 \Gbr}\,\,\,\,\,\text{and}\,\,\,\,\, S_{induced}^{(1)} = \frac{L A(\RTsurf\cap\brane)}{4(d-2)\Gbk}\,.
% \eeq These standard results were already used at the end of section \ref{bulkrt}. As promised, we can use this formalism to study the higher curvature terms in the induced brane action to ensure that they provide the same information as the area of the bulk RT surface.
%
% We first consider the two curvature-squared terms independently, which will be combined by linearity. Consider the Lagrangian density
% \beq
% \mathcal{L} = \kappa R^2\implies \hat{\epsilon}^{ab}\hat{\epsilon}_{cd}\frac{\partial\mathcal{L}}{\partial R^{ab}_{\,\,\,\,\,cd}} = - 4 \kappa R\,.
% \eeq Also, we need to consider
% \beq\label{RicciTensorTerm}
% \mathcal{L} = \gamma R^{de}R_{de} =\gamma R^{ab}_{\,\,\,\,\,cd}R^{\,\,\,\,\,ld}_{jk}g_{ai}g_{be}g^{ic}g_{jm}g_{ml}g^{ke}\implies \hat{\epsilon}^{ab}\hat{\epsilon}_{cd}\frac{\partial\mathcal{L}}{\partial R^{ab}_{\,\,\,\,\,cd}} =-4\gamma\hat{R}\,,
% \eeq
% whenever $R_{ij} = \hat{R}g_{ij}$.
% Now we turn to the curvature-squared terms of the induced bulk action (\ref{bulkaction}). Applying the variations above, we find
% \beq
% S_{induced}^{(2)} = \frac{8 L^3 \s^2}{(d-4)(4L^2+\s^2)^2}\frac{A(\RTsurf\cap\brane)}{4 \Gbk}\,.
% \eeq Now expanding this to leading order in $s$, we find
% \beq
% S_{induced}^{(2)} = \frac{ \s^2}{2(d-4)L}\frac{A(\RTsurf\cap\brane)}{4 \Gbk}\,,
% \eeq which matches the analogous term from \ref{brane area}.
%
% \subsubsection{Dong entropies and extrinsic curvature corrections}
%
% So far we ignored the extrinsic curvatures of the entangling surface on the brane. Following \cite{Bhattacharyya_2014_2, Dong_2014}, we consider a second derivative theory of gravity ($\mathcal{L}^{(2)} = \lambda_1 \tilde{R}^2 + \lambda_2 \tilde{R}_{\mu\nu}\tilde{R}^{\mu\nu}$) with entropy \vc{I vaguely recall that Dong defines his Lagrangians and actions with a minus sign relative to the usual definition. See, for example, (3.35) which would give a negative area term for entropy if an Einstein Hilbert action with the usual sign is used. I think the minus sign he puts in front of the $S$ in (2.4) is inconsistent with his convention for the rest of the paper, \eg see (2.12). Also, his formulas are for Euclidean signature. For us, I think we should scrap the minus sign out front in \eqref{dong}.}
% \beq\label{dong}
% S = -4\pi \int d^{d-2}x \sqrt{-\bar{g}}\Big[2 \lambda_1 \tilde{R} +\lambda_2 \Big(\tilde{R}_{\mu\nu}n_i^{\mu}n_i^{\nu}-\frac{1}{2}\tilde{\mathcal{K}}_i\tilde{\mathcal{K}}^i\Big)\Big]\,,
% \eeq where $n_i$'s are the two normals to the entangling surface. Note that in our setup,
% \beq
% \tilde{R}_{\mu\nu}n_i^{\mu}n_i^{\nu} = \hat{R}\tilde{g}_{\mu\nu}n_i^{\mu}n_i^{\nu} = \hat{R}\sum_{i=1}^2 n_i^{\mu}n_{i \mu} = 2\hat{R}\,,
% \eeq where we used the normalization of the normal vector. This contribution to the entropy agrees with equation (\ref{RicciTensorTerm}). In our calculations below we consider only the one-sided bulk. Including both contributions simply requires a factor of two multiplying the Dong entropy.
%
% We now present an argument to show that the minimal surface calculation also includes the extrinsic term of equation (\ref{dong}). The argument follows \cite{Hung_2011}.
%
%
%
% It was shown in \cite{Hung_2011} that the second-order contribution to the RT surface embedding coordinates can be written in terms of the extrinsic curvature,
% \beq
% X^{(1)i} = \frac{L^2 \tilde{\mathcal{K}}^i}{2(d-2)}\,,
% \eeq and the induced metric can be expanded via
% \beq
% h_{zz} = \frac{L^2}{z^2}\Big(1+\frac{4z^2}{L^4}(X^{(1)i})^2+\dots\Big)\implies h^{(1)}_{zz} = \frac{L^2 (\tilde{\mathcal{K}}^i)^2}{(d-2)^2}\,.
% \eeq
% We now substitute this expression into equation (\ref{correctedarea}) and integrate out the $z$ direction. Upon expanding at small $\s$, we obtain
% \beq
% A(\RTsurf)^{(1)}_{brane} = \frac{L \s^2}{2 (d-4)(d-2)^2}(\tilde{\mathcal{K}}^i)^2 \int d^{d-2}x \sqrt{-\tilde{g}}\,,
% \eeq and hence the second order contribution to the entanglement entropy is
% \beq
% S^{(1)} = \frac{1}{4 \Gbk} \frac{L \s^2}{2 (d-4)(d-2)^2}(\tilde{\mathcal{K}}^i)^2 A(\RTsurf\cap\brane)\,,
% \eeq which precisely matches equation (\ref{dong}) after computing $\lambda_2$ from the induced brane action (\ref{bulkaction}),
% \beq
% \lambda_2= \frac{L^3}{16 \pi(d-4)(d-2)^2 \Gbk}\,.
% \eeq
% \josh{I need to be a bit more careful... the left over $s^2/L^2$ comes from the raising and lowering of the $i$ indices compared to Dong's formula or from the metric in Dong's formula?.}
% From these calculations we conclude that the entropies associated to the induced action on the brane in the Randall-Sundrum picture give exactly the leading contributions to the RT surface area in the $(d+1)$-dimensional bulk!
% %

\subsection*{A comment on $d=2$ case} \label{DeeTwo}
\rcm{comment that we can only get contributions of $\ric$ or $\ric^2$ terms with details of profile. Is that true??} \vc{I think so. This was another reason I wanted to treat these as part of the matter effective action rather than as part of a gravitational action \Smiley. I don't think applying the Wald-Dong entropy formula to the finite part in \eqref{induct} will ever recover the bulk profile of the RT surface, even if the $\cdots$ are continued to arbitrarily high orders.}

\rcm{note to leading order contributions derived from eq.~\reef{induct} or from eq.~\reef{PolyAct2} and then substituting eq.~\reef{sol4} match. Would this be true beyond leading order??}

% We see that the equations are slightly different in $d=2$ since the calculation in (\ref{area}) will introduce a log rather than a powerlaw behaviour. This will again match the RS-picture side.

To close this section, we briefly remark that the $d=2$ case is somewhat special in that the intersection between the RT surface and the brane is a point. Consequently, the leading UV contribution to entropy is not a standard area term, but rather a logarithmic term. Integrating the RT area (in this case, length) gives
% The leading order behaviour of the bulk RT surface is just a single integral,
\beq
S
\sim \frac{1}{2 G_\bulk}\int \frac{L}{z}dz
\sim \frac{L}{2G_\bulk} \log\left(\frac{L_\IR}{\s}\right)\,,
\label{eq:kaboom}
\eeq
Here, we have selected out the contribution due to the RT surface approaching the brane and we have introduced an IR length scale $L_\IR$ to make the argument of the logarithm dimensionless. A factor of two has been included to account for both sides of the brane. This can also be obtained by evaluating the Wald entropy formula \cite{Wald:1993nt} (see also eq.~(3.35) in \cite{Dong:2013qoa}) for the induced gravity action \eqref{induct} with Lagrangian $\sqrt{-\inducedg}\Lcal(\inducedR)$:
% We also take the variation of the $d=2$ induced action to compute its Wald entropy \cite{Dong_2014}. We find
\begin{align}
 S
 =& 4\pi \frac{\partial \Lcal(\inducedR)}{\partial \inducedR}
 \sim -\frac{1}{4G_\eff} \log\left(-\frac{L^2 \inducedR}{2}\right)
 \sim \frac{L}{2G_\bulk} \log\left(\frac{L}{\s}\right)
 % \frac{\partial \mathcal{L}}{\partial \tilde{R}} = \frac{1}{4 G_{3}}\frac{\partial }{\partial \tilde{R}}\Big(\frac{2}{L} -\frac{1}{2}L \tilde{R} \log\Big(-\frac{L^2}{ 2} \tilde{R}\Big) + \frac{L}{2}\tilde{R}+\frac{L^3}{16}\tilde{R}^2\Big)\\=-\frac{L}{4G_3} \log\Big(\frac{\s}{L}\Big)\,,
\end{align}
in agreement with \eqref{eq:kaboom} upon setting $L_\IR=L$. Alternatively, one may apply this formula to the Lagrangian for the Polyakov-Liouville action \eqref{PolyAct2}, giving the same answer upon setting $\phi$ equal to the on-shell value \eqref{sol4}.
% which matches the RT surface calculation (after expanding to leading order in $\s$)!
% \josh{This calculation is using equation 3.35 of \cite{Dong:2013qoa}}


==> sections/HEE2__Vincent_Chen_s_conflicted_copy_2020-06-08_.tex <==
% !TEX root = ../lifeonbrane3.tex

\subsection{Explicit Calculations}\label{sec:examples}

In this section, we explicitly evaluate the holographic EE and examine the transition between the two classes of RT surfaces. While we set up the calculations for general $d>2$, our explicit results are given for $d=3$ in which case the bulk spacetime locally has the geometry of AdS$_{4}$. We add some comments about $d=2$, and the addition of Jackiw-Teitelboim gravity \reef{JTee} on the brane, in the discussion section.

\subsubsection*{Setting up the calculation for general dimension}

In section \ref{sec:enzyme}, we reviewed two different coordinate systems in AdS$_{d+1}$. The AdS$_d$ foliation \reef{metric3a} was well suited to discuss the brane geometry, while the global coordinates are adapted to discuss the background geometry of the boundary CFT. However, our explicit calculations of the holographic EE are best performed in a new `cylindrical' coordinate system. In particular, following \cite{Krtous:2014pva}, we introduce cylindrical coordinates $P,\,\zeta$ where $\zeta$ specifies the position along the axis of the cylinder while $P$ measure the distance from the axis. These are related to the global coordinates in eq.~\reef{metric2s} by
\begin{align}\label{cylie}
\cosh r&=\sqrt{P^2+1}\,\cosh\zeta\,,\\
%\sinh r&=\sqrt{\frac{P^2+\tanh^2\zeta}{1-\tanh^2\zeta}}\,,\\
\tan\theta&=\frac{P}{\sqrt{1+P^2}}\,\frac{1}{\sinh\zeta}\,,
\end{align}
while the rest of the spherical angles remain unchanged. With this transformation, the metric becomes
\beq\label{cylindd}
ds^2=L^2\[ -(P^2+1)\cosh^2\zeta\, dt^2+\frac{dP^2}{1+P^2}+\left( 1+P^2 \right)d\zeta^2+P^2\,d\Omega_{d-2}^2\]\,.
\eeq
The range of these coordinates is $P\in (0,\infty)$ and $\zeta\in(-\infty,\infty)$. The conformal boundary is reached with $P\to \infty$ (or $\zeta\to\pm\infty$ with fixed $P$).  The upper ($0\le\theta\le\pi/2$) and lower ($\pi/2\le\theta\le\pi$) hemispheres are mapped to the upper ($\zeta\ge0$) and lower ($\zeta\le0$) halves of the cylindrical system. The conformal defect is positioned at $\zeta=0$. As noted above, the RT surfaces will be restricted to a constant time surface and hence the convenience of the cylindrical coordinates becomes evident, \ie  $\zeta$ becomes an extra Killing coordinate in the corresponding spatial geometry.


A few more technical details are needed  for our calculations:
in cylindrical coordinates \reef{cylindd}, the boundary entangling surface corresponds to the two circles $\zeta=\pm\zeb$, where
\beq\label{zeta0}
\sinh\zeb=\tan\thb\,,
\eeq
seen in the limit $P\to\infty$ of the second line in eq.~\reef{cylie}. Using the AdS foliation of eq.~\reef{metric3a}, the position of the brane was $z=\s$. Using eq.~\reef{eq:foobar}, the brane position can be specified in cylindrical coordinates \reef{cylindd} according to 
\beq\label{eq:foobar2}
 \(1+P^2\)\sinh^2\!\zeta=\frac{L^2}{\s^2}\(1-\frac{\s^2}{4L^2}\)^2\,.
\eeq
Recall that the brane intersects the asymptotic boundary at the position of the conformal defect, \ie at $\theta=\pi/2$ with $r\to\infty$, which corresponds to $\zeta= 0$ with $P\to \infty$ in cylindrical coordinates. Further recall that RT surface areas are UV divergent since they extend to the asymptotic boundaries.  Hence we introduced a UV regulator surface at $r=r_\mt{UV}$, which in cylindrical coordinates becomes
\beq\label{regular}
(P^2+\tanh^2\zeta)\cosh^2\zeta=\sinh^2\! r_\mt{UV}\,.
\eeq
We will be mainly interested in comparing the areas of different surfaces for fixed $\zeb$, as discussed above. Since the UV divergent terms only depend of the geometry of the entangling surface, they will cancel in the difference of the two areas. Hence, we can then safely take the UV cutoff to infinity.

As noted, the RT surfaces all lie in a fixed time slice and thus we only need consider configurations with cylindrical symmetry (\ie rotational symmetry on the $S^{d-2}$). Hence it is convenient to use the cylindrical coordinates \reef{cylindd} and  parametrize the profile of the bulk surfaces as $\zeta=\zeta(P)$. The bulk contribution to the holographic EE is given by
\begin{align}\label{area}
S_\mt{bulk}= \frac{L^{d-1}\, \Omega_{d-2}}{2\,\Gbk} \int dP P^{d-2} \sqrt{\frac{1}{1+P^2}+(1+P^2)\,\zeta'^2}
\end{align}
where again $\Omega_{d-2}$ is the area of the unit $(d-2)$-sphere -- see footnote \ref{footsphere}. As in eq.~\reef{area0}, an overall factor of 2 is included here to account for the reflection symmetry of the profile $\zeta(P)$ about the brane. Since this expression does not contain an explicit $\zeta$ dependence, it is straightforward to derive
\begin{align}\label{zetap}
\zeta'(P)=\pm \frac{1}{1+P^2}\,\sqrt{\frac{P_0^{2(d-2)}\(1+P_0^2\)}{P^{2(d-2)}\(1+P^2\)-P_0^{2(d-2)}\(1+P_0^2\)}}
\end{align}
where the two branches correspond to two identical surfaces related by a reflection with respect to $\zeta=0$. $P_0$ corresponds to the turning point, where the surface makes its closest approach to the symmetry axis.

We now discuss the disconnected phase described at the beginning of this section. It corresponds to the `trivial' solution with $P_0=0$. We find $\zeta(P)=\pm\zeb$, which in cylindrical coordinates looks simply as a pair of disks anchored at the boundary entangling surface. Substituting $\zeta'=0$ into eq.~\reef{area}, the area of the two discs can be integrated up to some cutoff radius $P_\mt{UV}$, and the corresponding holographic EE is
\begin{align}\label{A_disc}
S_\mt{disc}=\frac{L^{d-1}\, \Omega_{d-2}}{2(d-1)\,\Gbk} \ \puv^{d-1}\, {}_{2}F_1\left[ \frac{1}{2},\frac{d-1}{2},\frac{d+1}{2},-\puv^2 \right]\,.
\end{align}
In this case, the entanglement wedge corresponds to two identical disconnected pieces contained between each component of the RT surface and the asymptotic boundary, \ie the regions $\zeta\ge+\zeb$ and $\zeta\le-\zeb$, as sketched in the upper panel of figure \ref{fig:RTPhases}. 
%\dn{changed non-existent reference to figure \ref{fig:RTPhases}. Note that there are no a) / b) labels in the figure though. Do you just want to refer to \ref{fig:RTPhases}, or should we add a new figure to the beginning of section 4 which shows the two possible RT surfaces in the style of \ref{fig:cutoffs}?}
%
%\begin{figure}[h]
%\begin{center}
%\includegraphics[scale=.5]{images/EWs}
%\caption{Sketch of fixed time slices of our setup, showing the two possible configurations. The shaded region corresponds to the entanglement wedge.}
%\label{fig:EWs}
%\end{center}
%\end{figure}


\begin{figure}
	\def\svgwidth{0.8\linewidth}
	\centering{
		\input{RTPhases2.pdf_tex}
		\caption{Sketch of fixed time slices of our symmetric setup, showing the two possible configurations. The shaded red region corresponds to the entanglement wedge. The connected solution contains an island on the brane, where gravity is dynamical.}
		\label{fig:RTPhases}
	}
\end{figure}

The connected phase corresponds to $P_0>0$, which leads to a cylindrical RT surface. Integrating eq.~\reef{zetap} yields a family of bulk surfaces, which are symmetric about the brane and which are anchored on the asymptotic boundary at $\zeta=\pm\zeb$. Recalling the discussion below eq.~\reef{area0}, we observe that in this configuration, $P_0$ is the second integration constant which must be tuned in order to satisfy the appropriate boundary condition \reef{ortho1} at the brane, see the lower panel of figure \ref{fig:RTPhases}.

Before we calculate the entropy in the most general setting, let us consider the case of a zero-tension brane with $1/\Gbr=0$, \ie empty AdS$_{d+1}$. In this case, the brane is positioned at $\s=2L$ or simply, $\zeta=0$. Now, the `plus' branch of eq.~\eqref{zetap} can be integrated to produce a profile extending from $P=\puv$ at $\zeta=+\zeb$ to the maximal depth $P=P_0$ at some $\zeta=\zeta_0(\zeb,P_0)<\zeb$. Since eq.~\reef{ortho1} indicates that the RT surface must intersect the brane orthogonally, we must tune $P_0$ (with fixed $\zeb$) such that $\zeta_0=0$, \ie the RT surface reaches its maximal depth at the brane position. Now, substituting eq.~\reef{zetap} into eq.~\reef{area}, the holographic EE (for empty AdS$_{d+1}$) becomes
\begin{align}\label{A_conn}
S_\mt{conn}(T_o=0)
%&=2L^{d-3}S_{d-2} \int_{P_0}^P dp \frac{p^{d-2}}{\sqrt{1+p^2}} \sqrt{1+\frac{P_0^{2(d-2)}+P_0^{2(d-1)}}{p^{2(d-2)}+p^{2(d-1)}-P_0^{2(d-2)}-P_0^{2(d-1)}}}\\
&=\frac{L^{d-1}\, \Omega_{d-2}}{2\,\Gbk} \int_{P_0}^{\puv}\!\!\! dP\,  \frac{P^{2(d-2)}}{\sqrt{P^{2(d-2)}(1+P^2)-P_0^{2(d-2)}(1+P_0^2)}}\,.
\end{align}

In the general case, this exercise is slightly more complicated for the case of interest with a finite-tension DGP brane at some $z=\s\ll L$, and the geometry of the corresponding RT surface is illustrated in the lower panel of figure \ref{fig:RTPhases}. The RT surface is again symmetric about the brane and so as above, we focus on the portion starting at $\zeta=+\zeb$ at the asymptotic boundary (\ie at $P=\puv$). As before, the `plus' branch of eq.~\eqref{zetap} produces a surface reaching its maximal depth $P=P_0$ at some $\zeta=\zeta_0(\zeb,P_0)<\zeb$.\footnote{In fact, $\zeta_0(\zeb,P_0)$ is precisely the same function introduced above, since the turning point of the RT surfaces are completely independent of the brane properties.}  Now one continues from this point using the `minus' branch of eq.~\reef{zetap}, which then meets the brane as some $P=P_\mt{B}(\zeb,P_0)$ and $\zeta=\zeta_\mt{B}(\zeb,P_0)$.\footnote{Of course, $P_\mt{B}$ and $\zeta_\mt{B}$ are related as in eq.~\reef{eq:foobar2}.} One would again tune $P_0$ (for fixed $\zeb$) to ensure the appropriate boundary condition \reef{ortho1} is satisfied at the brane.
The bulk contribution to the holographic EE then becomes
\beqa
S_\mt{conn}(T_o>0)&=&\frac{L^{d-1}\, \Omega_{d-2}}{2\,\Gbk}\[ \int_{P_0}^{\puv}\!\!\!  dP\,  \frac{P^{2(d-2)}}{\sqrt{P^{2(d-2)}(1+P^2)-P_0^{2(d-2)}(1+P_0^2)}}\right.
\labell{Acon2}\\
&&\qquad\qquad\qquad+\left. \int_{P_0}^{\pb}\!\!  dP\,  \frac{P^{2(d-2)}}{\sqrt{P^{2(d-2)}(1+P^2)-P_0^{2(d-2)}(1+P_0^2)}}\]\,.
\nonumber
\eeqa
Of course, if there is no gravitational term on the brane (\eg as in eq.~\reef{newbran}), then this expression yields the entire generalized entropy \reef{eq:sgen_intro} for the connected phase. Now
rather than explicitly examining the brane boundary condition \reef{ortho1} in cylindrical coordinates, we will simply evaluate the generalized entropy and find the minimum numerically in the following. Hence to proceed further we will have to choose a specific value for the boundary dimension $d$.

\subsubsection*{Explicit results for $d=3$}
In this section, we consider the above discussion for $d=3$, in which case the boundary geometry becomes $\Rbb\times S^{2}$, the bulk spacetime is locally AdS$_4$, and the branes have an AdS$_3$ geometry. We will also consider supplementing the the four-dimensional bulk action \reef{act2} with a Gauss-Bonnet term, %\iar{I suggest including this term with an extra $L^2/\Gbk$, so that 1) it is of the same 'order' as the area term when $\lgb\sim 1$, and 2) we can remove this global prefactor in e.g. fig \ref{figdeltaA} }
 \beq
I_\mt{top} = \frac{\lgb}{16\pi^2}  \int \mathrm{d}^4x \, \sqrt{-g}\, \left[ R_{abcd}R^{abcd}-4\,R_{ab}R^{ab}+R^2 \right]\,.
 \labell{top2}
 \eeq
Note that we have ignored the necessary boundary terms which ensure that this interaction is proportional to the Euler density, \eg see \cite{Myers:1987yn}. Although this curvature-squared term does not effect the bulk equations of motion, it will contribute to the generalized entropy \cite{Dong:2013qoa,Hung:2011xb}\footnote{One may worry that the topological nature of $I_\mt{top}$ undercuts the usual derivations of the generalized entropy. However, individually the three terms in eq.~\reef{top2} are dynamical and one can apply the results of \cite{Dong:2013qoa} for each separately and then take the sum of the corresponding contributions to the holographic entropy, which one finds matches the result in eq.~\reef{Euler3}.}
 \beq
S_\mt{JM} = \frac{\lgb}{4\pi} \int_{\Sigma_\xR} d^2x\sqrt{h}\,\mR +\frac{\lgb}{2\pi} \int_{\partial \Sigma_\xR}
dx\sqrt{h}\,\mK_g \,,
 \labell{Euler3}
 \eeq
where $\mR$ denotes the Ricci scalar for the intrinsic geometry on the RT surface $\Sigma_\xR$. Similarly, $\mK_g$ denotes the geodesic curvature of the boundary $\partial \Sigma_\xR$. Of course, eq.~\reef{Euler3} gives a topological contribution proportional to the Euler character of the two-dimensional extremal surfaces\footnote{The normalization is chosen so that for an RT surface with two-sphere topology, $S_\mt{JM} = 2 \lgb$.} and so their geometry remains unaffected by this term. However, in the following, this additional contribution will  provide an extra parameter which allows us to adjust the transition between the connected and disconnected phases.

For $d=3$, some analytic expressions for the extremal surfaces can be obtained \cite{Krtous:2014pva}. For example,
integrating eq.~\eqref{zetap} yields the following profile for the extremal surface in empty AdS$_4$ \cite{Krtous:2014pva}
\beqa
&&\zeta_\pm(P;P_0,\zeta_0)=\zeta_0\pm \frac{P_0}{\sqrt{(1+P_0^2)(1+2P_0^2)}} \labell{zetasol} \\
&&\times\left[ (1+P_0^2)\, F\!\left( \mbox{Arcos} \frac{P_0}{P},\sqrt{\frac{1+P_0^2}{1+2P_0^2}} \right)-P_0^2\, \Pi\!\left( \mbox{Arccos}\frac{P_0}{P},\frac{1}{1+P_0^2},\sqrt{\frac{1+P_0^2}{1+2P_0^2}} \right) \right]
\nonumber
\eeqa
where $F$ and $\Pi$ correspond to incomplete elliptic integrals of the first and third kind, respectively.\footnote{Our notation for the elliptic integrals matches that in \cite{Gradshteyn:1702455}, section 8.1.} Again, the $\pm$ branches correspond to the two portions of the surface, symmetric with respect to $\zeta_0=0$. Of course, we need to know where this surface is anchored at the boundary. Hence we define
\beqa
\zeta_\infty&\equiv&\zeta_+(P\to \infty;P_0,\zeta_0)-\zeta_0
\labell{alphadog}\\
&=&\frac{P_0\left[ (1+P_0^2)\,K\!\left( \sqrt{ \frac{1+P_0^2}{1+2P_0^2} }\right) - P_0^2\, \Pi\!\left( \frac{1}{1+P_0^2},\sqrt{\frac{1+P_0^2}{1+2P_0^2}} \right) \right]}{\sqrt{(1+P_0^2)(1+2P_0^2)}}
\nonumber
\eeqa
and the surface reaches the asymptotic boundary at $\zeta_\pm(P\to \infty)=\zeta_0\pm \zeta_\infty$. Hence the two components of the entangling surface in the boundary theory are separated by $2\zeta_\infty$, in the cylindrical coordinates.

Figure \ref{figzetainfty} plots $\zeta_\infty$ as a function of $P_0$. The maximum is obtained at $P_0=P_0^{\mt{crit}}\approx 0.51633$ with $\zeta_\infty=\zeta_\infty^{\mt{crit}}\approx 0.5011$. An interesting observation in \cite{Krtous:2014pva} was that, for $P_0<P_0^{\mt{crit}}$, there exist \textit{two} values of $P_0$ with the same $\zeta_\infty$. That is, if the two components of the entangling surface are sufficiently `close' on the boundary sphere, there actually exist \textit{two} extremal RT surfaces that connect them in the bulk. However, one branch (with the smaller value of $P_0$) is always subdominant, and therefore will be of little interest in our analysis. On the other hand, if the separation of the two entangling spheres  is larger than the critical value $2\zeta_\infty^{\text{max}}$ (in cylindrical coordinates), there is no connected extremal surface that joins them.
%
%\begin{figure}[h]
%\begin{center}
%\includegraphics[scale=0.4]{images/zetainfty}
%\caption{Plot of the `height' of the RT surface in cylindrical coordinates, as a function of the turning point $P_0$ characterising the surface. For $\zeta_\infty<\zeta_\infty^{\mt{crit}}$, there are two minimal surfaces anchored at the same regions; otherwise there exists none. }
%\label{figzetainfty}
%\end{center}
%\end{figure}

\begin{figure}[h]
	\def\svgwidth{0.5\linewidth}
	\centering{
		\input{rtHeight.pdf_tex}
		\caption{Plot of the `height' of the RT surface in cylindrical coordinates, as a function of the turning point $P_0$ characterising the surface. For $\zeta_\infty<\zeta_\infty^{\mt{crit}}$, there are two minimal surfaces anchored at the same regions; otherwise there exists none. 
		}
		\label{figzetainfty}
	}
\end{figure}

Let us now describe the solutions corresponding to different values of the tension and DGP term:
%\dn{Should we mention somewhere around here that $T_o = 0$ is not einstein gravity on the brane?}\iar{Not needed here, since T_o=0 means the brane doesn't exist}.
\paragraph{a) $T_o=0;\ 1/\Gbr=0$\ :} First we consider the holographic EE in empty AdS$_4$ as a lead-in to the case with a brane. As emphasized above, the area of these surfaces is divergent, and so one introduces a UV regulator surface,  integrating of the area from $P_0$ to some $\puv\gg1$ \cite{Krtous:2014pva}. For the disconnected solution (\ie a pair of disks), eq.~\eqref{A_disc} with $d=3$ gives
\begin{align}\label{Sdisc}
S_\mt{disc}(\puv)
=& \frac{\pi L^2}{\Gbk}\,\left( \sqrt{1+\puv^2}-1 \right)+2 \lgb
\\
=& \frac{A(S^1_{\puv})}{4G_\mt{eff}}
- \frac{\pi L^2}{G_\bulk} + 2\lgb
+ \Ocal(\puv^{-1})\,.
\label{eq:lonely}
\end{align}
where
\beq\label{sample}
\frac{A(S^1_P)}{4G_\mt{eff}}=\frac{\pi L^2}{\Gbk}\,P\,,
\eeq
is the length of $S^1_P$, a circle with radius $P$, and we used eq.~\reef{Newton2} to write $\frac{1}{G_\mt{eff}}=\frac{2\,L}{\Gbk}$.
We have included in eq.~\eqref{Sdisc} the topological contribution in eq.~\reef{Euler3}. On the other hand, for the connected surfaces the area formula \eqref{A_conn} yields
\begin{align}\label{eq:dietCoke}
\begin{split}
\MoveEqLeft[3]
S_\mt{conn}(\puv,P_0)
\\
=& \frac{\pi L^2}{\Gbk}\,\frac{P_0^2}{\sqrt{1+2P_0^2}}\, \Pi\!\left( \mbox{Arccos}\frac{P_0}{\puv},1,\sqrt{\frac{1+P_0^2}{1+2P_0^2}} \right)
\end{split}
\\
\begin{split}
=& \frac{A(S^1_{\puv})}{4G_\mt{eff}}
+ \frac{\pi L^2}{G_\bulk}\left[
-\sqrt{1+2P_0^2} E\left(\sqrt{\frac{1+P_0^2}{1+2P_0^2}}\right)
+ \frac{P_0^2}{\sqrt{1+2P_0^2}} K\left(\sqrt{\frac{1+P_0^2}{1+2P_0^2}}\right)
\right]
\\
&+ \Ocal(\puv^{-1})\,,
\end{split}
\label{eq:friendless}
\end{align}
where $E$ is the elliptic integral of the second kind. We emphasize that this result only applies for  vanishing $T_o$ and vanishing $1/\Gbr$, \ie  for the AdS$_4$ vacuum. Note that the Euler character of the cylindrical RT surface is zero and hence there is no contribution proportional to $\lgb$. As expected, the divergence in the $\puv\to\infty$ limit matches for the areas of the connected and disconnected surfaces. Hence we can safely take the limit when considering the difference
\begin{align}\label{dAP01}
\Delta S(P_0)&=\lim_{\puv\to \infty}\left( S_\mt{conn}(\puv,P_0)-S_\mt{disc} (\puv)\right)\,,
\end{align}
given by the difference in $O\left( \left( P_0/\puv \right)^0 \right)$ terms in eq.~\eqref{eq:friendless} and eq.~\eqref{eq:lonely}.
A plot of $\Delta S$ is shown in figure \ref{figdeltaA}. When $\Delta S>0$, the disconnected RT surface is the dominant saddle, while for $\Delta S<0$, the connected solution dominates. Notice that with a larger (positive) topolgical coupling $\lgb$, the entropy in eq.~\reef{Sdisc} increases while eq.~\reef{eq:dietCoke} is unaffected, and hence the range of the disconnected phase is decreased in figure \ref{figdeltaA}.

%\footnote{Of course, $\Delta S(P_0)$ is closely related to the mutual information. \rcm{words:} Mutual information between two subsystems $A$ and $B$ is defined via $I=S_{A\cup B}-S_A-S_B$. Notice that whenever $\Delta S>0$, phase $I$ dominates and therefore the mutual information vanishes, since $S_{A\cup B}=S_A+S_B$.}
%
%\begin{figure}[h]
%\begin{center}
%\includegraphics[scale=0.3]{images/dAP0}
%\caption{Renormalised entropy from eq. \eqref{dAP01}. The connected (disconnected) surface dominates when $\Delta S<0\,(\Delta S>0)$. When $\lgb$ to becomes very large, $\lgb\sim c_T$, the connected solution becomes favoured. }
%\label{figdeltaA}
%\end{center}
%\end{figure}

\begin{figure}[th]
	\def\svgwidth{0.8\linewidth}
	\centering{
		\input{figdeltaA2.pdf_tex}
		\caption{Renormalised entropy from eq. \eqref{dAP01}. The connected (disconnected) surface dominates when $\Delta S<0\,(\Delta S>0)$. When $\lgb$ becomes very large, $\lgb\sim c_T$, the connected solution becomes favoured.}
		\label{figdeltaA}
	}
\end{figure}

\paragraph{b) $T_o\ne 0;\ 1/\Gbr=0$\ :} The next step is to introduce the brane, however, we do not include an additional gravitational interaction in the brane action yet, \ie $1/\Gbr=0$. In this case, we saw  in eq.~\reef{Acon2} that there is an additional contribution as the RT surface extends from the maximal depth $P_0$ back out to meet the brane at $P_\mt{B}$. Both contributions in eq.~\reef{Acon2} take the same form except for the limits of integration, hence the $d=3$ result in eq.~\reef{eq:dietCoke} is replaced by
\beqa
S_\mt{conn}(\puv,P_0)&=& \frac{\pi L^2}{\Gbk}\,\frac{P_0^2}{\sqrt{1+2P_0^2}}\,\[ \Pi\!\left( \mbox{Arccos}\frac{P_0}{\puv},1,\sqrt{\frac{1+P_0^2}{1+2P_0^2}} \right)\right.
\labell{CokeZero}\\
&& \left.\qquad\qquad+\Pi\!\left( \mbox{Arccos}\frac{P_0}{\pb},1,\sqrt{\frac{1+P_0^2}{1+2P_0^2}} \right)\]\,.
\nonumber
\eeqa


Of course, the entropy for the disconnected phase remains the same as in eq.~\reef{Sdisc} and we can consider the difference of the generalized entropy evaluated on the connected and disconnected extremal surfaces, as in eq.~\reef{dAP01}. Just as we saw a leading divergent contribution in eq.~\reef{eq:dietCoke} for $\puv\to\infty$, we expect that eq.~\reef{CokeZero} will contain an analogous large contribution for $\pb\gg P_0$. However, this term will not be cancelled in $\Delta S$. In fact, in this regime, we can expand the difference as
\begin{align}\label{radishes}
\begin{split}
\MoveEqLeft[2]\Delta S(P_0)
\\
=& \frac{A(\sigma_\xR)}{4G_\mt{eff}}
+ \frac{\pi L^2}{G_\bulk}\left[
1-2\sqrt{1+2P_0^2} E\left(\sqrt{\frac{1+P_0^2}{1+2P_0^2}}\right)
+ \frac{2P_0^2}{\sqrt{1+2P_0^2}} K\left(\sqrt{\frac{1+P_0^2}{1+2P_0^2}}\right)
\right]
\\
&-2 \lgb
+ \Ocal(\pb^{-1})\,.
\end{split}
\end{align}
Here, the intersection $\sigma_\xR$ of the RT surface and the brane is a circle of radius $\pb$ with area $A(\sigma_\xR)=2\pi L\,\pb$ given by eq.~\eqref{cylindd}. The fact that the leading term can be expressed as the gravitational entropy for the induced gravity action \reef{act3} on the brane is in perfect agreement with our discussion in the previous section. As we will see below, the finite terms will play a role once we turn on the DGP term, allowing for the appearance of a different island on the brane. 

From the above expansion, we see that there is a strong penalty for having a large $\sigma_\xR$ in the connected phase. From the brane perspective, the gravitational entropy results in a large penalty against forming an island on the brane. In fact, generally we expect that $\Delta S>0$ in this regime and hence the disconnected solution provides the dominant saddle point. However, if we tune the topological coupling $\lgb$ to be large\footnote{We note that this requires $\lgb\sim {L^2}/{\Gbk}\sim \cT$, the central charge of the boundary CFT -- see further discussion in section \reef{sec:discussion}.} (and positive), this contribution can compensate for the leading gravitational entropy term, at least for $\sigma_\xR$ up to a certain size.

On the other hand, we must note that $\pb$  is not an independent parameter. Rather it is implicitly determined by $\zeb$ and the brane tension $T_o$, as well as the value of $P_0$ that minimises the area functional in eq. \eqref{radishes}. $\pb$ can be determined in the following way (see figure \ref{fig:RTPhases}). One begins by solving for $\zeta_0$ using
$\zeta_0+\zeta_\infty(P_0)=\zeb$ where $\zeta_\infty(P_0)$ is given in eq.~\reef{alphadog}. Then one finds `sample' values of $\pb,\zeta_\mt{B}$ where the extremal surface meets the brane by combining eqs.~\reef{eq:foobar2} and \reef{zetasol} and simultaneously solving
\beqa
 \(1+\pb^2\)\sinh^2\!\zeta_\mt{B}&=&\frac{L^2}{\s^2}\(1-\frac{\s^2}{4L^2}\)^2\,,\nonumber\\
 \zeta_-(\pb;P_0,\zeta_0)&=&\zeta_\mt{B}\,.
 \label{solver3}
\eeqa
This yields $P_B$ as a function of $P_0,\zeta_{\mt{CFT}}$ and $T_o$, and substituting $\pb$ into eq.~\reef{CokeZero} gives the area of the associated extremal surface. Below, we perform this calculation numerically. However, we have not yet considered the boundary conditions \reef{ortho1} in this analysis. Rather than explicitly examining the latter, we simply evaluate the area (or rather the difference $\Delta S$) over the range of possible $P_0$ (with fixed $\zeb,T_o$), as shown in figure \ref{fig:dS0}a. The correct RT surfaces are then identified as the minima in these plots. Further, the examples in the figure illustrate that without the topological contribution, $\Delta S>0$ for all minima and so the disconnected phase dominates, as generally expected. That is, no quantum extremal islands form on the brane in this case. However, as shown in figure \ref{fig:dS0}b, we see that with a sufficiently large topological coupling $\lgb$ one can achieve $\Delta S<0$, where a first order transition leads to the formation of an island. 

Although the above recipe is valid for arbitrary brane tensions, in the limit of very large tension we can approximate the solution analytically. Since, as stated above, the leading contribution to the entropy \eqref{sample} scales as $A(\sigma_\xR)\sim \pb$, the RT surface corresponds to that which has the minimal value of $\pb$. Moreover, since the function $\zeta_{\mt{B}}(P)$ defining embedding of the brane in \eqref{solver3} is monotonically decreasing with $P$, the surface must maximise its hight $\zeta_\infty(P_0)$, which is achieved for $P_0=P_0^{\mt{crit}}$, by definition (see discussion around figure \ref{figzetainfty}). This can be readily checked in figure \ref{fig:dS0}a, where the curves attain a minimum around $\mbox{arctan}(P_0^{\mt{crit}})\approx 0.47$, with a small correction due to the finite terms in \eqref{radishes}, which becomes smaller and smaller as we increase the tension. We shall refer to this solution with $P_0\approx P_0^{\mt{crit}}$ as the \textit{small island}, in order to distinguish it from a second island appearing below which corresponds to a circle with a larger radius.  


%\begin{figure}[h]
%\begin{center}
%\includegraphics[scale=0.3]{images/setup}
%\caption{A half of the geometric setup in cylindrical coordinates, with the radial direction compactified to a finite coordinate value. The `tube' (orange) corresponds to the connected RT surface $\sigma$, anchored at conformal infinity and intersecting the brane (green) at the codim-$3$ surface $\del\sigma_{brane}$ (red). The disk (blue) corresponds to the trivial disconnected phase. A second copy of this is glued along the brane, as depicted in figure \ref{fig:brane2}.  }
%\label{figsetup}
%\end{center}
%\end{figure}

%The total renormalised area of the connected phase is given in eq. \eqref{Acon2}. Notice that the intersection point $\pb=\pb(\s,\zeb,P_0)$ depends on the location of the brane via $\s$, together with the anchoring hight $\zeb$ and the turning point $P_0$ the surface. To find the entanglement entropy, we fix $\s$ and $\zeb$, and vary $P_0$ in order to find the minimum of the area
%\begin{align}\label{dAtilde}
%\Delta \tilde A=S_{\mt{conn}}(T_0> 0)-S_{\mt{disc}}
%\end{align}
%where the first and second term are given by eqs. \eqref{Acon2} and \eqref{Sdisc} respectively. We perform this computation numerically. In figure \ref{figClassAreas} where we plot the area of minimal surfaces that intersect the brane, for fixed anchoring point $\zeb$ as we vary the turning point $P_0$, for different values of $\s$, the parameter controlling the tension of the brane. For large tensions $L/\s\gg 1$, it can be checked that the minimum is always attained for $P_0=\bar P_0\approx 0.44$.


%\begin{figure}
%\begin{center}
%  \begin{subfigure}[b]{0.4\textwidth}
%    \includegraphics[width=\textwidth]{images/ClassAreas}
%    \caption{}
%  \end{subfigure}
%  %
%  \begin{subfigure}[b]{0.4\textwidth}
%    \includegraphics[width=\textwidth]{images/GB_u}
%    \caption{}
%  \end{subfigure}
%  \end{center}
%  \caption{a) Renormalised area from eq. \eqref{radishes} of connected RT surfaces, anchored at $\zeb=0$, with $\lgb=0$. b) Critical value of $\lgb$ such that $\mbox{min} \Delta S<0$.}
%  \label{fig:dS}
%\end{figure}

\begin{figure}[h]
	\def\svgwidth{0.9\linewidth}
	\centering{
		\input{dS2.pdf_tex}
		\caption{Panel a. illustrates the renormalised area from eq. \eqref{radishes} of connected RT surfaces, anchored at $\zeb=0$, with $\lgb=0$. Panel b. is a plot of the critical value of $\lgb$ such that $\mbox{min}( \Delta S)<0$.
		}
		\label{fig:dS0}
	}
\end{figure}

\paragraph{c) $T_o\ne 0;\ 1/\Gbr\ne 0$\ :} Finally, we examine the holographic EE in the presence of a DGP brane. The only difference in this analysis is the additional contribution coming at the intersection of the RT surface with the brane in eq.~\reef{eq:sad}.
In the present setting, this means that we add the following,
\beq\label{sample2}
S_\mt{brane}=\frac{A(\sigma_\xR)}{4\Gbr}=\frac{\pi L}{2\Gbr}\,\pb\,,%\frac{\pi L^2}{\Gbr}\,\pb\,,
\eeq
to the bulk contribution in eq.~\reef{CokeZero}. In fact, the  expansion of $\Delta S$ for $\pb\gg P_0$ takes precisely the same form as in eq.~\reef{radishes}. The only difference is that the induced Newton's constant on the brane is now given by eq.~\reef{Newton33}, \ie $\frac{1}{G_\mt{eff}}=\frac{2\,L}{\Gbk}+\frac{1}{\Gbr}$.

Generally, we might think of $1/\Gbr$ as a positive quantity, and so the DGP contribution \reef{sample2} would simply increase the penalty for having a large $\sigma_\xR$ in the connected phase, and enhance the dominance of the disconnected phase. However, there is no apriori reason why we should not also consider a negative gravitational coupling on the brane,\footnote{For example, integrating out quantum fields on the brane could produce either a positive or negative shift in Newton's constant. In particular, it can be negative for gauge fields or nonminimally coupled scalar fields, as was discussed in the context of EE in \cite{Larsen:1995ax,Kabat:1995eq} -- see further discussion in section \ref{sec:discussion} and appendix \ref{bubble}.}%\dn{Maybe shouldn't put so much emphasis on integrating out business. Talk about counterterms? Or just say we comment in the discussion section?}

in which case the DGP term serves as another mechanism to reduce the penalty for forming an island on the brane. It is this scenario that we will examine further here -- as well as in appendix \ref{bubble}.

It will prove convenient to work with the ratio $\lamb$ introduced in eq.~\reef{newdefs}. Let us recall what parameters are in play. The tension of the brane is controlled by $\s$, which we keep small but finite. The dimensionless ratio between the bulk and brane gravitational constants is controlled by $\lamb$. As discussed above, interesting things happen when $\lamb<0$, which is when $\Gbr<0$ while $\Gbk>0$.

\begin{figure}[h]
	\def\svgwidth{\linewidth}
	\centering{
		\input{IslandPlot.pdf_tex}
		\caption{ Panel a.: Generalised (renormalised) area from eq. \eqref{radishes} as function of $P_0$, for different values of the DGP coupling $\lamb$. Notice the appearance of a `large' island when $\lamb$ approaches $-1$, due to the partial cancellation of the induced and DGP area terms. Panel b. Phase diagram: the black lines correspond to first order phase transitions, while the blue one at $\lamb=-1$ indicates the region where gravity becomes unstable. Both plots are done for fixed $L/\s=100$. 
		}
		\label{fig:dS}
	}
\end{figure}
%\begin{figure}
%\begin{center}
%  \begin{subfigure}[b]{0.5\textwidth}
%    \includegraphics[width=\textwidth]{images/A_gen}
%    \caption{}
%  \end{subfigure}
%  %
%  \begin{subfigure}[b]{0.4\textwidth}
%    \includegraphics[width=\textwidth]{images/GB_B}
%    \caption{}
%  \end{subfigure}
%  \end{center}
%  \caption{ a) Generalised (renormalised) area from eq. \eqref{radishes} as function of $P_0$, for different values of the DGP coupling $\lamb$. Notice the appearance of a `large' island when $\lamb$ approaches $-1$, due to the partial cancellation of the induced and DGP area terms. b) Phase diagram: the black lines correspond to first order phase transitions, while the blue one at $\lamb=-1$ indicates the region where gravity becomes unstable. Both plots are done for fixed $L/\s=100$. }
%  \label{fig:dS}
%\end{figure}
Using the same approach described above, we can explore the transition between the connected and disconnected phases numerically. In figure \ref{fig:dS}a, we plot $\Delta S$ as function of $P_0$ for a fixed $\zeb=0.095,L/\s=100$ and $\lgb=0$, for different values of $\lamb$. These plots are analogous to those presented in figure \ref{fig:dS}a where $\lamb=0$ (but $L/\s$ is varied). Again, these plots are made in lieu of a detailed examination of the boundary conditions where the RT surfaces meet the brane, rather the correct boundary conditions \reef{ortho1} will be acheived where $P_0$ is tuned to produced an minimum in these plots. For small $\lamb$ the curves show a single minimum but $\Delta S>0$, indicating that the disconnected solution dominates in this case. As $\lamb$ becomes more negative, the curves are pulled down and eventually $\Delta S$ enters the negative region so that the connected solution becomes the dominant saddle point. This behaviour is as expected but we note that $\lamb$ is very close to $-1$ in this regime, which according to eq.~\reef{newdefs} means there is almost a complete cancelation between the induced gravitation coupling $1/G_\mt{RS}$ and the DGP term $1/\Gbr$. Of course, this near cancellation is alleviated by turning on the topological coupling $\lgb$, as shown in figure \ref{fig:dS}b. 

Another interesting feature shown in figure \ref{fig:dS}a is the appearance of a second minimum in the curves. This second solution occurs at a larger value of $P_0$ and also of $P_B$, and corresponds to a larger circle $\sigma_\xR$ on the brane, and therefore we refer to it as a \textit{large island}. The existence of this second island is due to the finite terms in \eqref{radishes}. Indeed, these terms are essentially what is plotted in figure \ref{figdeltaA}, and they are unbounded from below for large $P_0$. Therefore, when $\lamb$ becomes sufficiently negative as to produce a significant cancellation between the induced and DGP gravitational entropies, there is a new competition, now between $A(\sigma_\xR)/4G_\mt{eff}$ and the finite terms, producing the large island. As $\lamb\to-1$, the minimum rolls down to infinity ($P\to \infty,\Delta S_{\mt{gen}}\to-\infty$), indicating an instability at this point, which we explore further in appendix \ref{bubble}.

Figure \ref{fig:dS}b summarises the phase diagram of the system, for a fixed value of the tension $L/\s=100$, as we vary both the DGP coupling $\lamb$ and the topological coupling $\lambda_{\mt{GB}}$. The lines between no/small/large islands correspond to first order phase transitions, while the blue line at $\lamb$ indicates the region where the theory becomes unstable. 




==> sections/bubblesA.tex <==
% !TEX root = ../lifeonbrane3.tex
%





%\subsection{`Bubbles' on the brane}\label{bubblesX}


In this closing section, we consider a simple but surprising class of RT surfaces. In particular, we show below that there are closed extremal surfaces with the topology of a sphere, \ie $S^{d-1}$ in the locally AdS$_{d+1}$ bulk geometry. In empty AdS space, one could consider such spherical surfaces, but their area would be extremized when they collapse to zero size. In the present case, we will show that in certain situations, the spherical RT surfaces can be supported at finite size by the brane.  To illustrate the situation, we continue with the special case of $d=3$ as in the previous section, and afterwards comment on the situation with general $d$. 
%
\begin{figure}[h]
\begin{center}
\includegraphics[scale=0.2]{images/bubble}
\caption{One half of an RT bubble supported on the brane. \rcm{Lets illustrate this in the `style' of figure \ref{fig:EWs}.}}
\label{figbubble}
\end{center}
\end{figure}

Consider the geometry illustrated in figure \ref{figbubble}. On either side of the brane, we have a disk satisfying $\zeta=$constant, \ie satisfying eq.~\reef{zetap} with $P_0=0$. Hence locally these surfaces extremize the entropy functional \reef{area} in the bulk. However, rather than extending out to the asymptotic boundary, as shown in the figure, the two disks intersect the brane and meet at some radius $\pb$.  Hence this RT surface has the topology of a sphere and we use the nomenclature `bubble' to describe these surfaces. For $d=3$, the generalised entropy \reef{eq:sad} of this bubble is
\begin{align}\label{Agenbubble}
\sgen&=\frac{\pi L^2}{\Gbk} \left(  \sqrt{1+\pb^2}-1  + \lamb\, \pb \right) +2\,\lgb 
\end{align}
with $\lamb$ defined in eq. \eqref{newdefs}. We have also included the topological term introduced in eq.~\reef{Euler3}.
%It also illuminating to contrast this with the formula for the effective gravitational constant on the brane, eq.~\eqref{Newton33}, which can be rewritten in terms of $\lambda$ as
%\begin{align}\label{Gefflambda}
%\Geff=\frac{\lambda}{1+\lambda}\Gbr
%\end{align}
%\rcm{see instead eq.~\reef{Newton34}.}

Extremizing eq.~\reef{Agenbubble} with respect to the radius of the bubble, we find
\beq\label{gamdot}
\partial_{\pb}\sgen=0 \qquad
\implies\qquad \frac{\pb}{\sqrt{1+\pb^2}}=-\lamb=-\frac{\Gbk}{2L\,\Gbr}\,.
\eeq
Now recall that we will always have $\Gbk>0$, but considered the possibility of $\Gbr$ becoming negative in the previous section. But let us first consider the case $\lamb\ge 0$, which implies $1/\Gbr\ge 0$. In this case, we can not satisfy eq.~\reef{gamdot} or rather both the bulk and brane contributions to the generalised entropy \eqref{Agenbubble} are positive monotonically increasing functions of $\pb$, and therefore the minimum lies at $\pb=0$, \ie where the bubble collapses to zero size -- see figure \reef{figAbubble}. 

Further, we might comment that for large $\pb$, the leading contribution in eq.~\reef{Agenbubble} takes the expected form
\beq\label{expect4}
\sgen\simeq =\frac{A(\sigma_\xR)}{4G_\mt{eff}} +\cdots \qquad{\rm where}\ \ \ \frac{A(\sigma_\xR)}{4G_\mt{eff}}=\frac{\pi L^2}{\Gbk}\,(1+\lamb)\,\pb\,,
\eeq
just as in eq.~\reef{radishes}. That is, \rcm{******}


Of course, the more interesting scenario is when $\lamb$, and hence
$1/\Gbr$, are negative. Then eq.~\reef{gamdot} has the solution
\begin{align}
\pbo=-\frac{\lamb}{\sqrt{1-\lamb^2}}\,,
\label{cookie}
\end{align}
for which the generalized entropy \reef{Agenbubble} becomes
\begin{align}\label{Sbubble}
\sgen= \frac{\pi L^2}{\Gbk} \left( \sqrt{1-\lamb^2} - 1 \right)+2\,\lgb 
\end{align}
We note that these expressions are only sensible for $-1<\lamb<0$. In fact, for $\lamb<-1$, there is no minimum for the generalized entropy \reef{Agenbubble}, \ie there is no solution for eq.~\reef{gamdot}, and rather $\pb$ runs off to infinity -- see figure \reef{figAbubble}.  This is, perhaps, not so surprising since we can see from eq.~\reef{Newton34} that this regime is pathological, with the graviton localized on the brane becoming a ghost.

Therefore we only consider the regime $-1<\lamb<0$ where eqs.~\reef{cookie} and \reef{Sbubble} apply. As illustrated in figure \reef{figAbubble}, eq.~\reef{cookie} is indeed the global minimum of the generalized entropy \eqref{Agenbubble}. We might note that the sum of the first two terms in eq.~\reef{Sbubble} is negative. That is, the combined contributions of the two area terms in eq.~\reef{eq:sad} is in fact {\it negative!} Hence we only get a sensible (\ie positive) result for the generalized entropy \reef{Agenbubble} with the inclusion of the topological term \reef{Euler3}, which was also favoured in section \ref{sec:examples}.


\begin{figure}[h]
\begin{center}
\includegraphics[scale=0.4]{images/Abubble}
\caption{The generalised area \eqref{Agenbubble} for a bubble as a function of its radius. For $\lambda>0$, the area is minimal for vanishing size, whereas for $-1<\lambda<0$ it has a finite size. For $\lambda<-1$, there is no global minimum, signalling an instability of the system. }
\label{figAbubble}
\end{center}
\end{figure}

\begin{align}\label{genbubble1}
S_\mt{gen}=\frac{L^{d-1}\,\Omega_{d-2}  }{2(d-1)\Gbk}\,P^{d-1}\, {}_{2}F_1\left[ \frac{1}{2},\frac{d-1}{2},\frac{d+1}{2},-P^2 \right]+\frac{L^{d-2}\, \Omega_{d-2}}{4\Gbr}\,P^{d-2}
\end{align}
\vc{From
\begin{align}
  \hyperF\left(
  \frac{1}{2},
  \frac{d-1}{2},
  \frac{d+1}{2},
  -P^2
  \right)
  \sim\begin{cases}
  1 & \text{if $P\ll 1$}
  \\
  \frac{d-1}{d-2}\frac{1}{P} &\text{if $P\gg 1$}
\end{cases}
\label{eq:bubblegum}
\end{align}
we see that the bulk contribution, for small $P$, is extensive, and for large $P$, is dominated by a term identical to the QES area term in \eqref{genbubble1} with $1/G_\brane$ replaced by the induced $1/G_\eff |_{1/G_\brane=0}$ given in \eqref{Newton2}. Note that performing a large $P$ expansion in the hypergeometric function \eqref{eq:bubblegum} is equivalent to the process of extracting the `divergent' entropy piece described around \eqref{eq:apple} --- in \eqref{genbubble1}, $G_\bulk$ is written in terms of $c\sim L^{d-1}/G_\bulk$ and $P$ is rescaled by $L$ to obtain a dimensionful coordinate, then a small $L$ expansion is performed. However, the extremal condition $\partial_P S_\gen =0$ can in fact be solved exactly for any $d$ as
\beq\label{amazing}
  \partial_P S_\gen
  = \frac{L^{d-1}\Omega_{d-2}}{2 G_\bulk} P^{d-3}\left(
  \frac{P}{\sqrt{P^2+1}} + \lambda
  \right)
\eeq
with the parenthesized factor vanishing at the radius \eqref{eq:cookie}.
}


To gain an intuitive understanding of bubbles from the brane's perspective, it is helpful to rewrite \eqref{Agenbubble} in the following suggestive form:
\begin{align}
  S_\gen
  =& \frac{\area}{4 G_\eff} + S_\ren.
  \label{eq:pear}
\end{align}
Here,
\begin{align}
  \frac{\area}{4 G_\eff}
  =& \frac{\area}{4 G_\brane} + S_\dive
\end{align}
is a sum of the bare area term (scaled by the bare Newton's constant of the brane),
\begin{align}
  \frac{\area}{4 G_\brane}
  =& \frac{\pi L P}{2 G_\brane}
  = \frac{\pi L^2 \lambda P}{G_\bulk}
  \label{eq:cucumber}
\end{align}
and the `divergent' part
\begin{align}
  S_\dive
  =& \frac{c \area}{L}
  = \frac{\pi L^2 P}{G_\bulk},
  &
  c \equiv& \frac{L^2}{2 G_\bulk}
  \label{eq:apple}
\end{align}
of the CFT entropy
\begin{align}
  S_\CFT
  =& S_\dive + S_\ren
  \label{eq:banana}
  \\
  S_\ren
  =& 2\pi c(\sqrt{1+P^2}-1-P)
  = \frac{\pi L^2(\sqrt{1+P^2}-1-P)}{G_\bulk}.
  \label{eq:orange}
\end{align}
To identify the terms introduced here, we first subtracted the bare area term \eqref{eq:cucumber} from \eqref{Agenbubble}, leaving the bulk area of the RT surface. We identify the latter as the entropy \eqref{eq:banana} of the matter CFT. To separate out the `divergent' contribution \eqref{eq:apple}, we invoke the usual holographic proportionality $G_\bulk \propto L^{d-1}/c$ (here $d=3$) between the bulk Newton's constant and the CFT central charge, temporarily remove $P$ in favour of a dimensionful coordinate $\tilde{P}\equiv P L$, and expand in $L$. This is because the displacement of the brane from the AdS boundary sets a UV cutoff in the brane theory at a proper length scale of $L$ (as measured by the induced metric). For $d>3$, divergent terms other than the area term are also expected to make an appearance. We collect the remaining `finite' contribution to the CFT entropy in $S_\ren$ given in \eqref{eq:orange}.


\subsection{Wormholes and Cutoffs}\label{wormy}

\rcm{old words:} These bubbles are a remnant of replica wormholes in the limit $n\to1$. What are lessons that we learn? Note that it is important that the wormholes depend on the quantum contributions of the matter fields. Hence they do not exist on their own, \ie they need to be anchored by a twist operator on the boundary.
What are the implications for the new discussions of baby universes and ensembles??

Having written the generalized entropy of the bubble in the form \eqref{eq:pear}, it becomes evident that bubbles can only form at sizes where quantum effects become significant. In particular, note that the renormalized area term $A/4 G_\eff$, being monotonically increasing with bubble size, is alone insufficient to support bubbles. Bubbles can only favourably form when $S_\ren$ is negative and larger than $A/4 G_\eff$. We see from \eqref{eq:orange} that $S_\ren$ is indeed negative. Even so, to have this `quantum' piece compete with the `classical' area term $A/4 G_\eff$, one ordinarily require system sizes at most on the Planck scale $A\lesssim G_\eff$ which invalidates the treatment of QFT in semiclassical gravity. However, as we have many $c\gg 1$ degrees of freedom in our matter CFT, $S_\ren \sim c \sim L^2/G_\bulk$, it becomes possible for $S_\ren$ to compete with $A/4 G_\eff$ for system sizes $A\lesssim c G_\eff \sim L^2 G_\eff/G_\bulk$. Should the bare constant $1/G_\brane$ be chosen to largely cancel against $L/2G_\bulk$, \ie $\lambda>-1$ be chosen close to $-1$, this upper bound $A\lesssim L (1+\lambda)^{-1}$ can be well above the Planck scale. In fact, the bubble size $P \lesssim (1+\lambda)^{-1}$ we do find in \eqref{eq:cookie}, can be made parametrically large compared to the Planck scale $P\sim G_\eff/L$.



\rcm{More old words:} It seems that as soon as $1/G_\mt{brane}$ is slightly negative, that the brane supports RT surfaces which are closed spheres, \ie bubbles. This suggests that the {\it vacuum} state now has a finite entanglement entropy, \ie the vacuum is a mixed state -- seems like an inconsistency. Further one should be able to place the bubble anywhere on the brane, \ie it need not be positioned at the center of the geometry (but this simplifies the calculation). What would this new zero-mode mean?

For $-1<\lamb<0$, the bubbles are stable, and for $\lamb<-1$, they are unstable and become infinitely large.

\rcm{Still not sure what to do with this. See following comments:}
Note that integrating out quantum fields on the brane can produce either a positive or negative shift in Newton's constant. In particular, it is found to be negative for gauge fields \cite{Larsen:1995ax,Kabat:1995eq}. There is a tension between this negative renormalization interpreting the contribution to the entanglement entropy which `should always be positive.' I believe this puzzle was resolved in terms of edge modes by \cite{Donnelly:2014fua,Donnelly:2015hxa}. In principle, there is a similar puzzle for non-minimally coupled scalars \cite{Larsen:1995ax}, which was resolved (perhaps implicitly) in \cite{Faulkner:2013ana}.

I believe similar bubbles appear in the AdS vacuum when considering HEE for Gauss-Bonnet gravity (with an appropriate sign of the curvature-squared coupling). However, in this case, we would just say that these are spurious solutions, \eg the curvature-squared term is competing with the Einstein term in an essential way. Can we argue analogously here?


==> sections/details.tex <==
% !TEX root = ../lifeonbrane3.tex
%



We will give some detailed calculations which show how the change in bulk parameters is related to changes in the brane/boundary picture. For simplicity, we consider the case of a Poincare patch with a time-like co-dimension one defect which passes through the origin. The defect breaks the conformal symmetry from $SO(d,2)$ to $SO(d-1,2)$.

\subsection{Interface OPE expansion in holography}
An operator in the CFT has an expansion in terms of operators living at the interface. If we denote by $x$ the direction perpendicular to the brane and by $y$ the direction along the brane, we have that
\begin{align}
    O_{\Delta}(x,y) = \sum_{\Delta'} c_{O_{\Delta}O_{\Delta'}} \frac{O_{\Delta'}(y)}{|x|^{\Delta - \Delta'}}.
\end{align}
We will now discuss how this expansion is realized holographically. To this end we choose AdS slicing coordinates
\begin{align}
    ds_{AdS_{d+1}}^2 = \frac{L^2}{\sin^2 \theta}(d\theta^2 + ds_{AdS_d}^2).
\end{align}
The boundaries are located at $\theta = \pm \pi$.
As mentioned above, we will for simplicity assume that $ds_{AdS_d}^2$ is the AdS metric in Poincare coordinates,
\begin{align}
    ds_{AdS_d}^2 = \frac{dx^\mu dx_\mu + dz^2}{z^2}
\end{align}
Consider a scalar field of mass $m$. We will make a the ansatz
\begin{align}
    \phi(x,z,\theta;p) = e^{i p x} \psi(z) f(\theta).
\end{align}
The equation of motion then yields
\begin{align}
    \psi(z) \left(f''(\theta )-(d-1) \cot (\theta ) f'(\theta )\right)\\
    +f(\theta ) \left(z \left(-(d-2) \psi'(z) +z \psi''(z)-z \psi(z) p^2\right)-m^2 \psi(z) \csc ^2(\theta )\right) = 0
\end{align}
We need to solve
\begin{align}
    z \left(-(d-2) \psi'(z)+z \psi''(z) - z \psi(z) p^2 \right)=\lambda  \psi(z).
\end{align}
This is the $z$ dependent part for the equation of a scalar field on AdS$_d$ with mass-squared $\lambda$. As we will see immediately, this means that $\lambda$ is bounded from below by the Breitenlohner-Freedman bound, $\lambda \geq - (\frac{d-1}{2})^2$. As is well known, the general solution can be expressed in terms of Bessel functions,
\begin{align}
    \psi(z) = c_1 z^{\frac{d-1}{2}} J_{\frac{1}{2} \sqrt{d^2-2 d+4 \lambda +1}}\left(z \sqrt{-p^2}\right)+c_2 z^{\frac{d-1}{2}} Y_{\frac{1}{2} \sqrt{d^2-2 d+4 \lambda +1}}\left(z \sqrt{-p^2}\right).
\end{align}
The equation for $f(\theta)$ then becomes
\begin{align}
\left(f''(\theta )-(d-1) \cot (\theta ) f'(\theta )\right)+f(\theta ) \left(\lambda - m^2 \csc ^2(\theta )\right)=0
\end{align}
with solutions
\begin{align}
    \left( c_1 P_{\frac{1}{2} \left(\sqrt{d^2-2 d+4 \lambda +1}-1\right)}^{\frac{1}{2} \sqrt{d^2+4 m^2}}(\cos (\theta ))+c_2 Q_{\frac{1}{2} \left(\sqrt{d^2-2 d+4 \lambda +1}-1\right)}^{\frac{1}{2} \sqrt{d^2+4 m^2}}(\cos (\theta ))\right)\left(\sin ^2(\theta )\right)^{d/4},
\end{align}
where $P$ and $Q$ are Legendre functions. Note that $\lambda$ has not been fixed yet, so we have two continuous families of solutions. We will see in a bit that by carefully considering the situation at the bulk dual of the defect, $\lambda$ will be quantized. The defect operators will then be given as the dual operators to the $d$-dimensional fields $\psi[z]e^{ipx}$.


The Legendre functions are somewhat hard to work with, since for generic mass both solutions diverge as $\theta \to - \pi$ and only a particular linear combination forms the normalizable modes. It would therefore probably be useful to re-express them in terms of hypergeometric functions. We will not do this here, however, but continue discussing a special case in which $P$ becomes the normalizable mode. This happens for $m=0$, a massless field in the bulk.

In the case discussed in this paper, we have two copies of the spacetime between the boundary and the brane, which are identified along the brane. Since the asymptotic boundary is compact it is clear that the bulk modes must be quantized and in fact, it is well known that requiring regularity of the normalizable mode in the bulk in global AdS imposes a quantization condition on the bulk modes. By $\mathbb Z_2$ symmetry of the setup, we know that all modes are either even or odd under reflection across the brane. Without any additional sources added, the solution for a scalar field is is regular everywhere.\footnote{We will revisit this assumption below.} The even modes have vanishing normal derivative at the brane, while the odd modes vanish at the brane. We must also impose this condition on our solutions. This condition quantizes $\lambda$. The exact value must be determined numerically, however for simple cases, it can also be done analytically.

\paragraph{Example. } Let us take $x=0$ as the defect, i.e., we do not introduce a defect, but simply pretend that $x=0$ is a special place. The defect OPE then becomes simply the Taylor expansion of an operator around $x=0$. For a generalized free fields we have that the conformal family simply consists of derivatives of the operators, i.e., operators or dimensions $\Delta' = \Delta + n$. The relation between $\lambda$ and $\Delta'$ is 
\begin{align}
    \lambda = \Delta'(\Delta'-(d-1)).
\end{align}
In the case at hand we assumed a massless scalar field, so $\Delta = d$. The correct boundary condition is Dirichlet conditions at both boundaries. One can confirm explicitly by a numerical computation, that the quantization condition yields
\begin{align}
    \lambda = (d+n)(n+1).
\end{align}
In the case we present in the paper, we need to focus on even modes, since only those induce dynamical fields on the brane.

\subsection{Bound states and mode counting}
What happens if we introduce a defect and couple bulk fields to it? Before we answer this question, let us consider a somewhat simpler situation, namely that of a Randall--Sundrum brane. The aim of this section is to understand under which conditions bound states appear and which other modes we have to integrate out in order to obtain an effective theory for such modes. Other questions are about the number and orthogonality of modes. Lastly, we are interested in the holographic dictionary for the effective theory on the RS brane. 

We will take AdS in Poincare coordinates and consider a scalar field. The ansatz for the wavefunction reads
\begin{align}
    \psi(t,\vec x,z) = \iint d\omega d\vec p \; c_{\omega p }\; e^{i \omega t + i \vec p \vec x} f(z;p,\omega).
\end{align}
Using this, we want to solve the equations of motion in $d+1$ dimensions,
\begin{align}
    z^2 f''(z;p,\omega) - z (d-1) f'(z;p,\omega) + z^2 (-\omega^2 + p^2) f(z;p,\omega) + m^2 f(z;p,\omega) = 0.
\end{align}
The solutions are well known and given in terms of a linear combination of Bessel functions,
\begin{align}
    f(z;p,\omega) = c_1 z^{\frac{d}{2}} J_{\frac 1 2 \sqrt{d^2 - 4m^2}}(k z) + c_2 z^{\frac{d-1}{2}} Y_{\frac 1 2 \sqrt{d^2 - 4m^2}}(k z),
\end{align}
with $\omega^2 - p^2 = k^2$. If $\frac 1 2 \sqrt{d^2 - 4m^2}$ is not integer, we could have replaced $Y_{\frac 1 2 \sqrt{d^2 - 4m^2}}(k z) \to J_{-\frac 1 2 \sqrt{d^2 - 4m^2}}(k z)$ to obtain another set of linearly independent functions. Both, $Y_\alpha(k z)$ and $J_\alpha(kz)$ diverge as $z \to 0$, where the asymptotic boundary is located. Since we do not intend to turn on sources we drop those solutions and are left with $J_\alpha$. It obeys the identity
\begin{align}
    \int_0^\infty x J_{\alpha}(ux) J_{\alpha}(vx) dx = \frac 1 u \delta(u-v),
\end{align}
which we can use to normalize the solutions. The reason is that this integral takes the same form as the Klein Gordon norm along the $z$-direction.
\begin{align}
    \sim \int dz z^{-d+1} (\psi_1 \partial_t \psi_2 - \psi_2 \partial_t \psi_1).
\end{align}
Note that if we require regularity of the solution, we also have that $k^2 > 0$.

We now introduce a Randall--Sundrum brane at $z = z_*$. In order to understand how different boundary conditions change the number of modes, consider first the case where we impose Dirichlet conditions at the brane. It is clear already that now $k$ will be quantized. At leading order, the large $z$ expansion of $J_\nu$ is
\begin{align}
    J_\nu(k z) = \sqrt{\frac{2} {\pi k z}} \cos(k z - \frac 1 2 \nu \pi - \frac 1 4 \pi).
\end{align}
Clearly, for $k z_* \gg 1$ the zeroes are at 
\begin{align}
    k = \frac{\pi}{z_*} (n + \frac 1 2 \nu - \frac 1 4).
\end{align}
How does this change if we introduce non-trivial boundary conditions at the brane? In analogy with the gravitational case, let us pick Robin boundary conditions,
\begin{align}
    \phi'(z_*) = c \phi(z_*).
\end{align}
It is important that our boundary condition takes this form (as opposed to, say, $\phi'(z_*) = c \phi(z_*)$), since otherwise a linear combination of solutions would not be a solution anymore. Using the large $z$ expansion, we find that (assuming $c \geq \mathcal O(1)$)
\begin{align}
   \sin(k z_* - \frac 1 2 \nu \pi - \frac 1 4 \pi) = -\frac{c}{k} \cos(k z_* - \frac 1 2 \nu \pi - \frac 1 4 \pi).
\end{align}
The key point is that the modes are spaced at order $\frac 1 {z_*}$ and changes in the spectrum for a range of modes of $\Delta k < \mathcal O(1)$ (these are still order $z_* k$ modes) can be neglected. In other words: the spectrum changes with respect to the one with Dirichlet boundary conditions, but only very mildly.
\\
\\
Open question: What happens for $k z_* \sim \mathcal O(1)$?
\\
\\
Crucially, thanks to the modified boundary condition, a new state appears with $k^2 < 0$. The relevant solution is $I_\nu(k z)$. at large $k z$ this takes the form
\begin{align}
    I_\nu(k z) \sim \frac{e^{kz}}{\sqrt{2 \pi k z}}.
\end{align}
Clearly, this could never satisfy a Dirichlet boundary condition $\phi = 0$ at large $z_*$, but the Robin condition becomes at leading order
\begin{align}
    k = c.
\end{align}

In order to compare the effects, we should normalize the modes. The bound state very roughly has a norm of
\begin{align}
    \int dz z{^-d} e^{2 k z} \sim \frac{e^{2 k z}}{z^{d-1}}, 
\end{align}
so that to properly normalized wave function in the large $kz$ limit roughly becomes 
\begin{align}
   \psi \sim z_*^{\frac{d-1}{2}}\frac{e^{k(z-z_*)}}{\sqrt{2 \pi k z}}.
\end{align}
The positive energy states are roughly normalized and thus we see that evaluated at the brane, the bound state is bigger by a factor of $\sim z_*^{\frac{d-1}{2}}$.

At the asymptotic boundary, we have that
\begin{align}
    J_\nu(kz) \sim (\frac 1 2 kz)^\nu \Gamma(\nu + 1)^{-1} \\
    \psi \sim z_*^{\frac{d-1}{2}} e^{-k z_*} (\frac 1 2 kz)^\nu \Gamma(\nu + 1)^{-1}.
\end{align}
As a result of the normalization, we see that the bound state is exponentially suppressed. We conclude that by integrating out all KK modes, we produce the CFT at the asymptotic boundary together with a scalar field on the brane. However, both, the CFT at the asymptotic boundary as well as the theory on the Randall-Sundrum brane are only effective theories. The corrections to the theory on the RS brane are a power-law in the coordinate distance of the RS brane to the asymptotic boundary, while the corrections to the CFT are exponentially small.

For massless particles we expect that $k\sim 0$ and it is unclear how much of the above analysis still holds.


\subsection{The CFT on the brane}
Let us consider a fixed time, e.g. $t=0$. The bulk modes can be classified into even and odd modes under the $\mathbb Z_2$ symmetry coming from reflecting the system at the brane. A certain linear combination of even and odd modes only has support on one side of the brane, while the orthogonal linear combination has support on the other side. Furthermore, all odd modes vanish on the brane and only even induce fields.

It should be clear from the preceding section that the acceptable values of $\lambda$ and thus also the defect operator spectrum is determined by the location of the brane. Let us assume that we locate the brane very close to $\theta = \pi$. Imposing Neumann boundary conditions at the brane, one can easily see that the allowed values for $\lambda$ are very close to the allowed values for $\lambda$ had we simply quantized AdS without a brane. This means that the OPE spectrum coming from one side of the brane looks very much like the one of a CFT with a ``fake defect'' as discussed in the example above. This suggests that the theory on the brane has approximately the same light spectrum as the CFT on the asymptotic AdS boundary. Since there are theories on either side of the brane, the brane carries a second copy of the theory.

The operators of the brane CFT are given by the limiting value of the bulk fields. Let's say the brane is placed at $\epsilon_{UV} \equiv \epsilon$. We can calculate correlation functions of brane operators $\bar {\mathcal O} = \epsilon^\Delta \bar \phi$ on the brane by introducing a source to the bulk Lagrangian,
\begin{align}
    \dots + \int_{\partial} \bar J \bar {\mathcal O}.
\end{align}
Adding this term changes the Neumann boundary condition of the bulk field $\phi$ from $n \cdot \nabla \phi = 0$ to $(n \cdot \nabla \phi - J) = 0$. We thus see that in the holographic dictionary of the brane theory, the role of sources is played by the Neumann boundary condition (as opposed to Dirichlet conditions at the asymptotic AdS boundary). Correlation functions can also simply be calculated by using a modified version of the extrapolate dictionary, where we do not divide out by $z^\Delta$, but include this factor into the definition of the operators. This factor is precisely what gives the induced field its scaling dimension. If we are interested in calculating correlation functions between CFT operators and operators on the brane, the easiest way should be by just using the extrapolate dictionary.

\subsection{Adding DGP terms}
We can add additional terms to the brane, which as we will now see change the bulk solution, change the dynamics of the brane theory, and modify the defect CFT.
\subsubsection{Scalar fields}
The simplest term we can add to the brane is a source term
\begin{align}
    S_{DGP} = -\alpha \int \bar \phi,
\end{align}
where $\bar \phi$ is the induced field on the brane. This modifies the background solution, but not the equation for fluctuations around the solution. The reason is clear: Any contribution to the equations of motion of fluctuations around the classical solution must be at order $\mathcal O(\delta \phi^2)$, but the term discussed here vanishes at this order. However, what does change is the classical solution and with it the vacuum expectation value of $\mathcal O$, the operator dual to the field $\phi$. The reduced conformal invariance allows scalar one-point functions of the form 
\begin{align}
    \langle \mathcal O \rangle = \frac a {|x|}
\end{align}
and such a term is turned on by coupling $\phi$ linearly to the brane.\footnote{I have not calculated the exact coefficient.} As mentioned already above, it now becomes clear that a minimal coupling of scalar fields to the brane does change the background, but is not sufficient to create a bound state on the brane. For this to happen, we must try harder.

The next term we will discuss takes the form of a kinetic term
\begin{align}
    S_{DGP} = - \frac 1 2 \int (\partial \bar \phi)^2 + \bar m^2 \phi^2.
\end{align}
If we vary the action, this contributes an extra term to the equations of motion.
\begin{align}
    \Box \phi + \frac{\delta(\theta - \theta_B)}{\sin^2 \theta_B} (\bar \Box - \bar m^2) \bar \phi = 0.
\end{align}
If we expand $\phi$ in eigenfunctions of the D'alembert operator along the brane as before, we obtain for a mode with eigenvalue $\lambda$
\begin{align}
    \Box \phi_\lambda(\theta) + \frac{\delta(\theta - \theta_B)}{\sin^2 \theta_B}  (\lambda - \bar m^2) \bar \phi_\lambda = 0.
\end{align}
Thus, we note that a kinetic term induces a source term, which depends on the mode we are considering. Integrating this equation around $\theta_B$ will give a discontinuity in the first derivative of the field at the location of the brane
\begin{align}
    (\bar \phi'_{\lambda,L} - \bar \phi'_{\lambda,R}) +  (\lambda - \bar m^2) \bar \phi_\sigma = 0.
\end{align}
For the $\mathbb Z_2$ even solution we find
\begin{align}
        2 \partial_\theta \log \bar \phi_{\lambda} +  (\lambda - \bar m^2) = 0,
\end{align}
which quantizes $\lambda$, now however as a function of the brane location, $\bar m$ and $\lambda$ itself. Note that those terms essentially are Robin bounday conditions. The mass-term changes the boundary condition universally, while the kinetic term changes it for different modes. This discussion only affects the modes which previously had Neumann boundary conditions. The modes with Dirichlet conditions at the location of the brane are unaffected, since the source term vanishes.


The action for fluctuations $\psi$ around this solution obtains two additional terms.
\begin{align}
    \dots + \int (\bar \Box \bar \phi - \bar m^2 \bar \phi ) \psi - \frac 1 2 \int (\partial \psi)^2 - \bar m^2 \psi^2
\end{align}
It is thus easy to see that $\psi$ is also sourced and that the equations of motion for $\psi$ might allow a bound-state close to the brane.
This means, amongst other things, that the normal derivative at the brane changes which induces a change in the operator spectrum.


\subsubsection{The gravitational field}
Since the gravitational field is non-linear, the situation is slightly richer here. As discussed above, adding a simple tension term to the brane,
\begin{align}
    S_\text{brane} = - T \int \sqrt{|h|}, 
\end{align}
warps spacetime. In the case of the $\mathbb Z_2$ quotient of our setting, this can also be interpreted as moving the brane closer to (or further away from -- depending on the value of $T$) the second asymptotic boundary. Before tackling the global AdS situation we are considering, let us look at the analogous situation in Randall-Sundrum. There, metric fluctuations around this background obey an equation of the form
\begin{align}
    \left[\frac{-m^2}{2} e^{2 k |y|} - \frac 1 2 \partial_y^2 - 2 k \delta(y) + 2 k^2 \right] \psi(z) = 0.
\end{align}
Here, we just used their notation in which metric fluctuations can be split into contributions orthogonal and transverse to the brane directions, $h(x,y) = \psi(y) e^{ipx}$, $p^2 = m^2$ and $k$ is a parameter in their solution which controls the ratio between the bulk cosmological constant and the brane tension, $k^{-1} \sim L^2 G_\text{bulk} T_\text{brane} \sim \frac 1 L$. The relation between those parameters is a special feature of the Randall-Sundrum model.

An important observation is that the appearance of the $\delta$ function term is responsible for the support of a bound state. The shape of the wave function is controlled by $\frac{e^{k|y|}}{k}$, where $y=0$ is the location of the defect, and so we see that small $k$ means the bound state is wider. Note that in this case, larger $T_\brane$ means a wider bound state. The reason is that the Randall-Sundrum solution does not allow to fix $G_\mt{bulk}$ and $L$ while changing $T_\brane$.

Consider now the case where we have added an additional Einstein-Hilbert DGP term to the action of our brane. Note that we are in the bulk picture, where we have not intergrated out the directions orthogonal to the brane. The variation of the action obtains a new source-term
\begin{align}
    \int\sqrt{h}(\frac{G_{ab}}{16 \pi G_\brane}   - \frac 1 2 T h_{ab} + \frac 1 2 \Delta T h_{ab}) \delta h^{ab}.
\end{align}
In order not to change the brane position, we have that 
\begin{align}
     G_{ab} = - 8 \pi G_\brane \Delta T h_{ab}. 
\end{align}
In the RS scenario, $\Delta T =0$, since the location of the branes is independent of the brane tension. 
Let us now look at fluctuations around this background. The relevant terms appear at second order in the above equation. Recall that the factor $k$ which determines the width of the bound state is proportional the the tension $T$. The question now is whether the other two terms we introduced (and fixed by making them cancel) modify $k$. The relevant contributions come from the second order expansion of the brane action. We get the relevant second order terms by looking at the first-order contribution from 
\begin{align}
    \delta(\frac{G_{ab}}{16 \pi G_\brane}),
\end{align}
which however are just the linearized field equations. We find\footnote{http://www.physics.fau.edu/~cbeetle/PHY6938.07F/linearized.pdf} that for zero modes, i.e., those which obey Einsteins equations, the linearized equations also cancel and clearly, even for zero mode fluctuations, there is no additional contribution at the location of the brane. However, for KK modes a coupling 
\begin{align}
 - \frac{m^2}{32 \pi G_\brane}
\end{align}
is generated.



To get closer to our situation, imagine that the theory on the brane was not on a flat, but on an AdS background. In this case we would need to add an additional $\Delta T$-term. The metric on the brane obeys
\begin{align}
\delta G_{ab} = \frac 1 2 \frac{(d-1)(d-2)}{\ell_B^2} h_{ab}.
\end{align}
Fluctuations $\delta h_{ab}$ around that background obey
\begin{align}
\delta G_{ab} = \frac 1 2 \frac{(d-1)(d-2)}{\ell_B^2} \delta h_{ab},
\end{align}
where $\delta G_{ab}$ is evaluated on the AdS background. The quantity $\ell_B$ is determined by the choice of $T_0$. To add DGP terms, we modify the action by
\begin{align}
\Delta I_\brane = \frac 1 {16 \pi G_\brane} \int \sqrt h R + \int \sqrt h \Delta T.
\end{align}
Here, we finally added a $\Delta T$ which is fixed by the requirement that $\Delta I_\brane$ does not modify the location of the brane. In order to ensure this, we require $\delta \Delta I_\brane = 0$, which fixes
\begin{align}
\Delta T = \frac{(d-1)(d-2)}{16 \pi G_\brane \ell_B^2}.
\end{align}
Let us now consider bulk fluctuations. Their leading order action is given by expanding the bulk action including brane terms to second order in the fluctuations. However, the DGP-term vanishes even at second order for zero-modes,
\begin{align}
\delta^2 \Delta I_\brane =& \int \sqrt \frac 1 2 h^{ab} \delta h_{ab} \left( \frac{G_{cd}}{16 \pi G_\brane} - \frac 1 2 \Delta T h_{cd}) \delta h^{cd} \right) \\
&+ \int \sqrt{h} \left( \frac{\delta G_{cd}}{16 \pi G_\brane} - \frac 1 2 \Delta T \delta h_{cd}\right) \delta h^{cd}.
\end{align}
The first equation vanishes by definition of $\Delta T$, while the second line vanishes for on-shell $\delta h_{ab}$. Note that the on-shell modes are precisely the zero-modes of Randall-Sundrum. The KK-modes are off-shell. For them, adding DGP terms changes the coupling.


\subsubsection{Randall--Sundrum}
We can treat the RS scenario as a toy model for our case. We aim at understanding what the effect of adding a DGP term is. Without a DGP term, the graviton bulk solutions take the form
\begin{align}
\psi = A \left(|z| + \frac 1 k\right)^{1/2} J_2\left( m\left(|z| + \frac 1 k\right) \right) + B \left(|z| + \frac 1 k\right)^{1/2} Y_2\left( m\left(|z| + \frac 1 k\right) \right).
\end{align}
Close to the origin, where the condition
\begin{align}
\psi'(0) = - \frac 3 2 k \psi(0)
\end{align}
holds, we can approximate
\begin{align}
J_2 \sim \frac{m^2 (|z| + \frac 1 k)^2}{8} \\
Y_2 \sim - \frac{4}{\pi m^2 (|z| + \frac 1 k)^2} - \frac 1 \pi.
\end{align}
From this we obtain
\begin{align}
\psi(0) = A \frac {m^2} 8 \frac 1 {k^{5/2}} - B \left( \frac{4 k^{3/2}}{\pi m^2} + \frac 1 {\pi k^{1/2}} \right) \\
\psi'(0) = A \frac 5 2 \frac {m^2} 8 \frac 1 {k^{3/2}} + B \left( \frac 3 2 \frac{4 k^{5/2}}{\pi m^2} - \frac {k^{1/2}}{2 \pi } \right).
\end{align}

Adding a DGP term modifies the coupling to the brane to
\begin{align}
T_\brane \to T_\brane (1 + \frac{m^2}{16 \pi G_\brane T_\brane}) = T_\brane (1 + \frac{m^2 L^2}{12} \frac{G_\mt{bulk}}{L G_\brane}) \equiv T_\brane \lambda.
\end{align}
The term which multiplies the delta-function in the equations of motion thus gets multiplied, $k \to \lambda k$. While this leaves the bulk solution unchanged, the condition at the brane changes to
\begin{align}
\psi'(0) = - \frac 3 2 k \lambda \psi(0).
\end{align}
In terms of the solutions we find that
\begin{align}
\frac A B = \frac 8 {5 + 3\lambda} \frac{k^2}{\pi m^2} \left(12 (\lambda - 1) \frac {k^2}{m^2} + (3 \lambda + 1) \right).
\end{align}
The case without DGP terms is $\lambda = 1$ and we find
\begin{align}
\frac A B = \frac{4 k^2}{\pi m^2}.
\end{align}
The vanishing of the first term, however, suggests some fine-tuning.
If we substitute the expression for $\lambda$ we end up with ($2G_\mt{bulk} = G_\mt{eff} L$)
\begin{align}
\label{eq:ratioAB2}
\frac A B = \frac 8 {5 + 3\lambda} \frac{k^2}{\pi m^2} \left(\frac{G_\mt{eff}}{2 G_\brane} + 4 + \frac{m^2}{4 k^2} \frac{G_\mt{eff}}{2 G_\brane} \right).
\end{align}
We are now especially interested in the coupling of the fairly light KK modes, \ie $m L \ll 1$. For positive values of $G_\brane$, we see that the relative strength of both terms in the linear combination changes, 
\begin{align}
\frac A B = \frac{4 k^2}{\pi m^2} \left(1 + \frac{G_\mt{eff}}{8 G_\brane} \right).
\end{align}
However, if we choose $G_\brane$ negative and are close to regime where
\begin{align}
\frac{G_\mt{eff}}{G_\brane} \sim - 8, 
\end{align}
we can make the first two terms in the parenthesis cancel. We end up with 
\begin{align}
\frac A B \sim - \frac 4 \pi \sim \text{constant}.
\end{align}
This would mean that the ``non-normalizable'' modes are not suppressed for light masses anymore.

The next obvious question is what is the forbidden range for $\frac{G_\mt{eff}}{2 G_\brane}$? Since the effect of massive KK modes on the gravitational coupling is exponentially suppressed by a Yukawa term, we can focus on only the light KK modes. Requiring that the first two terms of equation \eqref{eq:ratioAB2} dominate and approximating the last term by $0$, we find 
\begin{align}
 \frac{4}{G_\mt{eff}} \gg - \frac{1}{2 G_\brane}.
\end{align}
Up to numerical factors of order $\mathcal O(1)$, this agrees with the condition on $G_\brane$ in the main text, which came from a lower bound on $(1+\lambda_B)$.




\subsubsection{Our setting}
Let us discuss gravity in our case in more detail. We consider slicing coordinates
\begin{align}
\frac{1}{\sin(\mu)^2} \left(d\mu + ds^2_{AdS, d}\right).
\end{align}
Let us call indices in the $d+1$-dimensional spacetime $M,N,\dots$ and in the slices $i,j,\dots$. The non-vanishing Christoffel symbols are
\begin{align}
\Gamma^\mu_{\mu\mu} = -cot(\mu) && \Gamma^i_{j\mu} = -cot(\mu) \delta^i_j && \Gamma^\mu_{ij} = cot(\mu) \tilde g_{ij} && \Gamma^i_{jk} = \tilde \Gamma^i_{jk},
\end{align}
where tilde denotes objects with respect to the metric on the slices.
Gauge freedom allows us to fix $d+1$ components on the metric fluctuation. In order make good use of the symmetries of our system we go to a Fefferman-Graham-like gauge, where we set all components of the metric involving $\mu$ to zero.
If we assume a Lagrangian of the form
\begin{align}
L = R - (d-1)(d-2) \Lambda,
\end{align}
the linearized equations of motion in the bulk can be brought to the form\footnote{Note that in transverse-traceless gauge, the equations simply take the form $\frac 1 2 \Box h_{ab} - \Lambda h_{ab} = 0$.}
\begin{align}
\frac 1 2 \Box h_{ab} + \frac 1 2 g_{ab} \nabla^d \nabla^c h_{cd} - \frac 1 2 g_{ab} \nabla_d \nabla^d h^{c}_{c} + \frac 1 2 \nabla_a \nabla_b h^c_c - \frac 1 2 \nabla^c \nabla_a h_{bc}- \frac 1 2 \nabla^c \nabla_b h_{ac} + (d-1) \Lambda (h_{ab} - \frac 1 2 g_{ab} h^c_c) = 0.
\end{align}
We will start by computing the terms one by one, everthing with indices upstairs, though. The calculations are done by expanding the derivatives with xAct and then continuing by hand.
\begin{align}
(\Box h)^{\mu\mu} &= 2 \Gamma^{\mu}_{ij} \Gamma^\mu_{kl} g^{ik} h^{jl} \\
&= 2 \cos^2 \mu \sin^2 \mu h^c_c\\
(\Box h)^{\mu i} &= \partial_l (h^{ki} \Gamma^\mu_{jk} g^{lj}) + \Gamma^\mu_{jk} (\tilde \nabla^l h^{ik}) + \Gamma^i_{ml} g^{jl} \Gamma^\mu_{kj} h^{mk} - \Gamma^k_{kl} g^{lm} \Gamma^\mu_{mj} h^{ij}\\
(\Box h)^{ij} &= 
\end{align}
\begin{align}
\nabla^d \nabla^c h_{cd} &= \tilde \nabla_i \tilde \nabla_j h^{ij} + \partial_\mu(\Gamma^\mu_{ij} h^{ij}) + h^{ij} \Gamma^\mu_{ij} \Gamma^\mu_{\mu\mu} \\
&= \tilde \nabla_i \tilde \nabla_j h^{ij} + \sin \mu \partial_\mu (\cos \mu  h^c_c)
\end{align}
\begin{align}
\nabla_i \nabla_j h^c_c &= \tilde \nabla_i \tilde \nabla_j h^c_c - \Gamma^\mu_{ij} \partial_\mu h^c_c\\
&=\tilde \nabla_i \tilde \nabla_j h^c_c - \cos(\mu)\sin(\mu) g_{ij} \partial_\mu h^c_c\\
\nabla_\mu \nabla_\mu h^{c}_c &= \partial_\mu \partial_\mu h^c_c - \Gamma^\mu_{\mu\mu} \partial_\mu h^c_c.
\end{align}
\begin{align}
\nabla^i \nabla^j h^M_M &= \tilde \nabla^i \tilde \nabla^j h^M_M + \Gamma^i_{k\mu} g^{kj} g^{\mu\mu} \partial_\mu h^M_M\\
\nabla^\mu \nabla^\mu h^{M}_M &= g^{\mu\mu} \partial_\mu(g^{\mu\mu} \partial_\mu h^M_M) + g^{\mu\mu}g^{\mu\mu} \Gamma^\mu_{\mu\mu} \partial_\mu h^M_M
\end{align}
\begin{align}
\nabla_c \nabla^\mu h^{\mu c} = \Gamma^\mu_{cf} g^{\mu\mu} (\partial_\mu h^{fc} + \Gamma^c_{\mu e} h^{fe} + \Gamma^f_{\mu d} h^{dc}) + \Gamma^\mu_{cf} g^{fe} \Gamma^\mu_{ed} h^{dc}
\end{align}
The $\mu\mu$ component of the equations of motion thus becomes
\begin{align}
\frac 1 2 \Box h^{\mu\mu} + \frac 1 2 g^{\mu\mu} \nabla^M \nabla^N h_{MN} - \frac 1 2 g^{\mu\mu} \nabla_M \nabla^M h^N_N + \frac 1 2 \nabla^\mu \nabla^\mu h^M_M - \nabla^M \nabla^\mu h^\mu_M - \frac{\Lambda}{2}(d-1) g^{\mu\mu} h^M_M = 0. 
\end{align}

The goal now is to impose on-shell-ness of the gravitons the $d$-dimensional slice at the location of the brane (these are the zero-modes) and solve for the behavior in $\mu$ direction, after we have added a source term at the boundary.

\subsection{More detailed description about how holographic works}
everything is commented out.
 %Nonetheless, we expect that the CFT on the dynamical theory can still be treated as approximately holographic. On the asymptotic AdS boundary the Dirichlet boundary condition plays the role of sources while on the Planck brane, sources are the Neumann boundary conditions. \dn{Not sure anymore whether the story is that simple} \vc{I'm not sure how Neumann boundary conditions can be treated as sources. (For Dirichlet, we can say that a source is given by the coefficient of the $\sim z^{d-\Delta}$ part of a bulk field fixed by the Dirichlet boundary conditions; For Neumann boundary conditions, we don't to fix the $\sim z^{d-\Delta}$ asymptotic value of the fields, so I'm not sure what to equate the source to.)}

% At any fixed time-slice, we can separate the low lying operator spectrum into two pieces. There are light bulk-CFT operators which are dual to the fields away from the brane. Their dimensions are almost the same as those of the CFT without the defect. Secondly, there are defect operators, which describe excitations close to the brane. This set of operators will again almost look like the operator spectrum of a holographic CFT. \dn{$G_{eff}$ characterizes the ``number of channels'' between the brane CFT and the asymptotic CFT. This is fairly obvious from the gravitational perspective: Large $G_{eff}$ corresponds to a large overlap of the graviton wavefunction with modes away from the brane, \ie the effective brane theory loses information into the bath through a non-local(?) effect. What does this correspond to in the boundary perspective?}

%\dn{Can we make an argument, where we approximate the correlator by the length of a geodesic and relate this to the boundary entropy? For example in 2D, the boundary entropy should scale with be $\tilde c_T$ and }

% \dn{Preliminary:} We can be a bit more precise: Consider the CFT correlator
%\begin{align}
%\langle \mathcal O_\mt{bulk} \mathcal O_\mt{bdry} \rangle \sim \left(\frac{c_T}{\tilde c_T}\right)^{m/2}.
%\end{align}
%The scaling can be heuristically motivated as follows. At large $N$, a single trace operator $\mathcal O$ creates a single particle state with unit amplitude. The state consists of some power, $(\tilde c_T)^{m/2}$, of the degrees of freedom with equal probability. If $c_T$ is much smaller than $\tilde c_T$, then 

%For the stress energy two-point function, this indicates that 
%\begin{align}
%\langle T_{brane} T_{bath} \rangle \sim \sqrt{c_{bulk} c_{bdry}} \frac{c_{bulk}}{c_{bdry}}.
%\end{align}
%Holographically, this becomes  
%\begin{align}
%\langle g_{bulk} g_{bulk} \rangle \sim \sqrt{\frac{1}{G_\mt{bulk} G_\mt{eff}}}  \frac{G_\mt{eff}}{G_\mt{bulk}},
%\end{align}
%where the propagator on the left is the bulk-to-brane propagator. Note that this the correlator between graviton bound state and bulk gravitons must be much smaller.

%Again, we can remove the first square-root by choosing the canonical normalization of the two-point function. The second factor is the coupling between the gravity theory and the bath. It would be interesting if we could derive this using more detailed CFT methods.  


==> sections/ensemble-app.tex <==
% !TEX root = ../lifeonbrane3.tex
%



\rcm{lots of new references to read}

In order to derive the island formula, the appearance of wormholes in the replica trick is a crucial ingredient.
In the two-dimensional models involving JT gravity studied so far \cite{Almheiri:2019qdq,Penington:2019kki}, the existence of wormholes follows from the fact that JT gravity is defined by ensemble averaging over an ensemble of Hamiltonians.\footnote{For example, JT gravity emerges as the low energy effective description of the SYK model \cite{}, or has a UV complete definition in terms of a matrix model \cite{Saad:2019lba}.} In fact, by assuming ensemble averaging, one can easily reproduce many features \cite{Marolf:2020xie} demonstrated in the 2d models. 

However, it is generally assumed that in higher dimensions gravity on asymptotically AdS spacetimes is dual to a single, unitary theory.\footnote{The best known example is the duality between $\mathcal N=4$ super Yang-Mills theory and supergravity (or more precisely Type IIB string theory) on AdS${}_5\times S^5$.} In fact, in the higher dimensional case one would expect replica wormholes to be absent in any local theory. This can be seen by considering a theory on a higher-dimensional spacetime which couples to gravity in a subregion $U_\text{grav}$, and lives on a fixed background in the complement $U_\text{bath}$. If we want to compute the density matrix of a region $A \subset U_\text{bath}$, we are instructed to integrate out all degrees of freedom in the gravitating region $U_\text{grav}$. If we take products of the reduced density matrix -- like we would do in the replica trick -- no integral over the gravitating region is left to be performed and no Euclidean wormholes appear. More generally, in two dimensions, replica Wormholes appear in calculations of the spectral form factor and yield to a non-factorizability of products of the partition function. However, for a CFT${}_d$ the partition function is a number and a product of many partition functions clearly must factorize.

This opens the question if and how islands and replica wormholes appear in the higher dimensional case. As we have seen, in our model, they are readily explained from the bulk perspective, but in order to go beyond the case of holographic matter, it is important to also understand how they arise in the brane picture. Here, we will explain a possible mechanism suggested by the model discussed in this paper, and its relation to ensemble averaging.

As discussed in this paper, the description of the brane theory as a local CFT with a cutoff coupled to gravity in some region of space is only an effective one. In fact, we see from the bulk picture that the degrees of freedom in $U_\text{bath}$ and $U_\text{grav}$ are not independent. A particularly clear sign is the fact that under certain conditions parts of the gravitating region $\mathcal I_A \subset U_\text{grav}$ lie in the entanglement wedge of bath subregions $A \subset U_\text{bath}$. This signalled the appearance of an island on the brane picture. In this case, as is clear from EW reconstruction, specifying the state in $A$ also specifies the state in the island $\mathcal I_A$. In the presence of a brane, new bulk modes appear, which can be identified with the now-dynamical metric and sources of other primary operators on the brane. Specifying the state in $\mathcal I_A$ thus in particular means to specify the states of the metric and all other sources. The description that takes into account the link between degrees of freedom in the bath and the gravitating region corresponds to the full quantum gravity description of the state of \cite{Almheiri:2019yqk}.

In an effective, local and semi-classical approximation this link between the bath and the gravitating region is ignored so that $A$ and its associated island $\mathcal I_A$ are treated as independent subregions. If we are interested in a reduced density matrix $\rho^\text{s.c.}_A$ of a $A$ in the semi-classical approximation, we can obtain it from a fully quantum gravity density matrix $\rho^\text{q.g.}_A$, containing information of $A$ and $\mathcal I_A$, by treating the degrees of freedom in $\mathcal I_A$ as independent and tracing over them. Now, consider taking a product of $n$ density matrices $(\rho^\text{q.g.}_A)^n$. If we want to go to the semi-classical picture, we need to trace over the state on $\mathcal I_A$,
\begin{align}
(\rho^\text{s.c.}_A)^n = \tr_{\mathcal I_A}((\rho^\text{q.g.}_A)^n)
\end{align}
This correlates the states of the metric, quantum fields and other sources in any of the replica copies of $\mathcal I_A$ in the product. Moreover, since the trace also runs over modes which are associated with sources on the brane, this procedure effectively looks like ensemble averaging the sources on $\mathcal I_A$. This ensemble averaging then has an immediate description in terms of including Euclidean wormholes in the path integral.\\


==> sections/holoface.tex <==
% !TEX root = ../lifeonbrane3.tex
%

Our setup can be interpreted from three different `holographic' perspectives, which are analogous to the three descriptions of \cite{Almheiri:2019hni} \dn{We should really work through the references again and also give Karch-Randall credit where due.}, suitably generalised to arbitrary dimensions.  In this section we review each one of them, and explore their relation. 

First, we have the {\it bulk gravity perspective} corresponding to the geometric picture portrayed in section \ref{BranGeo}: we have an AdS$_{d+1}$ bulk region where gravity is dynamical, containing a DGP brane with tension running through the middle of the spacetime  -- see figure \ref{fig:threetales}a. The induced geometry on the brane is AdS$_d$. In the second picture, we integrate out the bulk action from the asymptotic boundary -- where gravity is frozen -- up to the brane, giving rise to Randall-Sundrum gravity \cite{Randall:1999vf,Randall:1999ee} on the brane. From the resulting {\it brane perspective}, the CFT$_d$ is then supported in a region with dynamical gravity (\ie the brane) and another non-dynamical one (\ie the asymptotic boundary) -- figure \ref{fig:threetales}b. Finally, the third description makes full use of the AdS/CFT dictionary, by using holography {along} the brane. This {\it boundary perspective} describes the system as a CFT$_d$ coupled to a conformal defect that stands at the position where the brane intersects the asymptotic boundary -- see figure \ref{fig:threetales}c. 

A holographic system was presented in \cite{Almheiri:2019hni} to describe the evaporation of two-dimensional black holes in JT gravity. This system has three descriptions analogous to those above. Of course, it also includes certain elements that we did not introduce in our model, \ie end-of-the-world branes to give a holographic description of conformal boundaries separating various components  \cite{Takayanagi:2011zk,Fujita:2011fp} and performing a $\mathbb Z_2$ orbifold quotient across the Planck brane, \ie the brane supporting JT gravity. However, the essential ingredients are the same as above. The boundary perspective in \cite{Almheiri:2019hni} describes the system as a two-dimensional holographic conformal field theory with a boundary, at which it couples to a (one-dimensional) quantum mechanical system -- figure \ref{fig:threetales}f. With the brane perspective, the quantum mechanical system is replaced by its holographic dual, the Planck brane supporting JT gravity coupled to another copy of the two-dimensional holographic CFT -- see figure \ref{fig:threetales}e. Finally, the bulk gravity perspective replaces the holographic CFT with three-dimensional Einstein gravity in an asymptotically AdS$_3$ geometry. Because of the $\mathbb Z_2$ orbifolding, the latter effectively has two boundaries, the standard asymptotically AdS boundary and the dynamical Planck brane -- see figure \ref{fig:threetales}d.

This initial model \cite{Almheiri:2019hni} raised a number of intriguing puzzles. For example, as emphasized in \cite{Almheiri:2019yqk}, implicitly two different notions of the radiation degrees of freedom are being used: one being the semi-classical approximation and the other one in the purely quantum theory. As we discuss in section \ref{sec:discussion}, our construction in higher dimensions provides a resolution of several of these questions.

\begin{figure}[h]
	\def\svgwidth{0.9\linewidth}
	\centering{
		\input{ThreeTales_EditcopyJS4.pdf_tex}
		\caption{This figure shows the relation between a time-slice in our construction and the holographic setup of \cite{Almheiri:2019hni}. The top row illustrates three perspectives with which the system discussed here can be described, while the bottom row displays the analogous descriptions of the model in \cite{Almheiri:2019hni}. The comparison can be made more precise by adding a $\mathbb Z_2$ orbifold quotient across the bulk brane/conformal defect in the top row. \rcm{Reordered to agree with tweaked discussion. Please put the QM/Planck brane on the left, and make the Planck brane a smooth arc.} \josh{I tried with a smooth arc, but it looks more confusing and is harder to relate to the previous papers.}\\
			\textbf{(a)} AdS$_3$ formulation with two boundary components: the asymptotic boundary (straight black line) and a ``Planck brane'' (wiggly black line). \\ 
			\textbf{(b)} The bulk spacetime has a holographic description as a 2D CFT coupled to gravity (shaded green). The CFT extends into a region with fixed metric (blue).\\
				\textbf{(c)} Microscopic dual description as a 2D BCFT (blue) coupled to a quantum mechanical system at its boundary (green).\\
			\textbf{(d)} Bulk gravity description with an AdS$_{d+1}$ space (shaded blue) which contains a co-dimension one Randall-Sundrum brane (shaded grey).\\ 
			\textbf{(e)} The dual CFT$_d$ (blue) now extending into an AdS$_d$ region where gravity is dynamical (shaded green).\\
			\textbf{(f)} Pure boundary description as a CFT$_d$ on $S^{d-1}$ (blue) with a co-dimension one defect (green).
		}
		\label{fig:threetales}
	}
\end{figure}




\begin{figure}[h]
	\def\svgwidth{1\linewidth}
	\centering{
		\input{bulkmodes_JSedit.pdf_tex}
		\caption{This figure illustrates the spatial profile of the first few normalized graviton modes with the slicing coordinate $\mu$, related to $\rho$ in eq.~\reef{metric} by $\tan\mu = 1/\sinh\rho$. \rcm{Or did you mean arcsinh$\rho$??} The left plot shows the spectrum in global AdS$_5$ and the right plot displays the bulk spectrum of gravitational modes in the presence of a large tension brane, \ie $\mu_\mt{B}\simeq\pi/2$, and a $\mathbb Z_2$ orbifolding across the brane. The tension is adjusted such that the location of the brane is at $\mu = \mu_\mt{B}$. As discussed in the main text, in the presence of the brane new bulk modes appear (orange) which are highly localized at the brane and subleading with respect to the other bulk modes at the asymptotic boundary at $\mu = 0$. Those modes play the role of the graviton localized to the brane. The remaining bulk modes remain essentially unchanged and appear as KK modes in the brane theory. \iar{I would leave only the RHS figure, and as a sketch rather than plot. The results can be promised for another paper.} \rcm{I tend to agree with Ignacio. We're filling the page with alot of white space here. Perhaps the profiles become clearer if you push $\mu_\mt{B}$ further from $\pi/2$. You say the regular bulk modes are ``essentially unchanged'' but what is the significance of the spikes in those profiles at the brane? If you plotted both pictures on top of each other, would we see any difference in the green and purple profiles?}
                  \vc{In our model, do we expect there to be quantum fluctuations of the spikey green and purple modes (in the left figure) in the bulk (which fulfill the role ordinarily played by normalizable graviton modes in braneless AdS/CFT)? E.g. would they contribute to the matter part of the generalized entropy of a bulk region?}
                }
                \label{fig:boundstate} 	}
\end{figure}

\rcm{My general sense is that below we are describing many/several(?) things that have been discussed elsewhere and so we should be including more references to the older RS/DGP literature.}

\paragraph{Bulk gravity perspective:} As discussed in section \ref{BranGeo}, the system has a bulk description in terms of gravity on an asymptotically AdS$_{d+1}$ spacetime containing a codimension-one brane, which splits the bulk into two halves -- see figure \ref{fig:threetales}a. The brane is characterized by the tension $T_o$ and also the DGP coupling $1/\Gbr$, introduced in eqs.\eqref{braneaction} and \eqref{newbran}, respectively. We can use the Israel junction conditions \reef{Israel1} to relate the brane stress-energy tensor to the discontinuity of the extrinsic curvature across the brane, which determines the location of the brane as embedded in the higher dimensional space. The backreaction causes warping around the brane, and after a change of coordinates, tuning the brane tension can be understood as moving the brane further to an asymptotic AdS region, as seen in eq.~\reef{positionbrane} or \reef{position}. For large brane tension, \ie with $\veps \ll 1$, the spectrum of graviton fluctuations in the bulk is almost unchanged with respect to the modes in empty AdS space. However, in addition to the modes which would normally be present in a holographic setting, gravitational states appear around the brane \cite{Randall:1999vf,Randall:1999ee,Karch:2000ct}, as illustrated figure \ref{fig:boundstate}. Their wavefunctions are highly localized around the brane, but only subleading close to the asymptotic boundary compared to all other bulk modes. The strong localization is caused by the nonlinear coupling of gravity to the brane. Unlike in the Randall--Sundrum model with a flat or de Sitter brane, these graviton modes are not true bound states, but merely very light states whose wavefunction peaks around the brane. As we will review below, the remaining graviton modes appear as Kaluza-Klein modes from the point of view of the theory on the brane. A similar set of localized modes appears for each bulk field, however, their boundary conditions at the brane differ from that of the graviton. for example, scalar field fluctuations have a vanishing normal derivative at the brane. 

By deforming the theory on the brane, it is possible to change the boundary condition of bulk modes at the brane. Such deformations can be realized by adding `generalized DPG couplings' to the brane which couple the bulk fields, and their derivatives to the brane. We leave a general investigation of such couplings for future work. As discussed in section \ref{sec:DGP}, here we focus here on the Einstein-Hilbert term \reef{newbran} for the the induced metric on the brane \cite{Dvali:2000hr}. In our setup, at the same time, we added a counterterm to the tension, with $\Delta T$ tuned as in eq.~\reef{tune3} to ensure that the warping, or equivalently the location of the brane, is unchanged. With this choice, the effect of the DGP term is to modify the coupling of different bulk graviton modes to the brane and thus modify the spectrum of bulk modes. This works as follows. After adding a DGP term, bulk fluctuations of the metric $h(x,z)$ have to obey equations of motion of the form
\begin{align}
\partial^2_z h(x,z) + \dots = \delta(z - z_B) \left(b \tilde h(x) + \frac{\kappa}{\Gbr} ( \partial_x^2 \tilde h(x) - \Lambda_\text{brane} \tilde h(x)) \right),
\end{align}
where $\tilde h$ is the induced metric on the brane. The left hand side comes from varying the equations of motion in the bulk, while the right hand side gives the discontinuity $b$ of the normal derivatives before adding the DGP terms. The term multiplied by $\frac{\kappa}{\Gbr}$ is the contribution of the DGP term in transverse-traceless gauge for the brane graviton. The ellipsis represents terms which are unimportant in the following, $\kappa$ is some unimportant constant we use to absorb numerical factors, and we have dropped the indices of $h$.

Integrating this equation in a small neighbourhood around the brane gives a condition on the normal derivative
\begin{align}
\partial_z h_L(x,z_B) - \partial_z h_R(x,z_B) = b \tilde h(x) + \frac{\kappa}{\Gbr} ( \partial_x^2 \tilde h(x) - \Lambda_\text{brane} \tilde h(x))
\end{align}
This condition, together with the Dirichlet condition at the asymptotic AdS boundary, determine the spectrum of bulk fluctuations. Expanding metric fluctuations in modes along and orthogonal to the brane $h(x,z) = h_{m,\dots}(z)h_{m,\dots}(x)$ with $ \partial_x^2 \tilde h(x) - \Lambda_\text{brane} \tilde h(x) = \tilde m^2 \tilde h_{m,\dots}(x)$ it is easy to see that the boundary condition is modified for each mode which is not a zero mode. For negative $\Gbr$ this leads to a squeezing of the spectrum \dn{Still need to check}. A more quantitative discussion of this mechanism and its interpretation from the point of view of the CFT will appear in \cite{domino}.

%The modification of the graviton mode couplings is determined by the DGP Newton's constant $G_\brane$. \rcm{expand on last three sentences, please; end by forshadowing a more detailed quantitative discussion in \cite{domino}.}


\dn{Maybe move the rest of the discussion to the respective sections.}

By the holographic dictionary, the boundary condition determines the defect operator spectrum. In particular the change is such that for negative $G_\brane$ the defect operator spectrum gets squeezed around the zero mode. This makes the contribution more important at lower energies. 


\rcm{Would be good to discuss the squeezing of the KK spectrum -- and how this makes them important at lower energies, and pointing to the statement that negative $\lamb$ produces negative anomalous dimensions for defect operators, which appears in the discussion section.}



\paragraph{Brane perspective:} This second perspective, discussed in section \ref{indyaction}, effectively integrates out the spatial direction between the asymptotically AdS boundary and the brane to produce an effective action for Randall-Sundrum gravity on the brane, with the new localized graviton state playing the role of the $d$-dimensional graviton. Hence we are left with a $d$-dimensional theory of gravity coupled to (two copies of) the dual CFT on the brane -- see figure \ref{fig:threetales}b. Amongst the new localized bulk modes, we have an almost massless graviton but also a tower of massive Kaluza-Klein states. However, as shown in \cite{Karch:2000ct}, those massive states are above the cutoff scale of the effective theory on the brane.
In section \ref{indyaction}, we demonstrated the consistency between the bulk gravity perspective and the brane perspective by observing how the equations of motion of the new effective action fix the brane position in the ambient spacetime. Of course, the bulk physics are also dual to the boundary CFT on the asymptotic AdS$_{d+1}$ boundary, and so this perspective is completed by coupling the gravitational and CFT degrees of freedom on the brane to the CFT on the fixed boundary geometry. We refer to that latter as the {\it bath} CFT. Next, we discuss how different parameters in the brane perspective are related to bulk parameters. 

There are four independent parameters which characterize the gravitational theory on the brane: the curvature scale $\ell_\mt{eff}$, the effective Newton's constant $G_\mt{eff}$, the central charge of the boundary CFT $\cT$, and the effective short-distance cutoff $\tilde\delta$. These emerge from the bulk theory through the four parameters characterizing the latter: the bulk curvature scale $L$, the bulk Newton's constant $\Gbk$, the brane Newton's constant $\Gbr$ and the brane tension $T_o$.\footnote{Recall that $\Delta T$ is determined by these parameters in eq.~\reef{tune3}, as well as eqs.~\reef{positionbrane} and \reef{curve1}.} From eq.~\reef{Newton2}, we see that $\ell_\mt{eff}$ is determined by a specific combination of $T_o$, $\Gbk$ and $L$. Similarly, $G_\mt{eff}$ is determined by $\Gbr$, $\Gbk$ and $L$ in eq.~\reef{Newton33}. Of course, the central charge of the boundary CFT is given by the standard expression $\cT\sim L^{d-1}/G_\mt{bulk}$, \eg see \cite{Buchel:2009sk}. We discuss how the effective cutoff $\tilde\delta$ emerges next.

As discussed in section \ref{indyaction}, the bulk analysis makes evident that the theory on the brane comes with a short-distance cutoff, \ie the description in terms of gravity coupled to a CFT breaks down at short distances of order $\tilde\delta\sim L$. As noted above,  this breakdown can be understood in terms of the strong coupling of the higher `Kaluza-Klein' modes to physics at shorter scales. Of course, one can also understand this effect directly from the brane perspective. In this case, there are actually a number of different effects that must be considered. 

Recall that integrating out the bulk (or their dual CFT) degrees of freedom produces a series of higher curvature terms in the effective action \reef{act3}, and hence demanding that $d$-dimensional Einstein gravity provides a good approximation of the brane theory introduces constraints. The suppression of these higher curvature corrections requires that the ratio $L/\ell_\mt{eff}$ be small. However, if we examine eq.~\reef{act3} carefully and note the distinction $G_\mt{eff}\ne G_\mt{RS}$, then suppressing the curvature-squared terms requires that
\beq
\frac{1}{1+\lamb}\,\frac{L^2}{\ell_\mt{eff}^2}
\ll 1\,,
\label{lmfao}
\eeq
using eq.~\reef{Newton34}.  As noted in section \ref{indyaction}, for a pure RS brane with no additional DGP gravity, \ie $\lambda_b=0$, we conclude that the short distance cutoff is $\tilde\delta\sim L$. More generally then, the above expression suggests that the DGP term \reef{newbran} affects a shift producing a new short-distance cutoff 
\beq
\tilde\delta\sim \frac{L}{\sqrt{1+\lamb}}\,.
\label{haiku}
\eeq
We should note that this result only applies for $d>4$. For $d=4$, the coefficient of the curvature-squared term is logarithmic in the cutoff, while for $d=2$ or 3, this interaction is not associated with a UV divergence.

While the above is a UV effect, there also IR effects resulting from having a large number of matter degrees of freedom propagating on the brane, as explained in \cite{Dvali:2007hz,Dvali:2007wp,Reeb:2009rm}. The usual regime of validity for QFT in semiclassical gravity lies at energy scales below the Planck mass, or at distance scales larger than $G_\eff^{1/(d-2)}$. However, with\vc{remove ``with''?} the boundary CFT has a large number of degrees of freedom, as indicated by the large $\cT$ CFT \vc{remove ``CFT''?}, and hence the semiclassical description of gravity in fact breaks down much earlier. A direct way to see this breakdown \cite{Dvali:2007wp} is to consider the computation of the (canonically normalized) graviton two-point function:\footnote{This propagator argument can also be applied for the higher curvature terms discussed above. For example, the curvature-squared terms gives a perturbative correction: $\langle h(p) \,h(-p)\rangle \sim p^{-2}\[1 + \frac{L^2}{1+\lamb}\, p^{2}+\cdots\]$. Hence this approach yields the same result for the cutoff in eq.~\reef{haiku}.}
\beq
\langle h(p)\, h(-p)\rangle \sim p^{-2}\[1 + \cT\, G_\eff\, p^{d-2}+\cdots\]\,.
\label{Dvali1}
\eeq
Here, the leading correction arises from a diagram involving the external gravitons coupling to the CFT stress tensor two-point function. We see that such corrections are only suppressed relative to the `tree-level' result for momenta below a cutoff scale of order $(\cT G_\eff)^{-1/(d-2)}$. 
For our model, the gravitational theory of the brane can therefore only be treated semiclassically for distance scales larger than
\beq
\tilde\delta\sim (\cT G_\eff)^{1/(d-2)} \sim \frac{L}{(1+\lambda_b)^{1/(d-2)}}\,.
\label{Dvali2}
\eeq
Again, for a pure RS brane with $\lambda_b=0$, we reproduce the expected short distance cutoff $\tilde\delta\sim L$. However, the addition of a DGP gravity term again modifies the cutoff, but in a manner distinct from eq.~\reef{haiku}, produced by the higher curvature terms. Note that the above result applies for $d\ge 3$.

The distinction between these two cutoffs indicates that these are really two different physical phenomena contributing to the breakdown of Einstein gravity in the brane perspective. Note that $\lamb>0$, in both eqs.~\reef{haiku} and \reef{Dvali2}, the effect is to produce a shorter cutoff scale, however, the second limit \reef{Dvali2} is the first to contribute (where we are assuming $d>4$). On the other hand with $\lamb<0$, the cutoff $\tilde\delta$ is pushed to larger distance scales. In this case, eq.~\reef{haiku} is the first to modify the gravitational physics on the brane as we move to smaller distances. \rcm{Please check above paragraphs about $\tilde\delta$.}


In order to be in the semiclassical regime on the brane, we need to require that $\ell_\eff\gg \ell_\mt{P}$, or alternatively $\ell_\mt{eff}^{d-2}/G_\mt{eff}\gg 1$. \rcm{How does this differ from the opening statement in the previous paragraph??}
Using eqs.~\reef{Newton33} and \reef{newdefs}, we can also write this constraint as
\begin{align}\label{ineq}
1+\lamb\gg\frac{G_\mt{RS}}{\ell_\mt{eff}^{d-2}}\simeq\frac{1}{\cT}\,\frac{L^{d-2}}{\ell_\mt{eff}^{d-2}}\,.
\end{align}
By adjusting $T_o$ in eq.~\reef{Newton2}, we can always make $\ell_\mt{eff}$ as big as we want and hence the ratio on the right-hand side, as small as we want. However, when we fix this tuning, eq.~\eqref{ineq} becomes a constraint on how negative $\lamb$ may be, \ie $\lamb$ may not be arbitrarily close to --1. \rcm{I added the last expression in eq.~\reef{ineq} so that we can compare this constraint to setting $\tilde\delta\ll \ell_\eff$ in the previous paragraphs. The factor of $1/\cT$ seems to make this one a much weaker constraint, \eg compare to eq.~\reef{lmfao}.}\vc{Agreed; this paragraph just sounds like the one around \eqref{Dvali2}, except weakened by forgetting that the cutoff gets enhanced by large $c_T$.}

\rcm{The following seems an overreach:} In this case, it is natural to choose $G_\mt{brane}$ to be negative and we need to require that
\begin{align}
\frac 1 {G_\mt{RS}} \gg \left| \frac 1 {G_\mt{brane}} \right| && (G_\brane  < 0)\,,
\end{align}
\ie $|\lamb|\ll 1$. \vc{Probably a stupid question: where did this come from? Didn't the sentence below \eqref{ineq} just say that $T_o$ can be tuned such that \eqref{ineq} (or better yet $\ell_\eff\gg$\eqref{Dvali2}) is satisfied?}
From the bulk gravity perspective, this condition ensures that the graviton states which correspond to KK modes do not couple too strongly to the brane. \dn{Still need to double-check that statement.} 




It is important to note that with the brane perspective at least two approximations are made: First, as discussed above, the CFT in the region with dynamical gravity is only an effective theory with a cutoff scale with $\tilde\delta\sim L$. \vc{Does this need to be updated with \eqref{haiku} or \eqref{Dvali2}?}Second, the bulk graviton zero modes -- which become the gravitational degrees of freedom on the brane -- contribute small corrections to the stress-energy tensor in the bath CFT. However, in going to the brane perspective, those are ignored.

\paragraph{Boundary perspective:} As the preceding discussion has made clear, the theory obtained by integrating out the bulk between the asymptotic boundary and the brane, \ie the brane perspective, only provides an effective theory. However, the standard rules of AdS/CFT allow for a fully microscopic description of the system in terms of the boundary theory. This is obtained by integrating out the bulk -- including the brane -- and the result  is given by the bath CFT on the fixed $d$-dimensional boundary geometry coupled to a ($d$--1)-dimensional conformal defect (positioned where the brane reaches the asymptotic boundary, \ie the equator of the boundary sphere) -- see figure \ref{fig:threetales}c. Of course, the bath CFT is characterized by the central charge $\cT\sim L^{d-1}/G_\mt{bulk}$, while the defect is characterized by its defect central charge $\tilde{c}_\mt{T}\sim \ell_\mt{eff}^{d-2}/G_\mt{eff}$.

In the bulk, the brane tension controls the ratio $\ell_\mt{eff}/L$ which by the standard holographic dictionary\footnote{Remember that the AdS/CFT dictionary tells us that $G_N\sim \ell_\mt{AdS}^{d-1}/ N_{dof}$ and $\lambda\sim \ell_\mt{AdS}/\ell_\mt{s}$. \vc{Should the RHS of the second equation have a power of $\frac{d-1}{2}$?}} translates to $\tilde \lambda/\lambda$, the ratio of bulk and defect t'Hooft coupling. \vc{I'm blaming my string-illiteracy, but why should the bulk string length be equal to the `string length' of the effective theory on the brane? (It's not clear to me, if the brane/defect AdS$_d$/CFT$_{d-1}$ correspondence has a stringy interpretation, that it should be the same string theory describing the AdS$_{d+1}$/CFT$_d$ correspondence.)} At the same time, in the absence of DGP terms, increasing tension increases the defect central charge $\tilde c_\mt{T}$. The bulk parameters scale in terms of the defect CFT data as
\begin{align}
\frac{\ell_\mt{eff}}{L} \sim \frac{\tilde \lambda}{\lambda}, &&
\frac{L^{d-2}}{G_\brane} \sim \frac 1 {\tilde c_\mt{T}}\left(\left(\frac{\lambda}{\tilde \lambda} \right)^{d-2} - \frac{2}{d-2}\frac{\cT}{\tilde c_\mt{T}}\right).
\end{align}
\vc{Should the $\frac{1}{\tilde{c}_T}$ be replaced by $\tilde{c}_T$?}The requirement to be in the semiclassical regime on the brane then corresponds to
\begin{align}
\frac{\tilde c_\mt{T}}{\cT} \sim \left(\frac{\ell_\mt{eff}}{L}\right)^{d-2}\gg 1\,,
\end{align}
\vc{where did the $\sim$ come from? I'm finding an extra factor of $1+\lambda_b$ multiplying the RHS of the $\sim$ using \eqref{Newton34}. (According to \eqref{Dvali2}, the $\gg$ should still be fine.)}
which implies that the defect central charge must be much bigger than the bulk CFT central charge, $\tilde c_T \gg c_T$. This can be heuristically understood from the brane perspective: A large defect central charge is needed so that energy and information are only leaking very slowly from the dynamical gravity region into the bath. It has been argued that this ratio also sets the Page time \cite{Rozali:2019day}. With the boundary perspective, this can be understood as a requirement which ensures that the degrees of freedom of the defect and the CFT only slowly mix. \rcm{Revisit paragraph after brane perspective is sorted.}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../lifeonbrane3"
%%% End:


==> sections/wormholes-extra.tex <==

In order to derive the island formula, the appearance of wormholes in the replica trick is a crucial ingredient.
In the two-dimensional models involving JT gravity studied so far \cite{Almheiri:2019qdq,Penington:2019kki}, the existence of wormholes follows from the fact that JT gravity is defined by ensemble averaging over an ensemble of Hamiltonians.\footnote{For example, JT gravity emerges as the low energy effective description of the SYK model \cite{}, or has a UV complete definition in terms of a matrix model \cite{Saad:2019lba}.} In fact, by assuming ensemble averaging, one can easily reproduce many features \cite{Marolf:2020xie} demonstrated in the 2d models. 

However, it is generally assumed that in higher dimensions gravity on asymptotically AdS spacetimes is dual to a single, unitary theory.\footnote{The best known example is the duality between $\mathcal N=4$ super Yang-Mills theory and supergravity (or more precisely Type IIB string theory) on AdS${}_5\times S^5$.} In fact, in the higher dimensional case one would expect replica wormholes to be absent in any local theory. This can be seen by considering a theory on a higher-dimensional spacetime which couples to gravity in a subregion $U_\text{grav}$, and lives on a fixed background in the complement $U_\text{bath}$. If we want to compute the density matrix of a region $A \subset U_\text{bath}$, we are instructed to integrate out all degrees of freedom in the gravitating region $U_\text{grav}$. If we take products of the reduced density matrix -- like we would do in the replica trick -- no integral over the gravitating region is left to be performed and no Euclidean wormholes appear. More generally, in two dimensions, replica Wormholes appear in calculations of the spectral form factor and yield to a non-factorizability of products of the partition function. However, for a CFT${}_d$ the partition function is a number and a product of many partition functions clearly must factorize.

This opens the question if and how islands and replica wormholes appear in the higher dimensional case. As we have seen, in our model, they are readily explained from the bulk perspective, but in order to go beyond the case of holographic matter, it is important to also understand how they arise in the brane picture. Here, we will explain a possible mechanism suggested by the model discussed in this paper, and its relation to ensemble averaging.

As discussed in this paper, the description of the brane theory as a local CFT with a cutoff coupled to gravity in some region of space is only an effective one. In fact, we see from the bulk picture that the degrees of freedom in $U_\text{bath}$ and $U_\text{grav}$ are not independent. A particularly clear sign is the fact that under certain conditions parts of the gravitating region $\mathcal I_A \subset U_\text{grav}$ lie in the entanglement wedge of bath subregions $A \subset U_\text{bath}$. This signalled the appearance of an island on the brane picture. In this case, as is clear from EW reconstruction, specifying the state in $A$ also specifies the state in the island $\mathcal I_A$. In the presence of a brane, new bulk modes appear, which can be identified with the now-dynamical metric and sources of other primary operators on the brane. Specifying the state in $\mathcal I_A$ thus in particular means to specify the states of the metric and all other sources. The description that takes into account the link between degrees of freedom in the bath and the gravitating region corresponds to the full quantum gravity description of the state of \cite{Almheiri:2019yqk}.

In an effective, local and semi-classical approximation this link between the bath and the gravitating region is ignored so that $A$ and its associated island $\mathcal I_A$ are treated as independent subregions. If we are interested in a reduced density matrix $\rho^\text{s.c.}_A$ of a $A$ in the semi-classical approximation, we can obtain it from a fully quantum gravity density matrix $\rho^\text{q.g.}_A$, containing information of $A$ and $\mathcal I_A$, by treating the degrees of freedom in $\mathcal I_A$ as independent and tracing over them. Now, consider taking a product of $n$ density matrices $(\rho^\text{q.g.}_A)^n$. If we want to go to the semi-classical picture, we need to trace over the state on $\mathcal I_A$,
\begin{align}
(\rho^\text{s.c.}_A)^n = \tr_{\mathcal I_A}((\rho^\text{q.g.}_A)^n)
\end{align}
This correlates the states of the metric, quantum fields and other sources in any of the replica copies of $\mathcal I_A$ in the product. Moreover, since the trace also runs over modes which are associated with sources on the brane, this procedure effectively looks like ensemble averaging the sources on $\mathcal I_A$. This ensemble averaging then has an immediate description in terms of including Euclidean wormholes in the path integral.\\

